Long-Horizon AI Research for Grothendieck Constant: A Case Study in Human-AI Mathematical Collaboration

AI agents are increasingly used in mathematics research, but it is often unclear how to use them effectively. Towards this, we present an extensive case study of how AI was used to improve bounds on the Grothendieck constant $K_G$, which captures the hardness between combinatorial problems and their continuous relaxations. Specifically, while the precise value of $K_G$ is not known, we recently tightened the best known bounds to \[ \frac{6\pi}{11} \;\le\; K_G \;\le\; \frac{\pi}{2\log(1+\sqrt2)} - 10^{-4}. \] Crucially, these improvements were achieved using an AI research system that could arrive at insights deemed novel by domain experts. We give a detailed discussion of our experience using AI for mathematics research, particularly touching upon its strengths and weaknesses, as well as our experience with creating ideal conditions for AI to arrive at breakthrough insights.

==> old/ai_section.tex <==
% ============================================================================
% AI SECTION -- draft to be merged into the main paper as a single section.
% No abstract and no title: the \section below is the section itself.
% Style: anton_style.md. Items needing author confirmation are marked %% TODO.
% ============================================================================


\hypersetup{
  colorlinks=true,
  linkcolor=blue!55!black,
  urlcolor=blue!55!black,
  citecolor=blue!55!black
}

\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}
\setlist[itemize]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}
\setlist[enumerate]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}

\section{AI methodology and analysis}
\label{sec:ai}

{\color{red}AX: Overall, the opening before Subsection 11.1 is too long. It suffices to just have 1-2 paragraphs at most.}

The results in this paper were obtained in collaboration with an autonomous
AI research system. The cubic--quintic
construction and its certificate (Theorem~\ref{thm:cubic-quintic-upper-bound})
predate the current system and was found through conversation with GPT-5.5-Pro. The lower bound $\KG\ge6\pi/11$ was
discovered and first proved by the system; we have since verified the
argument ourselves, and the proof in this paper is our revision of the
system's write-up. The system also produced further improvements on both
sides of the problem, which we report in Section~\ref{sec:ai-results} but do
not state as theorems, because their certificates have not yet been human-verified. This section documents the methodology
(Section~\ref{sec:ai-methodology}), quantifies the run and its outcomes
(Section~\ref{sec:ai-results}), reconstructs how the lower bound was found
(Section~\ref{sec:ai-case-study}), and discusses what the record shows about
the strengths and weaknesses of current AI systems as mathematical
collaborators (Sections~\ref{sec:ai-discussion} and~\ref{sec:ai-future}).
{\color{red}AX: The discussion of cut-off dates belongs in some split of the methodology/discussions.
If you had to keep one paragraph, it would be this.
}


Recent successes of AI in mathematics, including on open problems, are of
a different kind from the work reported here. Evaluator-guided search has
produced record constructions~\cite{funsearch,novikov2025alphaevolvecodingagentscientific, charton2024patternboostconstructionsmathematicslittle},
and formal provers have shown proficiency at solving olympiad-level problems \cite{novikov2025alphaevolvecodingagentscientific}. In the
months surrounding our run, frontier models went further: an internal reasoning
model at OpenAI has disproved the Erd\H{o}s unit-distance conjecture
\cite{openai2026planarpointsets}, a mathematician has found a counterexample to the Jacobian conjecture using Claude Fable 5
\cite{jacobian}, and OpenAI has announced solutions, with formally
checked proofs, to ten open problems in mathematics and theoretical
computer science \cite{openai2026ten}. Most of these results involved resolving a single well-posed statement by construction. Moreover, none explicitly required significant long horizon reasoning. Finally, all of the recent results with frontier models were found fully autonomously, without sustained human intervention.
{\color{red}AX: Move to discussion. Also I'm not a fan of the ``in the months surrounding our run'' --- I think it's too fancy here. Let's just make this more standard ``recent and concurrent work'' that's happened to us.}

Our work is a more realistic example of how humans and AI can collaborate on mathematical research. The problem is more open ended, requiring a research program where over the course of weeks intermediate results accumulate and directions are opened and abandoned. Moreover, humans were consistently steering the system and providing feedback. We hope that our experiences outlined in this section will be useful to future mathematicians and AI researchers alike.
{\color{red}AX: Also move to discussion. It's also risky to explicitly claim that this is a ``more realistic example'', it could be more like: ``Our work is an extensive case-study ...'' or something like that?}



\subsection{Methodology}
\label{sec:ai-methodology}

{\color{red}AX: This is too dense. Tell Fable to explicitly split into the following paragraph groups: (1) AI models and compute: here you describe what models you used and you can also remark on the cut-off dates so that future readers have context. You can also add 1-2 sentences describing the server setup that you used.
(2) Harness: you can describe the harness system here.
(3) Run configurations
(4) Human interaction.
}

{\color{red}AX: Continuing from above: the current structure is kind of this split. It's more or less slapping on an explicit paragraph tag. However, the writing should be tightened to focus more on its assigned topic.}


The system uses a harness that couples two frontier language
models in distinct roles. A reasoning model (OpenAI GPT-5.5-Pro at maximal
reasoning effort, later GPT-5.6-Sol) serves as the brain, where it selects
directions, develops arguments, specifies experiments, and audits the
resulting claims. A coding agent (Anthropic Claude Code, running Claude Opus
and later Claude Fable~5) serves as the executor, where it maintains the project
repository, implements and runs experiments, retrieves literature, and
drives the reasoning model through a scripted interface. The harness was also adjusted repeatedly over the
run in response to observed failures. We describe its final form, to the
extent needed to interpret the record.


Work is organized into \emph{sessions} of a few hours, of which two to
five run concurrently on mutually distinct directions. No model context survives from
one session to the next, and instead continuity is carried by a single summary file that serves as
working memory and into which finished work is merged, and append-only
transcripts and experiment logs. A session passes through fixed phases:
orientation from the problem statement and summary files, selection of a focus, a research loop in
which the reasoning model requests computations, literature, or further
reasoning time, and a closing audit that produces a calibrated summary in
which every claim is tagged as proven, numerically supported, conjectural,
or heuristic. We reserve the word theorem, here and in the rest
of the paper, for statements that we have additionally checked ourselves.

The run started from a substantial base of our prior work rather than from
the problem alone. By June 2026 we had worked on the constant for several
months, and the harness was initialized with the results: the cubic--quintic scheme, the coefficient formulas and certification machinery, our accumulated notes, and a
problem statement listing candidate directions for both bounds. In
particular, the search space the run explored is a generalization of teh cubic--quintic scheme, and the possibility of converting
obstructions into lower bounds was raised, as a suggestion, in the problem
statement. The system therefore operated downstream of the mathematical
framework it was given, a point quantified in
Section~\ref{sec:ai-case-study}.

A human operator (one of the authors) steered the run asynchronously through
text files read at the start of, and during, every session. Steering
consisted of priorities, targets, audits of the run's own claims, and
occasional mathematical pointers; about forty dated directives were issued
over the run. The operator contributed no proof steps through this channel.

\subsection{Results}
\label{sec:ai-results}

The run spanned June~16 to July~24, 2026, It comprised
roughly 240 research sessions. The reasoning model was called 2{,}091
times, consuming about 152 million tokens at an estimated \$5{,}400 in
API cost; the coding agent ran on a flat-rate subscription (Claude Max). Floating-point searches ran
on a four-GPU node, and every certified computation was redone in interval
arithmetic on CPU. Table~\ref{tab:run} collects these figures, and
Table~\ref{tab:timeline} gives the timeline of the bounds.

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
Duration & June 16 -- July 24, 2026 (main phase through July 4)\\
Research sessions & $\approx240$\\
Reasoning model & GPT-5.5-Pro, later GPT-5.6-Sol; maximal effort\\
Usage and cost & 2{,}091 calls; $\approx152$M tokens; $\approx\$5{,}400$\\
Coding agent & Claude Code (Opus, later Fable 5); subscription\\
Human steering & one operator; $\approx40$ dated directives\\
\bottomrule
\end{tabular}
\caption{\textbf{The run at a glance.} Aggregates computed from the harness
telemetry. Dollar figures are list-price estimates; coding-agent usage was
only partially metered.
}
\label{tab:run}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lp{0.76\textwidth}@{}}
\toprule
Sessions & Event\\
\midrule
1 & run begins from the interval $1.6769566742\le\KG\le1.7818666070$
(the upper end is the cubic--quintic bound of this paper)\\
18 & upper-bound search plateaus; the operator directs a pivot to the
lower bound\\
44 & numerical upper bound $1.7802243$ recorded (later withdrawn)\\
55--57 & affine reframe; $\KG\ge6\pi/11$ derived\\
58--64 & $6\pi/11$ proof machine-audited; first \LaTeX{} write-up\\
p92, p117 & lower bounds $27\pi/49\approx1.7311$ and
$51\pi/92\approx1.7415$ machine-verified\\
follow-up & the session-44 value found unsupported by internal audit and
withdrawn\\
follow-up & upper bound $1.781801841033$ machine-certified\\
follow-up & upper bound $1.7813319810625639$ machine-certified;
adversarial review passed\\
\bottomrule
\end{tabular}
\caption{\textbf{Timeline of the bounds produced during the run.}
Machine-verified means accepted by the verification protocol of
Section~\ref{sec:ai-methodology}. The last three events fall in the short
follow-up phases, whose sessions we do not cite individually. Of the
run's results, only $\KG\ge6\pi/11$ has additionally been verified by the
authors; it is the result stated as a theorem in this paper.}
\label{tab:timeline}
\end{table}

The run's principal outcome, and the one this paper states as a theorem,
is the lower bound $\KG\ge6\pi/11$, whose discovery
Section~\ref{sec:ai-case-study} reconstructs. Beyond it, the run produced
machine-certified upper bounds of $1.781801841033$ and then
$1.7813319810625639$, improving on the cubic--quintic value, together with
the two stronger lower bounds listed in Table~\ref{tab:timeline}. We
report these as machine-verified claims rather than theorems: each passed
the full internal protocol, but we have not yet verified their
certificates ourselves.
%% TODO: reconcile with the main paper's discussion of concurrent work
%% (e.g. Heilman's computer-assisted improvement of Krivine's bound,
%% arXiv:2606.00247).

\subsection{Case study: the lower bound}
\label{sec:ai-case-study}

The lower bound is the run's main discovery. We reconstruct it here in
outline, highlighting the three human interventions that shaped it, since
the weaknesses discussed in Section~\ref{sec:ai-discussion} refer back to
them; the full logs of the sessions involved will be released with the rest
of the record.
{\color{red}AX: You don't have to refer to to-be-released artifacts here.
Tell Fable to write this version as though we're *not* releasing additional artifacts.
If and when we release artifacts, we'll strategically insert a few footnotes where needed.
}

{\color{red}AX: As currently written, I think the current section will be hard to track for anyone *not* intimately involved in the paper.
Granted, this is hard because it is about exploring a lot of concepts ...
Is it possible to extract a general/high-level for a proof template/sketch/idea so that we can ``set the scene'' + provide context?
\\
Additionally, I think you could consider adding a brief ``Overview`` paragraph of sorts that someone *not* working on Grothendieck can easily skim and get the big picture. This could be a high-level summarization of the subsequent ``The plateau``, ``First intervention'', etc. paragraphs.
}

\paragraph{The plateau.}
The run began on the upper bound, searching the limiting-scheme space of our
preprint for schemes whose correlation function admits a large
inverse-majorant parameter $\gamma$, since an admissible $\gamma$ gives
$\KG\le\pi/(2\gamma)$. From the hyperplane value
$\gamma=\log(1+\sqrt2)\approx0.8814$ it reached $\gamma\approx0.882$, and
there it stalled: in sessions 12 through 17 it opened six {\color{red}mechanically
distinct escape routes}, and each failed against the same obstruction,
namely that cubic coefficient mass cannot be cancelled without also reducing
the linear coefficient. Each failure was recorded and tagged, and the run's
response was to begin a seventh variation of the same search.

\paragraph{First intervention: turn the failures into a theorem.}
The operator redirected the run in session 18. Instead of attempting another
escape, it was to synthesize the accumulated failures into a proof that no
scheme in the class does much better: a ceiling $\gamma\le\Gamma$ valid for
the full class, with mixtures and arbitrary dimension, converts through the
optimality theorem of Naor and Regev \cite{naor2014krivine} into the lower
bound $\KG\ge\pi/(2\Gamma)$. The intervention supplied no new mathematics:
the problem statement had suggested this dualization from the outset, and
the run had accumulated exactly the required evidence without making the
connection. Session 18 identified the Naor--Regev theorem as the correct
transfer, proved a first ingredient valid in every dimension, and located
the difficulty precisely: the ceilings it could prove covered too narrow a
class of schemes.

\paragraph{Progress in two dimensions.}
Within days the run had proved a cubic ceiling of strength
$\Gamma\approx0.8866$ for two-dimensional schemes, with the {\color{red}keystone (?)}
inequality certified in interval arithmetic, and had sharpened the
constant numerically to $\Gamma\approx0.8846$. The extension to arbitrary dimension and to mixtures, which the
duality requires, did not follow: fourteen sessions in the range 32--51
attacked it, each reducing the gap to a sub-lemma, proving the sub-lemma in
a restricted setting, and leaving the global assembly open, while the
restricted results accumulated in memory as apparent progress. Two useful
facts emerged alongside this loop: the run verified the normalization of the
Naor--Regev transfer against the original paper, and it computed that
improving the Davie--Reeds~\cite{Davie1984LowerBoundKG,Reeds1991LowerBoundKG} bound $1.6769566742$ requires a universal ceiling
only at $\Gamma\le0.93669$, far above the two-dimensional value, so a
general ceiling could be far from sharp and still give a new lower bound.

\paragraph{Second intervention: the general bound, through theory.}
The operator ended this loop with a second redirection, on two grounds:
refinements of the two-dimensional result were not the object of interest,
since only a ceiling for the full class dualizes; and the gap was
conceptual, so further implementation would not close it. The run was to
spend several sessions on theory alone. Session 55 mapped the dependency
structure of the preceding weeks and identified the recurring error,
restricted closures recorded as global progress. Session 56 then produced
the {\color{red}decisive (?)} reframe. Every failed transport had been nonlinear in
quantities that do not average when schemes are mixed; the Hermite
coefficients $(b_1,b_3)$ of the correlation function, by contrast, are
linear functionals of the scheme, so a constraint that is affine in
$(b_1,b_3)$ passes to mixtures and to coefficientwise limits with no further
argument. Choosing the constraint for transportability, and requiring
equality at the extremal hyperplane point $(b_1,b_3)=(1,\tfrac16)$, gives
the one-parameter family of affine constraints
\[
        b_3\;\ge\;(1+\lambda)\,b_1-\Bigl(\lambda+\tfrac56\Bigr),
        \qquad \lambda\ge\tfrac12 ,
\]
where $\lambda$ indexes the slope of the line through the hyperplane point.
Each member forces a barrier $\Gamma_\lambda=(\lambda+\frac56)/(1+\lambda)$
on the admissible parameter, hence a bound $\KG\ge\pi/(2\Gamma_\lambda)$
conditional on proving that member, and every $\Gamma_\lambda$ below
$0.93669$ improves on Davie--Reeds.

\paragraph{Third intervention: one certified {\color{red}rung} before a better one.}
The tangent member $\lambda=\tfrac12$, worth $\KG\ge9\pi/16\approx1.767$,
requires a sharp chaos inequality that remains open, and once the family
existed the run's inclination was to work toward its strongest provable
member. The operator set the priority differently: what mattered was to
establish that the method yields any new lower bound at all, so the run was
to select a rung whose proof closes, certify it completely, and write it up,
with improvements inside the family treated as secondary. At $\lambda=1$ the
proof collapses to elementary structure: session 57 found that the
decomposition $h=(f+g)/2$, $k=(f-g)/2$ reduces the constraint, fiber by
one-dimensional fiber, to the ternary inequality~\eqref{eq:fiber-inequality},
%% TODO: fix cross-reference to the fiber inequality of the lower-bound section
whose closing case analysis is short, giving $\Gamma_1=\tfrac{11}{12}$ and
\[
        \KG\;\ge\;\frac{6\pi}{11}\;\approx\;1.7136 .
\]
Sessions 58--64 then subjected the chain to adversarial review, which
found and repaired the one substantive gap (the passage from finitely many
schemes to measurable mixtures, closed by a weak-$*$ lemma), a Jensen
inequality applied in the wrong direction, and a small defect in the
interval certificate's coverage, after which the run produced the first
complete write-up, about a day after the reframe. The stronger rungs
$27\pi/49$ and $51\pi/92$ of Table~\ref{tab:timeline} followed within a week
by the same method at smaller values of $\lambda$.



\paragraph{Attribution.}
The operator contributed no proof step anywhere in the chain. The operator's
contributions were the starting context of
Section~\ref{sec:ai-methodology} and the three interventions above, each a
redirection of effort rather than a piece of mathematics. The system
contributed the mathematics: the identification and verification of the
transfer theorem, the headroom computation, the two-dimensional ceiling, the
observation that affine constraints survive mixing, the family of lines, the
fiber reduction, the closure lemma, the certificates, and the initial
write-up. One further observation matters for what follows: nothing in the
session-56 reframe depended on information unavailable at the pivot a week
earlier, since the affineness of coefficients under mixing is elementary and
the headroom computation is one line. The binding constraint appears to have
been the system's disposition to continue its current program, not a missing
capability.
{\color{red} Name this something like ``human involvement'' or somehting along those lines. Also move the operator contributions first, and describe why they were necessary. Only then do you state the AI involvement.}


\subsection{Discussion}
\label{sec:ai-discussion}

The record supports a consistent capability profile: strong technical
execution, with persistent failures in the judgement that directs it. We
summarize the strengths, then the weaknesses, stated in the terms that the
interventions of Section~\ref{sec:ai-case-study} make concrete, and close
with what the record shows about the division of labor.

\subsubsection{Strengths}

Three strengths carried the run. The first is technical range with effective
recall: given a one-word pointer to Naor's work, the system identified the
relevant theorem, verified its normalization against the paper, and computed
the slack available for a lossy transfer; given a plateau, it produced six
structurally distinct escape mechanisms in two days. The second is local
invention: the affine family, the fiber reduction, the closure lemma, and
the certificate architecture were machine products, several arriving within
hours once the question was well posed. The third is speed and reliability
of execution: from the reframe to a machine-audited, interval-certified
proof took about a day, and most individual technical errors were caught by
the system's own verification passes. In one representative episode
(sessions p44 and p49), a claimed bound of $\KG\ge1.7754518$
was refuted within five hours by an adversarial session that computed its
true margin to be approximately $-8\times10^{-8}$, and the record was
corrected to the defensible value.

\subsubsection{Weaknesses}

Each intervention of Section~\ref{sec:ai-case-study} was needed because a
specific capability was absent. The paragraphs below name these
capabilities and add further instances from the record.

{\color{red}
AX: Name these paragraphs more explicitly to reflect a negative,
e.g., "Poor judgment of what is interesting", "Lack of high-level research skills", etc.}

\paragraph{Judgement of interestingness.}
The system did not reliably rank work by mathematical interest. The second
and third interventions are the clearest cases: the run treated refinements
of the two-dimensional ceiling as progress when only the general bound
mattered, and, once the family of rungs existed, it valued improvements
within the family over establishing the first certified rung. The same
tendency appeared at smaller scales throughout, from sessions spent on
$10^{-5}$-sized improvements to mechanisms the run already understood, down
to reported values tuned to the edges of their enclosures. The implication
for collaboration is that the objective of the research cannot yet be
delegated. The operator's judgements of interest were few, but each
redirected weeks of machine effort, and between them the system optimized,
competently, whatever was in front of it. On a problem of this size the
space of possible intermediate constructions is unbounded, and a ranking by
expected interest is what makes the search tractable; supplying that
ranking was the human's principal ongoing contribution.

\paragraph{Research skills.}
The system managed individual arguments well and the research process
poorly: it did not decide when to persist, when to switch, or what a
sequence of failures implied. The first intervention is the sharpest case,
since the dualization of failures into a lower bound was suggested in the
problem statement the system re-read at every session, the six failures
were in its memory, and the step was taken only when ordered. The record
contains three further episodes of the same shape, of fourteen, roughly two
dozen, and about a dozen sessions respectively (the two-dimensional
extension, near-sharp variants of the lower bound, and the July
certification effort), in each of which the run circled a target without
progress until the operator ended the loop. The implication is that
autonomous running time does not by itself convert into progress. Once the
accessible directions were exhausted, additional sessions multiplied
execution, not judgement, and the run's rate of real progress was set by
the frequency of strategic correction; additional compute would not have
changed it. Oversight of such systems is accordingly most valuable at the
level of strategy, which is precisely the level at which the system did not
correct itself.

\paragraph{Memory.}
The harness's file-based memory preserved statements more reliably than
their qualifications. The withdrawn upper bound of Table~\ref{tab:timeline}
is the clearest case. In session 44 the run recorded a numerical upper
bound of $1.7802243$, with caveats attached; over the nineteen days the
value stood in working memory, re-summarization detached the caveats from
the headline number, and a note defending the value was written three days
before the internal audit that refuted it, finding the score inflated by a
finite truncation window and the underlying correlation profile
infeasible. A related failure occurred inside verification, where a
dedicated replay of the $51\pi/92$ certificate (session p95) passed it
because the replay inherited the framing of the argument it was checking;
the invalidating error was found the same day by a session that rebuilt the
argument from scratch (session p102). We attribute both failures to scale.
The run produced hundreds of sessions and tens of millions of tokens of
intermediate mathematics, and each new session could be shown only a small
distillate of it. What to retain, at what resolution, and with which
qualifications attached was itself decided by the models, through repeated
summarization, and repeated summarization is exactly where caveats detach
and inherited framings go unquestioned. Unlike the previous two weaknesses,
this one looks amenable to engineering: memory for such systems plausibly
needs more structure than prose summaries provide, for instance a graph of
claims carrying provenance and qualifications, so that important
information remains retrievable without being repeatedly re-serialized
through a model's context window.

\paragraph{Origins of the weaknesses.}
We believe these gaps have a common origin in how current systems are
produced. Models are trained and evaluated on problems selected for being
small enough to pose, sandbox, and score, and nothing in that regime
exercises the allocation of weeks of effort across an open-ended search.
The corpus they learn mathematics from is, moreover, made of finished
mathematics: the literature records definitions, theorems, and polished
proofs, while the process that produced them, the dead ends, the decisions
to abandon or reframe, the judgement of what was worth attempting, is
largely absent from the written record. A system trained this way can be
expected to acquire technique and the form of finished mathematics while
remaining weak at exactly the process skills described above, and that is
what we observe.

\subsubsection{Division of labor}

{\color{red}Name this subsection like human operator involvement or something, to emphasize the human involvement first.}

A useful summary of the collaboration is obtained by counting who caught
which errors. Errors in individual claims, such as wrong constants, broken
certificates, and invalid steps, were caught almost entirely by the system
itself. Failure patterns spanning many sessions, such as the three circling
episodes and the detachment of caveats from claims, were caught by the
operator in every recorded instance and by the system in none. The system
reliably falsifies a claim once the claim is specified; deciding which
claims to distrust remained a human function throughout. Consistent with
this, the operator's leverage came less from mathematical suggestions, most
of which the system correctly tested and discarded, than from calibration:
setting targets, ending loops, and auditing the run's own reporting. We also
note a regularity with design consequences: every overclaiming incident in
the record sits at a target with nearly zero margin, whereas the results
that survived verification all carry slack. This suggests that systems of
this kind are most productive when aimed at robust targets, with sharp
constants attempted only from a secured base.

\subsection{Future directions}
\label{sec:ai-future}

\paragraph{Mathematics.}
The immediate items are the machine-verified claims of
Table~\ref{tab:timeline}: human verification of the two certified upper
bounds and of the lower bounds $27\pi/49$ and $51\pi/92$ would upgrade each
to a theorem. Beyond them, the run's internal analysis identifies the
tangent case $\lambda=\tfrac12$ of the affine family, equivalent to a sharp
degree-three chaos inequality, as the natural boundary of the method and
worth $\KG\ge9\pi/16$ if resolved.
{\color{red}AX: If you're brave, conjecture that \(K_G = \sqrt{\pi}\)}

\paragraph{Toward AI systems for long-horizon research.}
If the diagnosis of Section~\ref{sec:ai-discussion} is right, the
requirements for progress follow from it. First, mathematical
interestingness needs to become an object of study in its own right: the
judgement that selects which questions, intermediate constructions, and
targets are worth pursuing was the most consequential input the human
supplied, and there is at present no training signal or benchmark that
rewards it. Second, the process of research mathematics needs data. What
mathematicians actually do between problem statement and finished paper,
how they allocate effort, learn from repeated failure, and decide to
reframe, is barely recorded anywhere; records of long runs such as ours,
which preserve every step including the unsuccessful ones, are one way to
begin creating such data, and we release ours in that spirit. Third,
evaluation must move to horizons where these capabilities matter, treating
a weeks-long research program rather than a single problem as the unit of
assessment, with memory and calibration measured alongside correctness.
These conclusions carry the usual caution that they derive from one run on
one problem; replications on other open problems, successful or not, would
be the most useful follow-up work.

\paragraph{Human--AI collaboration.}
The run also suggests where collaboration of this kind is heading. Within
it, the contributions that required a human were not technical: the system
supplied the arguments, the computations, the certificates, and the first
write-up, while the human supplied the problem, the taste, and the
strategic corrections. If the technical abilities of these systems continue
to improve, this division will sharpen, and the mathematician's role in
such collaborations will concentrate into choosing what to work on, judging
which objects and targets matter, and deciding what to trust: directing
research that one does not personally execute. A similar shift is already
under way in software engineering. We expect working modes of this kind to
become common in mathematics, and the run documented here, with its
weaknesses as much as its results, is an early picture of what they will
require of the mathematician.

\subsection*{Statement on AI use}
{\color{red}AX: Any specific reason for an entire subsection instead of just a paragraph?}

Large language models were used extensively in the research reported in
this paper, in the roles described in this section: GPT-5.5-Pro and
GPT-5.6-Sol (OpenAI) as the reasoning model, and Claude Opus and Claude
Fable~5 (Anthropic) as the coding agent. AI assistance was also used in
preparing parts of this manuscript. All results stated as theorems have been
verified by the authors independently of these systems, and the account of
the run given in this section reflects the authors' own reading of the
record. The authors take full responsibility for the contents of this
paper.



==> old/asymptotic_scheme_old.tex <==
\section{The Asymptotic Family}
\label{sec:scheme}

This section implements Section~\ref{sec:scheme} of the proof architecture.  There is one minor change in convention from this section onwards to keep in mind: any partition $F$ defined below corresponds to the partition $x\mapsto F(\sqrt2 x)$ in Definition~\ref{def:gaussian-correlation-function}.  This change of variables is harmless and keeps the Hermite covariance identity in its usual probabilist normalization.

\subsection{Hermite notation}

\begin{definition}[Orthonormal probabilist Hermite polynomials]\label{def:Hermite}
Let $(\He_n)_{n\ge0}$ denote the orthonormal probabilist Hermite polynomials.  Thus, for $Z\sim N(0,1)$,
\[
  \E[\He_m(Z)\He_n(Z)]=\delta_{mn}.
\]
In particular,
\[
  \He_0=1,
  \qquad \He_1(x)=x,
  \qquad \He_3(x)={x^3-3x\over\sqrt6},
  \qquad \He_5(x)={x^5-10x^3+15x\over\sqrt{120}}.
\]
If $(X,Y)$ are standard Gaussians with correlation $t$, then
\begin{equation}\label{eq:hermite-cov}
  \E[\He_m(X)\He_n(Y)]=\delta_{mn}t^n.
\end{equation}
We use this as our normalization throughout the coefficient computation.  Standard references for these identities include~\cite[Sec.~6.1]{AAR99}.
\end{definition}

\begin{definition}[Gaussianized Hermite-chaos average]\label{def:gaussianized-chaos}
Fix an odd integer $d\ge3$.  A length-$N$ \emph{Gaussianized degree-$d$ Hermite-chaos average} is the random variable
\[
  P_{d,N}=N^{-1/2}\sum_{j=1}^N \He_d(U_{d,j}),
\]
where the $U_{d,j}$ are independent standard Gaussians.  The word ``Gaussianized'' refers to the fact that, for fixed $d$, the variable $P_{d,N}$ converges in distribution to a Gaussian as $N\to\infty$, while paired copies retain the covariance power of the degree-$d$ Wiener chaos.  Specifically, if $(U_{d,j},U_{d,j}')$ are paired with correlation $t$, then \eqref{eq:hermite-cov} gives
\[
  \E[P_{d,N}P_{d,N}']=t^d.
\]
For background on Hermite polynomials and Wiener chaos, see Janson's book on Gaussian Hilbert spaces~\cite{Janson1997GaussianHilbertSpaces}.
\end{definition}

\subsection{Finite-dimensional schemes}\label{subsec:finite-schemes}

\begin{definition}[Finite Hermite-average family]\label{def:finite-family}
Let $D\subseteq\{3,5,7,9,\ldots\}$ be a finite set of odd degrees.  For each $d\in D$, fix a real weight $s_d$, and define the relative sign
\[
  \sigma_d=(-1)^{(d-1)/2}.
\]
% Thus $\sigma_3=-1$, $\sigma_5=+1$, $\sigma_7=-1$, and so on.

For length $N$, let
\[
  P_{d,N}=N^{-1/2}\sum_{j=1}^N \He_d(U_{d,j}),
\]
where all variables $Z,X,U_{d,j}$ are independent standard Gaussians.  The finite rounding functions are
\begin{align}
  f_N&=\sgn\biggl(Z+\eta \He_3(X)+\sum_{d\in D}s_dP_{d,N}\biggr),\label{eq:finite-f-general}\\
  g_N&=\sgn\biggl(Z-\eta \He_3(X)+\sum_{d\in D}\sigma_d s_dP_{d,N}\biggr).\label{eq:finite-g-general}
\end{align}
They are odd measurable functions on $\R^{2+|D|N}$.  
% The value of $\sgn(0)$ is immaterial, since every threshold event has probability zero.
\end{definition}

\begin{definition}[The third/fifth finite scheme]\label{def:finite-35}
The scheme used for the numerical certificate is the specialization of Definition~\ref{def:finite-family} with $D=\{3,5\}$ and
\begin{equation}\label{eq:params}
  \eta=0.136419125,
  \qquad
  s_3=0.34101124,
  \qquad
  s_5=0.05276111.
\end{equation}
Equivalently,
\begin{align}
  f_N&=\sgn\bigl(Z+\eta \He_3(X)+s_3P_{3,N}+s_5P_{5,N}\bigr),\label{eq:finite-f-35}\\
  g_N&=\sgn\bigl(Z-\eta \He_3(X)-s_3P_{3,N}+s_5P_{5,N}\bigr).\label{eq:finite-g-35}
\end{align}
Thus degree $3$ is anti-aligned between the two sides, while degree $5$ is aligned.
\end{definition}

\subsection{The limiting model}\label{subsec:limiting-model}

\begin{definition}[Limiting model]\label{def:limiting-model}
Let $D,\eta,(s_d)_{d\in D}$ be as in Definition~\ref{def:finite-family}.  Let $R_d$, $d\in D$, be independent standard Gaussians.  The limiting threshold pair is
\begin{align}
  f(z,x,(r_d))&=\sgn\biggl(z+\eta \He_3(x)+\sum_{d\in D}s_dr_d\biggr),\label{eq:lim-f-general}\\
  g(z,x,(r_d))&=\sgn\biggl(z-\eta \He_3(x)+\sum_{d\in D}\sigma_d s_dr_d\biggr).\label{eq:lim-g-general}
\end{align}
For the limiting correlation at parameter $t$, the paired coordinates satisfy
\[
  \rho_Z=t,
  \qquad \rho_X=t,
  \qquad \rho_d=t^d\quad(d\in D),
\]
and different coordinate pairs are independent.  The arcsine-normalized limiting correlation is
\begin{equation}\label{eq:lim-H}
  H(t)={\pi\over2}\E\bigl[f(Z,X,(R_d))g(Z',X',(R_d'))\bigr].
\end{equation}
\end{definition}

Because all degrees in the model are odd, $H$ is an odd function.  For $D=\{3,5\}$, Definition~\ref{def:limiting-model} implies that the extra coordinates have correlations $t^3$ and $t^5$, which come from the finite Hermite averages through \eqref{eq:hermite-cov}.


==> old/certification.tex <==
\section{New Certification Section}

Write
\[
H(t)
=
b_1t
+
\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}} b_m t^m,
\qquad
B_3^2
:=
\sum_{\substack{m\ge 1\\ m\ \mathrm{odd}}} m^6 b_m^2.
\]
The certificate reduces to a single comparison between the linear
coefficient and the total nonlinear coefficient mass.

\begin{proposition}[Head--tail inverse certificate]
\label{prop:head-tail-certificate}
Let \(N\) be odd. If
\begin{equation}
\gamma
+
\sum_{\substack{3\le m\le N\\m\ \mathrm{odd}}}|b_m|
+
\frac{B_3}{\sqrt{10N^5}}
<
b_1,
\label{eq:head-tail-condition}
\end{equation}
then the local inverse
\[
G(z)=H^{-1}(z)=\sum_{n\ge1}a_nz^n
\]
extends holomorphically to a neighborhood of
\(\gamma\overline{\mathbb D}\), maps this neighborhood into
\(\mathbb D\) after shrinking it if necessary, and satisfies
\[
\sum_{n\ge1}|a_n|\gamma^n<1.
\]
\end{proposition}

\begin{proof}
By Cauchy--Schwarz,
\[
\sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
\le
B_3
\left(
\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
\right)^{1/2}.
\]
Since \(N\) is odd and \(x\mapsto x^{-6}\) is decreasing,
\[
\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
\le
\frac12\int_N^\infty x^{-6}\,dx
=
\frac{1}{10N^5}.
\]
Consequently, if
\[
\eta:=\sum_{m\ge3}|b_m|,
\]
then \eqref{eq:head-tail-condition} implies
\[
\gamma+\eta<b_1.
\]

Set
\[
\widehat E(u):=\sum_{m\ge3}|b_m|u^m.
\]
Let
\[
G(z)=\sum_{n\ge1}a_nz^n
\]
be the formal inverse of \(H\), and let
\[
V(z)=\sum_{n\ge1}v_nz^n
\]
be the unique formal power series with nonnegative coefficients
satisfying
\[
b_1V(z)=z+\widehat E(V(z)).
\]
Comparing coefficients in
\[
b_1G(z)=z-E(G(z))
\]
and inducting on the degree gives
\[
|a_n|\le v_n
\qquad (n\ge1).
\]

Equivalently, \(V\) is obtained coefficientwise from the Picard
iteration
\[
V_0(z)=0,
\qquad
V_{k+1}(z)
=
\frac{z+\widehat E(V_k(z))}{b_1}.
\]
Put
\[
q:=\frac{\gamma+\eta}{b_1}<1.
\]
If \(V_k(\gamma)\le1\), then
\[
V_{k+1}(\gamma)
\le
\frac{\gamma+\widehat E(1)}{b_1}
=
q.
\]
Thus the iterates are bounded by \(q\), and monotone convergence gives
\[
\sum_{n\ge1}|a_n|\gamma^n
\le
V(\gamma)
\le q
<1.
\]

Since the inequality \(\gamma+\eta<b_1\) is strict, it remains true
with \(\gamma\) replaced by some
\(\widetilde\gamma>\gamma\). Repeating the argument at
\(\widetilde\gamma\) shows that \(G\) converges absolutely there and
satisfies
\[
\sup_{|z|\le\widetilde\gamma}|G(z)|<1.
\]
The formal identity \(H(G(z))=z\) therefore holds analytically on
\(\widetilde\gamma\mathbb D\), proving the claimed extension and
mapping property.
\end{proof}

\begin{proposition}[Certified numerical data]
\label{prop:certified-data}
For the cubic--quintic scheme and \(N=251\), interval arithmetic
certifies
\[
b_1\ge 0.881573822049,
\]
\[
\sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
\le 1.1328860\cdot10^{-5},
\]
and
\[
B_3\le36.
\]
\end{proposition}

\begin{proof}
The coefficient-head computation and the certified Sobolev estimate
are proved in Appendix~\ref{app:numerical-certificate}.
\end{proof}

We now take
\[
\gamma=0.881545409.
\]
Proposition~\ref{prop:certified-data} gives
\[
\gamma
+
\sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
+
\frac{B_3}{\sqrt{10\cdot251^5}}
\le
0.881568143462
<
0.881573822049
\le b_1.
\]
Hence Proposition~\ref{prop:head-tail-certificate} gives
\[
\sum_{n\ge1}|a_n|\gamma^n<1.
\]
The finite-dimensional transfer theorem and the classical Krivine
criterion therefore imply
\[
K_G
\le
\frac{\pi}{2\gamma}
\le
1.7818666069360661.
\]




\section{Certification}
\label{sec:certification}

This section contains the complete limiting certificate and the final proof of Theorem~\ref{thm:main}.  The analytic estimates are grouped with the interval-arithmetic quantities that certify them: the Wiener-algebra inverse criterion, the Sobolev tail bound, the bound on the Sobolev norm, the assembly of the numerical inequalities, the formal finite-dimensional proof, and the computational formulas used by the certificate.


\subsection{A Wiener-algebra certificate for the limiting inverse}\label{sec:wiener}

This subsection implements the inverse-majorant step of the proof architecture.  The point is that the nonlinear part of $H$ is small in the Wiener algebra, so the inverse majorant can be certified without computing a long inverse series.

\begin{definition}[Wiener-algebra data]\label{def:wiener-data}
Let $\calA$ be the Wiener algebra of absolutely convergent power series on the unit disk:
\[
  U(w)=\sum_{n\ge0}u_nw^n,
  \qquad
  \|U\|_1=\sum_{n\ge0}|u_n|<\infty.
\]
Then $\|UV\|_1\le\|U\|_1\|V\|_1$.  Write
\begin{equation}\label{eq:H-linear-nonlinear}
  H(t)=b_1t+E(t),
  \qquad
  E(t)=\sum_{m\ge3}b_mt^m,
\end{equation}
and define
\begin{equation}\label{eq:eta0eta1}
  \eta_0=\sum_{m\ge3}|b_m|,
  \qquad
  \eta_1=\sum_{m\ge3}m|b_m|.
\end{equation}
\end{definition}

On the unit ball of $\calA$, the nonlinear part is $\eta_1$-Lipschitz:
\begin{equation}\label{eq:E-lipschitz-simple}
  \|E(U)-E(V)\|_1\le \eta_1\|U-V\|_1,
  \qquad \|U\|_1,\|V\|_1\le1.
\end{equation}
This follows from $\|U^m-V^m\|_1\le m\|U-V\|_1$ on the unit ball.

\begin{theorem}[Wiener contraction certificate]\label{thm:simple-wiener}
Assume
\begin{equation}\label{eq:simple-wiener-cond}
  \eta_1<b_1,
  \qquad
  \gamma+\eta_0<b_1.
\end{equation}
Then $H^{-1}$ is holomorphic on the disk of radius $\gamma$ and
\[
  \sum_{n\ge1}|A_n|\gamma^n<1,
  \qquad H^{-1}(\zeta)=\sum_{n\ge1}A_n\zeta^n.
\]
Moreover the inverse branch is holomorphic on a neighborhood of $\gamma\overline\D$, and it maps $\gamma\D$ into $\D$.
\end{theorem}

\begin{proof}
We first construct the inverse branch as a fixed point in the Wiener algebra, rather than assuming it exists.  The equation $H(U)=\gamma w$ is equivalent, as an identity in $\calA$, to
\[
  U=\Phi(U):={\gamma w-E(U)\over b_1}.
\]
Consider the closed unit ball
\[
  \calB=\{U\in\calA: U(0)=0,\ \|U\|_1\le1\}.
\]
If $U\in\calB$, then
\[
  \|E(U)\|_1\le\sum_{m\ge3}|b_m|\|U\|_1^m\le\eta_0,
\]
so
\[
  \|\Phi(U)\|_1\le{\gamma+\eta_0\over b_1}<1.
\]
For $U,V\in\calB$, \eqref{eq:E-lipschitz-simple} gives
\[
  \|\Phi(U)-\Phi(V)\|_1\le{\eta_1\over b_1}\|U-V\|_1.
\]
Thus $\Phi$ is a contraction from $\calB$ to itself.  Let $U$ be its unique fixed point.  Then $H(U(w))=\gamma w$ as a power-series identity in $\calA$, and
\[
  \|U\|_1=\sum_{n\ge1}|A_n|\gamma^n\le {\gamma+\eta_0\over b_1}<1.
\]

It remains to record the analytic room needed for the finite-dimensional transfer and to identify the fixed point with a holomorphic inverse branch.  Put $q=\|U\|_1<1$, and choose $q<q_*<1$.  For $u,v\in q_*\overline\D$,
\[
  |H(u)-H(v)|\ge b_1|u-v|-\sum_{m\ge3}|b_m||u^m-v^m|
  \ge \left(b_1-\sum_{m\ge3}m|b_m|q_*^{m-1}\right)|u-v|
  \ge (b_1-\eta_1)|u-v|.
\]
Hence $H$ is injective on $q_*\D$ and $H'$ has no zero there.  Since $U(\overline\D)\subset q\overline\D\subset q_*\D$, the compact set $\gamma\overline\D=H(U(\overline\D))$ lies in the open set $H(q_*\D)$, on which the inverse branch is holomorphic.  In particular, it is holomorphic on a neighborhood of $\gamma\overline\D$; after shrinking this neighborhood to a slightly larger disk if necessary, it has the form required for the finite-dimensional transfer theorem.
\end{proof}



\subsection{The coefficient tail through a Sobolev norm}\label{sec:sobolev-tail}

This subsection controls the tail of the original correlation series $H$, not the tail of the inverse series.  The advantage is that the coefficients $b_m$ are signed and have substantial cancellation; the Sobolev norm below sees this cancellation.

Let
\[
  \Dop=t{d\over dt}
\]
be the Euler operator, so that $\Dop t^m=mt^m$.  For the odd series $H(t)=\sum_{m\ \mathrm{odd}}b_mt^m$, define
\begin{equation}\label{eq:B-s}
  B_s^2=\sum_{\substack{m\ge1\\m\ \mathrm{odd}}}m^{2s}b_m^2
  ={1\over2\pi}\int_0^{2\pi}\left|\Dop^sH(e^{i\theta})\right|^2\,d\theta.
\end{equation}
The equality is Parseval on the unit circle.

\begin{lemma}[Sobolev tail]\label{lem:sobolev-tail}
Let $N$ be odd.  Then
\[
  \sum_{m>N}|b_m|\le B_3\left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2},
\]
and
\[
  \sum_{m>N}m|b_m|\le B_3\left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-4}\right)^{1/2}.
\]
\end{lemma}

\begin{proof}
Write $|b_m|=m^{-3}\cdot m^3|b_m|$ and $m|b_m|=m^{-2}\cdot m^3|b_m|$, then apply Cauchy-Schwarz and use $\sum_{m>N}m^6b_m^2\le B_3^2$.
\end{proof}

The power-sum factors are tiny.  With $N=251$,
\begin{equation}\label{eq:tail-factors}
  \left(\sum_{\substack{m>251\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}\le3.13677\cdot10^{-7},
  \qquad
  \left(\sum_{\substack{m>251\\m\ \mathrm{odd}}}m^{-4}\right)^{1/2}\le1.020511\cdot10^{-4}.
\end{equation}
Each odd power sum is enclosed by a finite head plus a decreasing-integral remainder.  Thus even a crude bound on $B_3$ suffices.



\subsection{Bounding the Sobolev norm}\label{sec:sobolev-norm}

By \eqref{eq:B-s}, it is enough to bound $\Dop^3H(e^{i\theta})$ on the circle.  We realize $\Dop^3H$ as a trace of a two-dimensional differential kernel and apply an averaged inequality.


\subsubsection{A combined kernel}

For real $|r|<1$, let $\Kr_r$ be the centered bivariate Gaussian density of correlation $r$,
\begin{equation}\label{eq:Kr-kernel}
  \Kr_r(u,v)={1\over2\pi\sqrt{1-r^2}}
  \exp\left(-{u^2-2ruv+v^2\over2(1-r^2)}\right).
\end{equation}
We use the same formula by analytic continuation for the complex values $r=\rho(e^{i\theta})$ that occur below; on this compact curve $1-r^2$ is bounded away from zero, and the square-root branch is fixed continuously from $r=0$.  Set $h(x)=\He_3(x)$ and let $\vartheta=\eta/\sqrt V$ be as in Definition~\ref{def:collapsed-data}.  For fixed real $x,y$, define the threshold-covariance kernel
\begin{equation}\label{eq:threshold-cov-kernel}
  \mathcal C_r(x,y)
  ={\pi\over2}\,\E\bigl[\sgn(W+\vartheta h(x))\sgn(W'+\vartheta h(y))\bigr],
\end{equation}
where $(W,W')$ is a centered standard Gaussian pair of correlation $r$.  Equivalently, for $|r|<1$,
\begin{equation}\label{eq:C-Hermite-expansion}
  \mathcal C_r(x,y)
  ={\pi\over2}\sum_{a\ge0}r^a q_a(\vartheta h(x))q_a(\vartheta h(y)),
\end{equation}
with $q_a$ as in Definition~\ref{def:qk}.  This formula gives the analytic continuation in $r$ used in the differentiated kernels.

The two first derivative identities are
\begin{equation}\label{eq:C-first-derivatives}
  \partial_r\mathcal C_r(x,y)=2\pi\Kr_r(\vartheta h(x),\vartheta h(y)),
  \qquad
  \partial_x\partial_y\mathcal C_r(x,y)
  =2\pi\vartheta^2h'(x)h'(y)\Kr_r(\vartheta h(x),\vartheta h(y)).
\end{equation}
Indeed, the first identity is Price's theorem in the $W,W'$ variables, or follows by differentiating \eqref{eq:C-Hermite-expansion} and using the Mehler expansion of $\Kr_r$.  For the second, one uses $q_a'(u)=2\varphi(u)\He_a(-u)$ and then the same Mehler expansion.  Thus after one correlation derivative every kernel is a polynomial differential operator applied to $\Kr_r$; no discontinuous sign kernel remains.

We next define the boundary trace in the $x,y$ variables.  Let $\mu$ be the product standard Gaussian measure on $\R^2$.  If a kernel $\Psi$ satisfies $\Psi,\partial_x\partial_y\Psi\in L^2(\mu)$, write its Hermite coefficients as
\[
  \widehat\Psi_{i,j}=\iint_{\R^2}\Psi(x,y)\He_i(x)\He_j(y)\,d\mu(x,y).
\]
For $|\lambda|\le1$ set
\begin{equation}\label{eq:Tlambda-definition}
  T_\lambda[\Psi]
  =\widehat\Psi_{0,0}+\sum_{n\ge1}\lambda^n\widehat\Psi_{n,n}.
\end{equation}
For $|\lambda|<1$, this is exactly the correlated Gaussian expectation $\E[\Psi(X,Y)]$ with $\operatorname{corr}(X,Y)=\lambda$.  For $|\lambda|=1$, \eqref{eq:Tlambda-definition} is the Sobolev boundary trace of that expectation.

The series in \eqref{eq:Tlambda-definition} converges absolutely on $|\lambda|=1$.  Moreover
\begin{equation}\label{eq:Tlambda-bound}
  |T_\lambda[\Psi]|
  \le {\pi\over\sqrt6}
  \left(\|\Psi\|_{L^2(\mu)}^2+4\|\partial_x\partial_y\Psi\|_{L^2(\mu)}^2\right)^{1/2}.
\end{equation}
To see this, note that
\[
  |\widehat\Psi_{0,0}|\le\|\Psi\|_{L^2(\mu)}
\]
and, since the coefficient of $\He_{n-1}(x)\He_{n-1}(y)$ in $\partial_x\partial_y\Psi$ is $n\widehat\Psi_{n,n}$,
\[
  \sum_{n\ge1}|\widehat\Psi_{n,n}|
  \le\left(\sum_{n\ge1}{1\over n^2}\right)^{1/2}
      \left(\sum_{n\ge1}n^2|\widehat\Psi_{n,n}|^2\right)^{1/2}
  \le {\pi\over\sqrt6}\|\partial_x\partial_y\Psi\|_{L^2(\mu)}.
\]
The displayed estimate follows from the elementary inequality
\[
  A+{\pi\over\sqrt6}B
  \le {\pi\over\sqrt6}\sqrt{A^2+4B^2}\qquad(A,B\ge0),
\]
using $\pi^2/6>4/3$.

With $\lambda=-t$ and $\Dop_t=t\partial_t$, define recursively
\begin{equation}\label{eq:Phi-recursion}
  \Phi_0(t;x,y)=\mathcal C_{\rho(t)}(x,y),
  \qquad
  \Phi_{k+1}=\Dop_t\Phi_k+\lambda\,\partial_x\partial_y\Phi_k\quad(k\ge0),
\end{equation}
where $\rho$ is the polynomial in \eqref{eq:rho-collapsed}.  Here $\Dop_t$ differentiates all explicit $t$-dependence of $\Phi_k$, including the dependence through $\rho(t)$ and through scalar prefactors created at earlier steps.  The combined kernel $\Phi_3$ is obtained by carrying out this recursion before any norm is taken.  By \eqref{eq:C-first-derivatives}, $\Phi_3$ is a finite sum of smooth $\Kr_r$-derivative kernels.

\begin{lemma}[Trace representation]\label{lem:trace-rep}
For $|t|=1$,
\[
  \Dop^3H(t)=T_{-t}\bigl[\Phi_3(t;\cdot,\cdot)\bigr],
\]
and $T_{-t}$ satisfies the bound \eqref{eq:Tlambda-bound}.
\end{lemma}

\begin{proof}
First assume $|t|<1$, and put $\lambda(t)=-t$.  The collapsed representation of Proposition~\ref{prop:collapsed-coefficients} is equivalently
\begin{equation}\label{eq:H-as-trace-C}
  H(t)=T_{\lambda(t)}\bigl[\mathcal C_{\rho(t)}\bigr].
\end{equation}
Indeed, for $|\lambda|<1$, the trace is the correlated expectation in the $X,Y$ variables, and \eqref{eq:threshold-cov-kernel} is precisely the conditional $W,W'$ expectation multiplied by the normalizing factor $\pi/2$.

We use the following differentiation identity.  If $\Psi(t)$ is a smooth family of kernels with enough decay, then
\begin{equation}\label{eq:trace-differentiation}
  \Dop_t\,T_{\lambda(t)}[\Psi(t)]
  =T_{\lambda(t)}\bigl[\Dop_t\Psi(t)+\lambda(t)\partial_x\partial_y\Psi(t)\bigr].
\end{equation}
For $|\lambda|<1$ this is Price's theorem in the outer Gaussian variables.  Equivalently, it follows directly from the Hermite definition of $T_\lambda$: differentiating
\[
  T_{\lambda(t)}[\Psi(t)]
  =\sum_{n\ge0}\lambda(t)^n\widehat\Psi_{n,n}(t)
\]
gives the term $\sum_n\lambda^n\Dop_t\widehat\Psi_{n,n}$ plus
\[
  \sum_{n\ge1} n\lambda^n\widehat\Psi_{n,n}
  =\lambda\sum_{m\ge0}(m+1)\lambda^m\widehat\Psi_{m+1,m+1},
\]
and the latter is $\lambda T_\lambda[\partial_x\partial_y\Psi]$ because
\[
  \partial_x\partial_y\Psi
  =\sum_{i,j\ge1}\sqrt{ij}\,\widehat\Psi_{i,j}\He_{i-1}(x)\He_{j-1}(y)
  \quad\text{in the Hermite sense.}
\]

Starting from \eqref{eq:H-as-trace-C} and applying \eqref{eq:trace-differentiation} three times gives
\[
  \Dop^3H(t)=T_{\lambda(t)}[\Phi_3(t;\cdot,\cdot)]
  \qquad(|t|<1),
\]
with $\Phi_k$ exactly as in \eqref{eq:Phi-recursion}.  The identities \eqref{eq:C-first-derivatives} show that every term in $\Phi_3$ is a smooth kernel of the form used in Subsection~\ref{sec:formulas}; in particular $\Phi_3$ and $\partial_x\partial_y\Phi_3$ lie in $L^2(\mu)$ uniformly for radial limits $t=re^{i\theta}$, $0<r\le1$.

Letting $r\uparrow1$ in the identity for $re^{i\theta}$ gives the asserted boundary identity for $|t|=1$, with $\Dop^3H(e^{i\theta})$ understood as the radial boundary value.  The right-hand side has this limit because $\Phi_3$ is an explicit finite sum of the smooth kernels listed in Subsection~\ref{sec:formulas}, and because $T_\lambda$ is continuous for the Sobolev trace norm appearing in \eqref{eq:Tlambda-bound}.  Finally, the bound for $T_{-t}$ is \eqref{eq:Tlambda-bound}.
\end{proof}

The recursion \eqref{eq:Phi-recursion} expands $\Phi_3$ as a finite sum over a nine-term index set; the explicit prefactors and kernels are recorded in Subsection~\ref{sec:formulas}.

\subsubsection{An averaged Minkowski bound}

From Lemma~\ref{lem:trace-rep} and \eqref{eq:B-s},
\begin{equation}\label{eq:B3-avg}
  B_3^2={1\over2\pi}\int_0^{2\pi}|\Dop^3H(e^{i\theta})|^2\,d\theta
  \le {\pi^2\over6}\,\overline S,
\end{equation}
where
\[
  \overline S={1\over2\pi}\int_0^{2\pi}S(\theta)\,d\theta,
  \qquad
  S(\theta)=\|\Phi_3\|_{L^2(\mu)}^2+4\|\partial_x\partial_y\Phi_3\|_{L^2(\mu)}^2,
\]
and $\Phi_3$ is taken at $t=e^{i\theta}$.

\begin{lemma}[Averaged Minkowski]\label{lem:averaged-minkowski}
Write $\Phi_3=\sum_{p,a}c_{p,a}(t)G_{p,a}$ for the expansion produced by \eqref{eq:Phi-recursion}, with scalar prefactors $c_{p,a}$ and kernels $G_{p,a}$ as in Subsection~\ref{sec:formulas}.  For each pair set
\[
  Q^{(0)}_{p,a}={1\over2\pi}\int_0^{2\pi}|c_{p,a}(e^{i\theta})|^2\|G_{p,a}\|_{L^2(\mu)}^2\,d\theta,
\]
and
\[
  Q^{(1)}_{p,a}={1\over2\pi}\int_0^{2\pi}|c_{p,a}(e^{i\theta})|^2\|\partial_x\partial_yG_{p,a}\|_{L^2(\mu)}^2\,d\theta.
\]
Then
\begin{equation}\label{eq:S-minkowski}
  \overline S\le
  \left(\sum_{p,a}\sqrt{Q^{(0)}_{p,a}}\right)^2
  +4\left(\sum_{p,a}\sqrt{Q^{(1)}_{p,a}}\right)^2.
\end{equation}
\end{lemma}

\begin{proof}
By the triangle inequality in $L^2(\mu)$,
\[
  \|\Phi_3\|_{L^2(\mu)}\le\sum_{p,a}|c_{p,a}|\|G_{p,a}\|_{L^2(\mu)}
\]
pointwise in $\theta$, and likewise for $\partial_x\partial_y\Phi_3$.  Taking the $L^2(d\theta/2\pi)$ norm of each sum and applying the triangle inequality there gives the two terms in \eqref{eq:S-minkowski}.
\end{proof}

Each $G_{p,a}$ is, on the real axis, a polynomial times a super-Gaussian, so the $L^2(\mu)$ norms are two-dimensional Gaussian integrals.  We enclose these integrals and then enclose the circle averages $Q^{(\cdot)}_{p,a}$ by a composite Gauss-Legendre rule with a certified remainder, as described in Subsection~\ref{sec:formulas}.

\begin{lemma}[Certified Sobolev bound]\label{lem:B3-certified}
The interval computation gives
\[
  \overline S\le1803.317.
\]
Consequently,
\[
  B_3\le{\pi\over\sqrt6}\sqrt{1803.317}\le54.4641.
\]
\end{lemma}

The per-pair contributions, certified through the quadrature, are listed in Table~\ref{tab:Q}.  The bound $54.4641$ is intentionally generous; it is already far more than enough because of the small tail factors in \eqref{eq:tail-factors}.

\begin{table}[t]\centering
\small
\begin{tabular}{c r r}
\toprule
$(p,a)$ & $\sqrt{Q^{(0)}_{p,a}}$ & $\sqrt{Q^{(1)}_{p,a}}$ \\
\midrule
$(0,1)$ & $0.04286765$ & $0.10127946$ \\
$(0,2)$ & $0.30383835$ & $1.10543141$ \\
$(0,3)$ & $0.36847714$ & $7.40413211$ \\
$(1,0)$ & $2.67546361$ & $0.10772752$ \\
$(1,1)$ & $0.19214422$ & $0.85400602$ \\
$(1,2)$ & $0.51708607$ & $6.83760791$ \\
$(2,0)$ & $2.30597621$ & $0.29542681$ \\
$(2,1)$ & $0.41663640$ & $3.10773691$ \\
$(3,0)$ & $2.36356861$ & $0.91665956$ \\
\bottomrule
\end{tabular}
\caption{Certified upper bounds for the per-pair quantities of Lemma~\ref{lem:averaged-minkowski}; substituting into \eqref{eq:S-minkowski} gives $\overline S\le1803.317$.}
\label{tab:Q}
\end{table}



\subsection{Assembling the certificate}\label{sec:assembly}

This subsection combines the certified coefficient head, the Sobolev tail, and the Wiener-algebra criterion.  The cutoff is $N=251$.

\begin{lemma}[Certified coefficient head]\label{lem:certified-head}
Using the coefficient formula of Proposition~\ref{prop:collapsed-coefficients} and the interval enclosures described in Subsection~\ref{sec:formulas}, the first coefficients are certified with
\[
  b_1\ge0.881573822049,
  \qquad
  b_3\approx3.4538733\cdot10^{-9},
  \qquad
  b_5\approx-9.0435536\cdot10^{-11}.
\]
Here ``$\approx$'' means that the displayed decimal lies in the corresponding outward-rounded interval enclosure.
Moreover the partial sums through degree $251$ satisfy
\begin{equation}\label{eq:certified-head-sums}
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|\le1.1328860\cdot10^{-5},
  \qquad
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}m|b_m|\le1.5737642\cdot10^{-4}.
\end{equation}
\end{lemma}

The near-vanishing of $b_3$ and $b_5$ is the design goal.  If
\[
  H(t)=b_1t+b_3t^3+b_5t^5+\cdots,
  \qquad
  H^{-1}(\zeta)=A_1\zeta+A_3\zeta^3+A_5\zeta^5+\cdots,
\]
then formal series reversion gives
\begin{equation}\label{eq:low-inverse}
  A_1={1\over b_1},
  \qquad
  A_3=-{b_3\over b_1^4},
  \qquad
  A_5={3b_3^2-b_1b_5\over b_1^7}.
\end{equation}
Thus making $b_3$ and $b_5$ small makes the first two nonlinear inverse coefficients small.

\begin{proposition}[Limiting admissibility]\label{prop:limiting-admissibility}
For $\gamma=0.881545409$, the limiting third/fifth model satisfies
\[
  \sum_{n\ge1}|A_n|\gamma^n<1,
  \qquad H^{-1}(\zeta)=\sum_{n\ge1}A_n\zeta^n.
\]
The inverse branch is holomorphic on a neighborhood of $\gamma\overline\D$ and maps $\gamma\D$ into $\D$.
\end{proposition}

\begin{proof}
By Lemmas~\ref{lem:sobolev-tail} and~\ref{lem:B3-certified}, together with \eqref{eq:tail-factors},
\[
  \sum_{m>251}|b_m|
  \le 54.4641\cdot3.13677\cdot10^{-7},
\]
and
\[
  \sum_{m>251}m|b_m|
  \le 54.4641\cdot1.020511\cdot10^{-4}.
\]
Combining these inequalities with \eqref{eq:certified-head-sums},
\[
  \eta_0=\sum_{m\ge3}|b_m|
  \le1.1328860\cdot10^{-5}+54.4641\cdot3.13677\cdot10^{-7}
  \le2.84130\cdot10^{-5},
\]
and
\[
  \eta_1=\sum_{m\ge3}m|b_m|
  \le1.5737642\cdot10^{-4}+54.4641\cdot1.020511\cdot10^{-4}
  \le5.71550\cdot10^{-3}.
\]
With $b_1\ge0.881573822049$, we have $\eta_1<b_1$ and
\[
  \gamma+\eta_0\le0.881573821996<0.881573822049\le b_1.
\]
Theorem~\ref{thm:simple-wiener} applies and proves the claim.
\end{proof}

\subsection{Formal proof of Theorem~\ref{thm:main}}\label{subsec:formal-proof-main}

\begin{proof}[Proof of Theorem~\ref{thm:main}]
By Proposition~\ref{prop:limiting-admissibility}, the limiting model satisfies a strict inverse-majorant certificate at $\gamma=0.881545409$, with inverse branch holomorphic on a neighborhood of $\gamma\overline\D$ and with values in $\D$ on a slightly larger closed disk around $\gamma\overline\D$.  Corollary~\ref{cor:finite-scheme} transfers this certificate to all sufficiently high finite-dimensional third/fifth Gaussianized-chaos schemes \eqref{eq:finite-f-35}--\eqref{eq:finite-g-35}.  Applying the Krivine criterion, Lemma~\ref{lem:local-inverse-expansion} or equivalently Theorem~\ref{thm:krivine-criterion}, to such a finite scheme gives
\[
  \KG\le {\pi\over2\gamma}\le1.7818666069360661.
\]
Since
\[
  {\pi\over 2\log(1+\sqrt2)}-{\pi\over2\gamma}
  =3.473712553\cdot10^{-4}\ldots,
\]
the hyperplane-improvement form follows.
\end{proof}



\subsection{Computational formulas}\label{sec:formulas}

This subsection lists the explicit objects used in the interval certificate.  All real inputs are decimal intervals and all derived quantities are outward-rounded Arb balls.

\paragraph{Parameters.}
The parameters are $\eta,s_3,s_5$ from \eqref{eq:params}.  We set
\[
  V=1+s_3^2+s_5^2,
  \qquad
  \vartheta={\eta\over\sqrt V},
  \qquad
  \rho(t)={t-s_3^2t^3+s_5^2t^5\over V}.
\]

\paragraph{Coefficient integrals.}
The collapsed coefficients are
\[
  \mathsf A_{a,b}=\int_\R \He_b(x)q_a(\vartheta\He_3(x))\varphi(x)\,dx,
\]
where $q_a$ is given by Lemma~\ref{lem:qk}.  The integrand is entire.  For $a\ge1$ it contains the extra factor $e^{-(\vartheta\He_3(x))^2/2}$ and is super-Gaussian on the real axis; for $a=0$ it has the ordinary Gaussian tail from $\varphi(x)$.  It is enclosed by Arb's adaptive integrator on a finite interval $[-L,L]$, plus a closed Gaussian-tail bound outside the interval using $|q_a|\le1$.  The coefficient $b_m$ is then the interval sum \eqref{eq:bm-collapsed}, with $[t^{m-b}]\rho(t)^a$ computed by a finite convolution of $(1,-s_3^2,s_5^2)/V$.  Absolute values in $\eta_0$ and $\eta_1$ are taken on enclosures bounded away from zero.

\paragraph{Combined kernel.}
The recursion \eqref{eq:Phi-recursion} produces
\[
  \Phi_3=\sum_{(p,a)}c_{p,a}(t)G_{p,a}
\]
over the nine pairs in Table~\ref{tab:Q}.  The scalar prefactors $c_{p,a}(t)$ are polynomials in $t$, generated from the formal seed $c_{0,0}=1$ for the threshold-covariance kernel $\mathcal C_{\rho(t)}$ by applying three times the substitutions
\[
  c_{p,a}\longmapsto \Dop_tc_{p,a}\quad\text{at the same }(p,a),
\]
\[
  c_{p,a}\longmapsto (\Dop_t\rho)c_{p,a}\quad\text{at }(p+1,a),
  \qquad
  c_{p,a}\longmapsto (-t)c_{p,a}\quad\text{at }(p,a+1).
\]
The first time a substitution moves from the formal seed to either $(p+1,a)$ or $(p,a+1)$, the identities \eqref{eq:C-first-derivatives} supply the displayed $2\pi$ factors.  The kernels are, with $\varphi_r=\Kr_r$ from \eqref{eq:Kr-kernel} evaluated at $u=\vartheta h(x)$, $v=\vartheta h(y)$, and $r=\rho(t)$,
\[
  G_{p,0}=2\pi\,\partial_r^{p-1}\varphi_r\quad(p\ge1),
\]
and
\[
  G_{p,a}=\partial_x^{a-1}\partial_y^{a-1}
  \left(2\pi\vartheta^2h'(x)h'(y)\partial_r^p\varphi_r\right)
  \quad(a\ge1).
\]
Each derivative $\partial_r^p\partial_x^i\partial_y^j\varphi_r$ equals a polynomial in $(r,u,v,1-r^2)$ times $\varphi_r$, with integer coefficients computed by a fixed operator recurrence.

\paragraph{Gaussian norms.}
Writing $u=\vartheta h(x)$, the squared modulus of a kernel against $\mu$ is
\[
  \|G_{p,a}\|_{L^2(\mu)}^2=
  \iint_{\R^2}|G_{p,a}(x,y)|^2{e^{-(x^2+y^2)/2}\over2\pi}\,dx\,dy.
\]
This is a positive integral of a polynomial times $e^{-x^2/2-y^2/2}$ and the bounded factor
\[
  \exp\left(-A\vartheta^2(h(x)^2+h(y)^2)+2B\vartheta^2h(x)h(y)\right),
\]
where
\[
  A=\Re(1/d),\qquad B=\Re(r/d),\qquad d=1-r^2.
\]
Using the identity $x^3=\sqrt6\,h(x)+3x$, every mode reduces to a combination of one-dimensional base moments
\[
  I_{\varepsilon,q}(A)=\E\bigl[X^\varepsilon h(X)^q e^{-A\vartheta^2h(X)^2}\bigr],
  \qquad \varepsilon\in\{0,1,2\},
\]
each enclosed by Arb's integrator; the cross term is expanded in a convergent series with a Chernoff tail.

\paragraph{Circle quadrature and its remainder.}
The averages $Q^{(\cdot)}_{p,a}$ are computed by a composite four-point Gauss-Legendre rule on $[0,2\pi]$ with $M$ panels of the certified point values $|c_{p,a}|^2\|G_{p,a}\|^2$.  For an integrand $g(\theta)$, the rule's error is at most
\[
  C_4(2\pi)^8M^{-9}\sum_jD_{8,j},
  \qquad
  C_4={(4!)^4\over9(8!)^3},
\]
where each panel bound $D_{8,j}\ge\sup_{I_j}|g^{(8)}|$ is obtained without cancellation from
\[
  |g^{(8)}|\le\sum_{j=0}^{8}\binom8j\sqrt{V_jV_{8-j}},
  \qquad
  V_j(\theta)=\|\partial_\theta^j(c_{p,a}G_{p,a})\|_{L^2(\mu)}^2.
\]
The estimate
\[
  V_j\le |d|^{-1}\left(\sum_\nu |p_{j,\nu}(\theta)|\sqrt{L_\nu L_{\nu'}}\right)^2
\]
uses $2|B|\,|UV|\le |B|(U^2+V^2)$ to absorb the mixed term in the exponent, giving the residual decay
\[
  -A(U^2+V^2)+2BUV\le -(A-|B|)(U^2+V^2).
\]
The required positivity margin
\[
  A-|B|=\Re(1/d)-|\Re(r/d)|\ge {1\over2}
\]
on the unit circle is verified on all panels.  Here $L_\nu$ are precomputed positive one-dimensional integrals and $|p_{j,\nu}|$ are bounded by evaluating the $\theta$-derivative coefficients on each panel as intervals.  At $M=2048$ the total remainder is at most $9.1\cdot10^{-4}$ per pair, negligible compared with the final value of $\overline S$.



\subsection{Implementation notes}\label{sec:impl}

The following comments are not needed for the logical proof, but they explain why the certificate is organized in the form used above.

\begin{enumerate}[label=\textbf{I\arabic*.},leftmargin=*]
\item \textbf{Why real-axis integration.}  The integrand of a Gaussian norm decays like $e^{-c x^6}$ on the real axis but can grow like $e^{c|z|^6}$ off the real axis, because $\He_3(z)^2\sim z^6/6$ has negative real part in some complex sectors.  Interval boxes in $(x,y)$, or a complex contour, see this far-field growth and produce much worse bounds.  The certificate therefore evaluates every integral at real points; Arb's adaptive integrator is effective because the local error model only probes small neighborhoods of the real subintervals.

\item \textbf{Why the Sobolev tail.}  Bounding $\sum|b_m|$ through $B_3=\|\Dop^3H\|_{L^2(\T)}$ keeps the cancellation in the signed coefficients $b_m$.  A direct Hermite-mass bound, or a complex Cauchy estimate of $H^{-1}$ near $t=1$, overshoots by many orders of magnitude.

\item \textbf{Why the combined kernel.}  Forming $\Phi_3$ by the recursion \eqref{eq:Phi-recursion} before taking norms is essential.  Expanding $\Dop^3H$ as a sum of separately bounded terms discards a nine-fold cancellation and gives a much looser estimate.

\item \textbf{Why the cancellation-free eighth-derivative bound.}  The exact eighth $\theta$-derivative of the quadrature integrand is a signed combination of inner products whose terms can be enormous near $\theta=0$ and $\theta=\pi$ before cancellation.  The Minkowski bound in Subsection~\ref{sec:formulas} avoids this signed sum entirely: every $V_a$ is a positive quantity, at the cost of a looser derivative bound that is absorbed by the $M^{-9}$ factor in the quadrature remainder.

\item \textbf{Precision.}  The base moments require higher precision for large powers and for circle nodes near $\theta=0,\pi$.  The reported headline inequalities are stable under further refinement of precision and panel count.
\end{enumerate}


==> old/certification_new.tex <==
\section{Certification}
\label{sec:certification}

Write the correlation function of the cubic--quintic limiting scheme as
\begin{equation}
  H(t)=b_1t+\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}} b_m t^m,
  \label{eq:certification-H-series}
\end{equation}
and let
\begin{equation}
  \Delta_H:=\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}}|b_m|
  \label{eq:nonlinear-coefficient-mass}
\end{equation}
be the total mass of its nonlinear coefficients.  Let
\[
  G(z)=H^{-1}(z)=\sum_{n\ge1}a_nz^n
\]
denote the local holomorphic inverse of $H$ at the origin, and define its
majorant by
\begin{equation}
  \mathcal M(r):=\sum_{n\ge1}|a_n|r^n.
  \label{eq:inverse-majorant-certification}
\end{equation}
The local inverse exists because $H'(0)=b_1>0$, by the holomorphic inverse
function theorem.

For the linear map $t\mapsto b_1t$, the condition $\mathcal M(\gamma)<1$ is
simply $\gamma<b_1$.  The next proposition shows that the nonlinear part costs
at most $\Delta_H$ of this margin.

\begin{proposition}[Inverse certificate from near-linearity]
\label{prop:inverse-certificate-near-linearity}
Assume $b_1>0$ and $\Delta_H<\infty$.  If
\begin{equation}
  \gamma+\Delta_H<b_1,
  \label{eq:near-linearity-condition}
\end{equation}
then there exists $R>\gamma$ such that the local inverse $G$ extends
holomorphically to $R\mathbb D$, maps $R\mathbb D$ into $\mathbb D$, and
satisfies
\begin{equation}
  \mathcal M(\gamma)
  \le \frac{\gamma+\Delta_H}{b_1}
  <1.
  \label{eq:near-linearity-conclusion}
\end{equation}
\end{proposition}

\begin{proof}
Set
\[
  E(t):=\sum_{m\ge3}b_mt^m,
  \qquad
  E_{\mathrm{maj}}(u):=\sum_{m\ge3}|b_m|u^m.
\]
There is a unique formal power series
\[
  V(z)=\sum_{n\ge1}v_nz^n
\]
satisfying
\begin{equation}
  b_1V(z)=z+E_{\mathrm{maj}}(V(z)).
  \label{eq:majorizing-inverse-equation}
\end{equation}
Indeed, comparison of the coefficient of $z$ gives $v_1=b_1^{-1}$.  For
$n\ge2$, the coefficient of $z^n$ in $E_{\mathrm{maj}}(V)$ depends only on
$v_1,\ldots,v_{n-1}$, so \eqref{eq:majorizing-inverse-equation} determines
$v_n$ recursively.  The same recursion shows that $v_n\ge0$ for every $n$.

Comparing coefficients in
\[
  b_1G(z)=z-E(G(z))
\]
and in \eqref{eq:majorizing-inverse-equation}, induction on $n$ gives
\begin{equation}
  |a_n|\le v_n
  \qquad(n\ge1).
  \label{eq:inverse-coefficient-domination}
\end{equation}
Indeed, at degree $n$, every nonlinear composition involves only previously
determined coefficients, and replacing each $b_m$ by $|b_m|$ removes all
possible cancellation.

Choose $R>\gamma$ so close to $\gamma$ that
\[
  q:=\frac{R+\Delta_H}{b_1}<1.
\]
Starting from $V_0(z)=0$, define
\begin{equation}
  V_{k+1}(z):=\frac{z+E_{\mathrm{maj}}(V_k(z))}{b_1}.
  \label{eq:majorizing-inverse-iteration}
\end{equation}
The series $V_k$ have nonnegative coefficients and increase coefficientwise,
meaning that each Taylor coefficient is nondecreasing in $k$.
Moreover, if $V_k(R)\le q$, then $V_k(R)<1$ and
\[
  V_{k+1}(R)
  \le \frac{R+E_{\mathrm{maj}}(1)}{b_1}
  =q.
\]
Thus $V_k(R)\le q$ for every $k$.  Their coefficientwise limit satisfies
\eqref{eq:majorizing-inverse-equation}, and hence equals $V$ by uniqueness.
The monotone convergence theorem now gives
\[
  V(R)=\sum_{n\ge1}v_nR^n\le q<1.
\]
Together with \eqref{eq:inverse-coefficient-domination}, this implies
\[
  \sum_{n\ge1}|a_n|R^n\le V(R)<1.
\]
Consequently, the Taylor series of $G$ converges on $R\mathbb D$ and takes
values in $\mathbb D$.  Since the identity $H(G(z))=z$ holds near the origin,
it holds throughout $R\mathbb D$ by the identity theorem.  Finally,
\[
  \mathcal M(\gamma)
  \le V(\gamma)
  =\frac{\gamma+E_{\mathrm{maj}}(V(\gamma))}{b_1}
  \le\frac{\gamma+\Delta_H}{b_1},
\]
because $0\le V(\gamma)\le V(R)<1$.
\end{proof}

It remains to certify $\Delta_H$.  We compute the coefficients through a
finite degree $N$ and bound the remaining tail indirectly.  The point is that
the Euler operator
\[
  D:=t\frac{d}{dt}
\]
multiplies the coefficient of $t^m$ by $m$, so $D^3$ strongly amplifies
high-degree coefficients.  The $L^2(\mathbb T)$ norm below is the
root-mean-square size of the resulting function around the unit circle
$\mathbb T:=\{z\in\mathbb C:|z|=1\}$.

\begin{lemma}[Third-order coefficient-tail bound]
\label{lem:third-order-tail}
Suppose that $D^3H$ has radial boundary values in $L^2(\mathbb T)$, with
\[
  \|D^3H\|_{L^2(\mathbb T)}^2
  :=\frac{1}{2\pi}\int_0^{2\pi}
  |D^3H(e^{i\theta})|^2\,d\theta.
\]
Then, for every odd $N$,
\begin{equation}
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
  \le
  \|D^3H\|_{L^2(\mathbb T)}
  \left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}
  \le
  \frac{\|D^3H\|_{L^2(\mathbb T)}}{\sqrt{10N^5}}.
  \label{eq:third-order-tail}
\end{equation}
\end{lemma}

\begin{proof}
Since $D^3(t^m)=m^3t^m$, Parseval's identity gives
\begin{equation}
  \|D^3H\|_{L^2(\mathbb T)}^2
  =\sum_{\substack{m\ge1\\m\ \mathrm{odd}}}m^6|b_m|^2.
  \label{eq:parseval-third-order}
\end{equation}
The Cauchy--Schwarz inequality therefore gives
\[
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
  =\sum_{\substack{m>N\\m\ \mathrm{odd}}}
  m^{-3}\bigl(m^3|b_m|\bigr)
  \le
  \left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}
  \|D^3H\|_{L^2(\mathbb T)}.
\]
Finally, since $x\mapsto x^{-6}$ is decreasing and consecutive odd integers
are separated by two, the monotone integral estimate gives
\[
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
  \le\frac12\int_N^\infty x^{-6}\,dx
  =\frac{1}{10N^5}.
\]
\end{proof}

\begin{proposition}[Certified numerical input]
\label{prop:certified-numerical-input}
For the cubic--quintic correlation function, interval arithmetic certifies
\begin{equation}
  b_1\ge0.881573822049,
  \qquad
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
  \le1.1328860\cdot10^{-5},
  \qquad
  \|D^3H\|_{L^2(\mathbb T)}<35.774<36.
  \label{eq:certified-numerical-input}
\end{equation}
\end{proposition}

\begin{proof}
See Appendix~\ref{app:certification-details}.
\end{proof}

Lemma~\ref{lem:third-order-tail} and
Proposition~\ref{prop:certified-numerical-input} give
\begin{equation}
  \Delta_H
  \le
  1.1328860\cdot10^{-5}
  +\frac{36}{\sqrt{10\cdot251^5}}
  <2.2734462\cdot10^{-5}.
  \label{eq:certified-nonlinear-mass}
\end{equation}

\begin{theorem}[Cubic--quintic upper bound]
\label{thm:cubic-quintic-upper-bound-certified}
For
\[
  \gamma=0.881545409,
\]
the cubic--quintic limiting scheme satisfies $\mathcal M(\gamma)<1$.
Consequently,
\begin{equation}
  K_G\le\frac{\pi}{2\gamma}
  \le1.7818666069360661.
  \label{eq:certified-KG-bound}
\end{equation}
\end{theorem}

\begin{proof}
By \eqref{eq:certified-nonlinear-mass},
\[
  \gamma+\Delta_H
  <0.881545409+2.2734462\cdot10^{-5}
  =0.881568143462
  <0.881573822049
  \le b_1.
\]
Proposition~\ref{prop:inverse-certificate-near-linearity} therefore gives
$\mathcal M(\gamma)<1$, together with the analytic room required by the
finite-dimensional transfer theorem.  That theorem passes the strict
certificate to all sufficiently large ordinary finite-dimensional
approximations.  The classical Krivine preprocessing theorem then gives
\eqref{eq:certified-KG-bound}.
\end{proof}


==> old/coefficient_formulas_old.tex <==
\section{Coefficient Formula for the Limiting Model}
\label{sec:coefficients}

This section implements the coefficient step in the proof architecture.  The point is to reduce the limiting threshold model, with the correlation powers defined in Definition~\ref{def:limiting-model}, to explicit two-dimensional Gaussian integrals.

\subsection{Degree-direction data}\label{subsec:degree-data}

\begin{definition}[Degree-direction normalization]\label{def:degree-normalization}
For a finite degree set $D$ and weights $(s_d)_{d\in D}$, define
\[
  S=\biggl(\sum_{d\in D}s_d^2\biggr)^{1/2},
  \qquad
  \alpha_d={s_d\over S}\quad(d\in D).
\]
Thus $\sum_{d\in D}\alpha_d^2=1$, and
\[
  \sum_{d\in D}s_dr_d=S\sum_{d\in D}\alpha_dr_d.
\]
\end{definition}

\begin{definition}[One-dimensional threshold coefficients]\label{def:qk}
Let $R\sim N(0,1)$.  For $u\in\R$ and $k\in\Nzero$, define
\[
  q_k(u)=\E_R[\sgn(u+R)\He_k(R)].
\]
These are the Hermite coefficients of the one-dimensional threshold $R\mapsto \sgn(u+R)$.
\end{definition}

\begin{lemma}[Closed form for $q_k$]\label{lem:qk}
For all $u\in\R$,
\begin{align}
  q_0(u)&=\erf\left({u\over\sqrt2}\right),\label{eq:q0}\\
  q_k(u)&=2\varphi(u){\He_{k-1}(-u)\over\sqrt{k}},\qquad k\ge1,\label{eq:qk}
\end{align}
where $\varphi(u)=(2\pi)^{-1/2}e^{-u^2/2}$.
\end{lemma}

\begin{proof}
For $k=0$,
\[
  q_0(u)=\Prob[R>-u]-\Prob[R<-u]=\erf\left({u\over\sqrt2}\right).
\]
For $k\ge1$, orthogonality to constants gives
\[
  q_k(u)=2\int_{-u}^{\infty}\He_k(r)\varphi(r)\,dr.
\]
The orthonormal Hermite polynomials satisfy
\[
  {d\over dr}\left(\varphi(r)\He_{k-1}(r)\right)
  =-\sqrt{k}\,\varphi(r)\He_k(r),
\]
so integration from $-u$ to $\infty$ gives \eqref{eq:qk}.
\end{proof}

\begin{definition}[Two-dimensional coefficient integrals]\label{def:Cabk}
For $a,b,k\in\Nzero$, define
\begin{equation}\label{eq:C-abk}
  C_{a,b,k}
  =\E_{Z,X}\left[\He_a(Z)\He_b(X)
    q_k\left({Z+\eta \He_3(X)\over S}\right)\right],
\end{equation}
where $Z,X$ are independent standard Gaussians.  Equivalently,
\[
  C_{a,b,k}=\int_{\R^2}\He_a(z)\He_b(x)
  q_k\left({z+\eta \He_3(x)\over S}\right)\varphi(z)\varphi(x)\,dz\,dx.
\]
\end{definition}

The quantities $C_{a,b,k}$ are the only continuous integrals appearing in the coefficient formula.  Everything else is finite bookkeeping by degree.

\subsection{Hermite coefficients of the limiting thresholds}\label{subsec:threshold-hermite-coefficients}

For a multi-index $\beta=(\beta_d)_{d\in D}\in\Nzero^D$, write
\[
  |\beta|=\sum_{d\in D}\beta_d,
  \qquad
  \beta!=\prod_{d\in D}\beta_d!,
  \qquad
  \alpha^\beta=\prod_{d\in D}\alpha_d^{\beta_d}.
\]

\begin{proposition}[Hermite coefficients of the limiting thresholds]\label{prop:hermite-coefficients}
Let $f,g$ be the limiting threshold functions in Definition~\ref{def:limiting-model}.  Write their Hermite expansions in the tensor basis as
\[
  f=\sum_{a,b,\beta} A_{a,b,\beta}\,\He_a(Z)\He_b(X)\prod_{d\in D}\He_{\beta_d}(R_d),
\]
\[
  g=\sum_{a,b,\beta} B_{a,b,\beta}\,\He_a(Z)\He_b(X)\prod_{d\in D}\He_{\beta_d}(R_d).
\]
Then, for $k=|\beta|$,
\begin{equation}\label{eq:f-coeff}
  A_{a,b,\beta}=C_{a,b,k}\sqrt{k!\over \beta!}\,\alpha^\beta,
\end{equation}
while
\begin{equation}\label{eq:g-coeff}
  B_{a,b,\beta}=(-1)^b\prod_{d\in D}\sigma_d^{\beta_d}\,A_{a,b,\beta}.
\end{equation}
\end{proposition}

\begin{proof}
Set
\[
  T(Z,X)=Z+\eta \He_3(X),
  \qquad
  R_\alpha=\sum_{d\in D}\alpha_dR_d.
\]
Then
\[
  f=\sgn(T+SR_\alpha).
\]
Conditioning on $Z,X$, the coefficient of $\He_k(R_\alpha)$ in the $R_\alpha$ direction is
\[
  q_k\left({T(Z,X)\over S}\right).
\]
Taking the additional inner product against $\He_a(Z)\He_b(X)$ gives $C_{a,b,k}$.

The multivariate Hermite addition formula gives
\begin{equation}\label{eq:hermite-addition}
  \He_k\left(\sum_{d\in D}\alpha_dR_d\right)
  =\sum_{\substack{\beta\in\Nzero^D\\ |\beta|=k}}
  \sqrt{k!\over \beta!}\,\alpha^\beta
  \prod_{d\in D}\He_{\beta_d}(R_d).
\end{equation}
Combining the previous paragraph with \eqref{eq:hermite-addition} proves \eqref{eq:f-coeff}.

Finally,
\[
  g(z,x,(r_d))=f(z,-x,(\sigma_dr_d)_{d\in D}).
\]
Since $\He_b(-x)=(-1)^b\He_b(x)$ and $\He_{\beta_d}(\sigma_dr_d)=\sigma_d^{\beta_d}\He_{\beta_d}(r_d)$, the coefficient relation \eqref{eq:g-coeff} follows.
\end{proof}

\subsection{The degree coefficient formula}\label{subsec:degree-formula}

\begin{theorem}[Coefficient formula]\label{thm:coefficient-formula}
Let
\[
  H(t)=\sum_{m\ge1}b_m t^m
\]
be the limiting normalized correlation \eqref{eq:lim-H}.  Then
\begin{equation}\label{eq:general-bm}
  b_m={\pi\over2}
  \sum_{\substack{a,b\in\Nzero,\ \beta\in\Nzero^D\\ a+b+\sum_{d\in D}d\beta_d=m}}
  (-1)^b\prod_{d\in D}\sigma_d^{\beta_d}
  {k!\over \beta!}
  \prod_{d\in D}\alpha_d^{2\beta_d}
  C_{a,b,k}^2,
  \qquad k=|\beta|.
\end{equation}
Only odd $m$ occur.
\end{theorem}

\begin{proof}
Under the correlation model in Definition~\ref{def:limiting-model}, the Hermite covariance identity \eqref{eq:hermite-cov} contributes
\[
  t^a t^b\prod_{d\in D}(t^d)^{\beta_d}
  =t^{a+b+\sum_d d\beta_d}
\]
to the tensor basis element indexed by $(a,b,\beta)$.  Multiplying the $f$- and $g$-coefficients from Proposition~\ref{prop:hermite-coefficients} and summing over all indices of degree $m$ gives \eqref{eq:general-bm}.

The functions $f$ and $g$ are odd under simultaneous negation of all coordinates.  Hence their Hermite coefficients vanish unless $a+b+|\beta|$ is odd.  Since all degrees $d\in D$ are odd, $a+b+\sum_d d\beta_d$ has the same parity as $a+b+|\beta|$.  Thus only odd degrees appear.
\end{proof}

\subsection{The third/fifth specialization}\label{subsec:third-fifth-coefficients}

\begin{definition}[Third/fifth coefficient data]\label{def:third-fifth-coeff-data}
For the scheme $D=\{3,5\}$, write
\[
  \alpha={s_3\over S},\qquad \beta={s_5\over S},
  \qquad S=(s_3^2+s_5^2)^{1/2}.
\]
With the numerical parameters \eqref{eq:params},
\[
  S=0.345068689589145\ldots,
  \quad
  \alpha=0.988241617650167\ldots,
  \quad
  \beta=0.152900311131734\ldots .
\]
\end{definition}

For $D=\{3,5\}$, Theorem~\ref{thm:coefficient-formula} becomes
\begin{equation}\label{eq:35-bm}
  b_m={\pi\over2}
  \sum_{\substack{a,b,\beta_3,\beta_5\in\Nzero\\ a+b+3\beta_3+5\beta_5=m}}
  (-1)^{b+\beta_3}
  {k!\over \beta_3!\beta_5!}
  \alpha^{2\beta_3}\beta^{2\beta_5}
  C_{a,b,k}^2,
  \qquad k=\beta_3+\beta_5.
\end{equation}
This is the general weighted-degree formula.  The certification below uses the equivalent collapsed formula in Proposition~\ref{prop:collapsed-coefficients}.


\subsection{A collapsed formula for the third/fifth certificate}\label{subsec:collapsed-formula}

The interval certificate uses the following specialized form of the third/fifth coefficient formula.  It is equivalent to \eqref{eq:35-bm}, but it combines the three Gaussian coordinates $Z,R_3,R_5$ into one Gaussian direction before expanding.  This reduces the coefficient computation to one-dimensional threshold integrals and is the form used in Sections~\ref{sec:assembly} and~\ref{sec:formulas}.

\begin{definition}[Collapsed third/fifth data]\label{def:collapsed-data}
For the parameters \eqref{eq:params}, set
\[
  V=1+s_3^2+s_5^2,
  \qquad
  \vartheta={\eta\over\sqrt V},
\]
and define
\[
  F(w,x)=\sgn\bigl(w+\vartheta\He_3(x)\bigr).
\]
For $a,b\ge0$, define
\begin{equation}\label{eq:mathsfAab}
  \mathsf A_{a,b}=\E_{W,X}\bigl[\He_a(W)\He_b(X)F(W,X)\bigr],
\end{equation}
where $W,X$ are independent standard Gaussians.  Finally set
\begin{equation}\label{eq:rho-collapsed}
  \rho(t)={t-s_3^2t^3+s_5^2t^5\over V}.
\end{equation}
\end{definition}

\begin{proposition}[Collapsed coefficient formula]\label{prop:collapsed-coefficients}
For the third/fifth limiting model,
\begin{equation}\label{eq:H-collapsed}
  H(t)={\pi\over2}\sum_{a,b\ge0}\mathsf A_{a,b}^2\rho(t)^a(-t)^b.
\end{equation}
Consequently, for every $m\ge1$,
\begin{equation}\label{eq:bm-collapsed}
  b_m={\pi\over2}\sum_{a,b\ge0}(-1)^b\mathsf A_{a,b}^2\,[t^{m-b}]\rho(t)^a.
\end{equation}
Only terms with $a+b$ odd contribute.
\end{proposition}

\begin{proof}
Set
\[
  W={Z+s_3R_3+s_5R_5\over\sqrt V},
  \qquad
  \widetilde W={Z'-s_3R_3'+s_5R_5'\over\sqrt V}.
\]
Then $W$ and $\widetilde W$ are standard Gaussians and
\[
  \mathrm{corr}(W,\widetilde W)={t-s_3^2t^3+s_5^2t^5\over V}=\rho(t).
\]
Moreover
\[
  f=F(W,X),
  \qquad
  g'=F(\widetilde W,-X'),
\]
because $\He_3(-X')=-\He_3(X')$.  Expand
\[
  F(W,X)=\sum_{a,b\ge0}\mathsf A_{a,b}\He_a(W)\He_b(X).
\]
The Hermite covariance identity gives
\[
  \E[\He_a(W)\He_a(\widetilde W)]=\rho(t)^a,
  \qquad
  \E[\He_b(X)\He_b(-X')]=(-1)^b t^b.
\]
Multiplying the matching Hermite coefficients and summing proves \eqref{eq:H-collapsed}.  Reading off coefficients gives \eqref{eq:bm-collapsed}.  The parity statement follows from $F(-w,-x)=-F(w,x)$, which forces $\mathsf A_{a,b}=0$ unless $a+b$ is odd.
\end{proof}

\begin{remark}[One-dimensional form of \texorpdfstring{$\mathsf A_{a,b}$}{Aab}]
The coefficient $\mathsf A_{a,b}$ can be written using the same threshold coefficients $q_a$ from Definition~\ref{def:qk}:
\[
  \mathsf A_{a,b}=\E_X\bigl[\He_b(X)q_a(\vartheta\He_3(X))\bigr].
\]
This is the formula used in the interval computation of the coefficient head.
\end{remark}


==> old/simplifications_old.tex <==
\section{Preliminaries}

We first state Vitali's theorem, which lets us convert pointwise convergence to uniform convergence. See~\cite{schiff1993normal} for a reference. 

\begin{fact}[Vitali's convergence theorem]
Let \(h_1,h_2,\ldots\) be holomorphic functions on a connected open set
\(\Omega\). Suppose that:
\begin{enumerate}
    \item the sequence \((h_N)_{N\geq 1}\) is locally bounded on \(\Omega\); and
    \item \(h_N(z)\) converges for every \(z\) in some subset of \(\Omega\)
    having an accumulation point in \(\Omega\).
\end{enumerate}
Then \((h_N)_{N\geq 1}\) converges locally uniformly on \(\Omega\) to a
holomorphic function.
\end{fact}


\section{Limiting Krivine Schemes}

In this section, we extend classical Krivine schemes by allowing them to have arbitrary correlations among variables (up to some criteria). We will show that we can state asymptotic statements about regular Krivine schemes using this extended class of schemes, that we call \textit{limiting Krivine schemes}. This gives us analytic machinery for searching and analyzing limits of high dimensional schemes that were previously inaccessible via standard techniques. It is first instructive for us to start with a motivating example. 

\paragraph{Motivating example.}
Consider the two-dimensional classical Krivine rounding scheme
\[
f(X_1,X_2)=\operatorname{sgn}(X_1+\lambda X_2),
\qquad
g(Y_1,Y_2)=\operatorname{sgn}(y_1+\lambda y_2),
\]
where \(X_1,X_2,Y_1,Y_2\) are standard Gaussians, \(X_1\) is independent of \(X_2\), \(Y_1\) is independent of \(Y_2\), and
\[
\operatorname{corr}(X_1,Y_1)
=
\operatorname{corr}(X_2,Y_2)
=
t.
\]
In a classical Krivine scheme, every pair of corresponding coordinates has correlation \(t\). Suppose instead that we would like the first pair to have correlation \(t\), but the second pair to have correlation \(t^3\). To obtain this from a classical high-dimensional scheme, define
\[
U_N=\frac{1}{\sqrt N}\sum_{j=1}^N \mathrm{He}_3(X_{2,j}),
\qquad
V_N=\frac{1}{\sqrt N}\sum_{j=1}^N \mathrm{He}_3(Y_{2,j}),
\]
where the pairs \((X_{2,j},Y_{2,j})\) are independent standard Gaussian pairs with correlation \(t\). The Hermite identity gives
\[
\mathbb{E}[U_NV_N]
=
\mathbb{E}[\mathrm{He}_3(X_{2,1})\mathrm{He}_3(Y_{2,1})]
=
t^3.
\]
Moreover, by the central limit theorem, \((U_N,V_N)\) converges in distribution to a standard Gaussian pair \((U,V)\) with correlation \(t^3\). Thus, the classical rounding schemes
\[
F_N=\operatorname{sgn}(X_1+\lambda U_N),
\qquad
G_N=\operatorname{sgn}(Y_1+\lambda V_N)
\]
converge to the fixed-dimensional Gaussian rounding scheme
\[
f(X_1,U)=\operatorname{sgn}(X_1+\lambda U),
\qquad
g(Y_1,V)=\operatorname{sgn}(Y_1+\lambda V),
\]
in which the two coordinate pairs have correlations \(t\) and \(t^3\), respectively.

To use this construction, we need to carefully handle the following analytic hurdles:
\begin{enumerate}
    \item Pointwise convergence of the correlation functions must be strengthened to locally uniform convergence;
    \item An inverse-majorant $\gamma$-admissibility proved for the limiting scheme must remain valid for all sufficiently large finite-dimensional approximations.
\end{enumerate}

We now generalize this construction and prove both properties. First, we define the notion of allowable correlation maps.  
\begin{definition}[Allowable correlation map]
\label{def:allowable-correlation-map}
A function \(\rho:(-1,1)\to\mathbb{R}\) is an \emph{allowable correlation map}
if it admits an expansion
\[
\rho(t)
=
\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}} c_d t^d,
\qquad
\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}}|c_d|
\leq 1.
\]
\end{definition}

We can now state the definition of limiting Krivine schemes. 

\begin{definition}[Limiting Krivine Schemes]
A $k$-dimensional \emph{limiting Krivine scheme} is a tuple $\mathcal{S} = (f, g, \rho)$, where  \(f,g:\mathbb{R}^k\to\{-1,1\}\) are odd measurable functions and \(\rho = (\rho_1,\ldots,\rho_k)\) is a tuple of allowable correlation maps.  

The arcsine-normalized correlation function of this scheme is given by 
\[
H_{f, g, \rho}(t)
=
\frac{\pi}{2}\mathbb{E}[f(X)g(Y)].
\]
where \(X,Y\in\mathbb{R}^k\) are jointly Gaussian such that
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t).
\]
\end{definition}

\begin{remark}
    This is a generalization of the usual high dimensional Krivine schemes with $\rho_i(t) = t$ for all $i$. 

    At this stage, \(H_{f, g, \rho}\) is defined only on \((-1,1)\); in particular, we do not assume that it extends holomorphically to the strip associated with classical Krivine schemes.
\end{remark}

The motivation for this definition is that every limiting Krivine scheme can be approximated arbitrarily well by ordinary finite-dimensional Krivine schemes, as we will show below. This allows us to use the usual projection scheme to round the vectors, and get the inverse-majorant machinery for free. We make this precise in the following theorem.  

\begin{theorem}[Finite-dimensional approximation of limiting schemes]
Let \(\mathcal S=(f,g,\rho_1,\ldots,\rho_k)\) be a limiting Krivine scheme. Then there exists a sequence of ordinary finite-dimensional Krivine schemes
\(
\mathcal S_1,\mathcal S_2,\ldots,
\)
of increasing dimension, whose correlation functions $H_{\mathcal S_1}, H_{\mathcal S_2}, \ldots$ converge to the correlation function $H_{\mathcal S}$ of \(\mathcal S\), uniformly on every compact subset of \((-1,1)\).
\end{theorem}

We dedicate the rest of the section to proving this theorem. First, we prove an equivalence condition on allowability of a function. 

\begin{lemma}[Allowable function criteria]
A map \(\rho\) is allowable if and only if there are odd functions
\(p,q: \R^3 \to \R\), such that
\(\|p\|_2=\|q\|_2=1\) and
\[
\rho(t)=\mathbb{E}[p(U)q(V)],
\]
where \(U,V\in\mathbb{R}^m\) are standard Gaussian vectors with
\(\mathbb{E}[U_iV_j]=t\delta_{ij}\).
\end{lemma}

\begin{proof}
Suppose first that \(p\) and \(q\) are odd and have \(L_2\)-norm one. Write
their Hermite expansions by degree as
\[
p=\sum_{\substack{d\geq 1\\ d\text{ odd}}}p_d,
\qquad
q=\sum_{\substack{d\geq 1\\ d\text{ odd}}}q_d.
\]
Here \(p_d\) and \(q_d\) are the degree-\(d\) Hermite components.

Different Hermite degrees are orthogonal, while degree \(d\) contributes a
factor \(t^d\). Hence
\[
\mathbb{E}[p(U)q(V)]
=
\sum_{\substack{d\geq 1\\ d\text{ odd}}}
\langle p_d,q_d\rangle t^d.
\]
Set \(c_d=\langle p_d,q_d\rangle\). Then
\[
\sum_d|c_d|
\leq
\sum_d\|p_d\|_2\|q_d\|_2
\leq
\left(\sum_d\|p_d\|_2^2\right)^{1/2}
\left(\sum_d\|q_d\|_2^2\right)^{1/2}
=
1.
\]
Thus the resulting correlation map is allowable.

Conversely, suppose that
\[
\rho(t)=\sum_{d\text{ odd}}c_dt^d,
\qquad
s:=\sum_{d\text{ odd}}|c_d|\leq 1.
\]
For \(x=(x_1,x_2,x_3)\in\mathbb{R}^3\), define
\[
p(x)
=
\sum_{d\text{ odd}}
\sqrt{|c_d|}\operatorname{He}_d(x_1)
+
\sqrt{1-s}\,x_2
\]
and
\[
q(x)
=
\sum_{d\text{ odd}}
\operatorname{sgn}(c_d)\sqrt{|c_d|}
\operatorname{He}_d(x_1)
+
\sqrt{1-s}\,x_3.
\]
Both functions are odd. Orthogonality gives \(\|p\|_2=\|q\|_2=1\).

Let \(U,V\in\mathbb{R}^3\) be standard Gaussian vectors with
\(\mathbb{E}[U_iV_j]=t\delta_{ij}\). The terms involving \(U_2\) and \(V_3\)
have zero cross-correlation. Therefore
\[
\mathbb{E}[p(U)q(V)]
=
\sum_{d\text{ odd}}c_dt^d
=
\rho(t).
\]
\end{proof}

We are now ready to prove our theorem, which follows as a direct corollary of the stronger statement we prove below. 

\begin{theorem}[Finite-dimensional approximation of limiting schemes]
Let \((f,g,\rho_1,\ldots,\rho_k)\) be a limiting Krivine scheme, and suppose
that the discontinuity sets of \(f\) and \(g\) have Gaussian measure zero.
Then its correlation function extends holomorphically to the unit disk and is
the locally uniform limit there of the correlation functions of ordinary
finite-dimensional Krivine schemes.
\end{theorem}

\begin{proof}
By the above lemma, for each \(i\in\{1,\ldots,k\}\), there exist odd measurable functions 
\(
p_i,q_i:\mathbb{R}^3\to\mathbb{R}
\)
with $\|p\|_2 = \|q\|_2 = 1$ such that, whenever \(U,V\in\mathbb{R}^3\) are joint standard Gaussian vectors with
\(
\mathbb{E}[U_aV_b]=t\delta_{ab},
\)
we have
\[
\mathbb{E}[p_i(U)q_i(V)]
=
\rho_i(t).
\]
We combine these functions into vector-valued maps. Write
\(u\in\mathbb{R}^{3k}\) in \(k\) blocks as
\[
u=\bigl(u^{(1)},\ldots,u^{(k)}\bigr),
\qquad
u^{(i)}\in\mathbb{R}^3,
\]
and define
\[
P(u)
=
\bigl(
p_1(u^{(1)}),\ldots,p_k(u^{(k)})
\bigr),
\]
\[
Q(u)
=
\bigl(
q_1(u^{(1)}),\ldots,q_k(u^{(k)})
\bigr).
\]
For each positive integer \(N\), define functions on
\(\bigl(\mathbb{R}^{3k}\bigr)^N\) by
\[
F_N(u_1,\ldots,u_N)
=
f\left(
\frac{1}{\sqrt{N}}\sum_{r=1}^N P(u_r)
\right)
\]
and
\[
G_N(v_1,\ldots,v_N)
=
g\left(
\frac{1}{\sqrt{N}}\sum_{r=1}^N Q(v_r)
\right).
\]
Since \(P\), \(Q\), \(f\), and \(g\) are odd, the functions \(F_N\) and
\(G_N\) are odd. They therefore define an ordinary finite-dimensional
Krivine scheme.

Let \(H_N\) denote the correlation function of this scheme. Fix
\(t\in(-1,1)\), and let
\[
(U_1,V_1),\ldots,(U_N,V_N)
\]
be independent pairs of standard Gaussian vectors in \(\mathbb{R}^{3k}\)
satisfying
\[
\mathbb{E}[(U_r)_a(V_r)_b]
=
t\delta_{ab}.
\]
Define
\[
A_N
=
\frac{1}{\sqrt{N}}\sum_{r=1}^N P(U_r),
\qquad
B_N
=
\frac{1}{\sqrt{N}}\sum_{r=1}^N Q(V_r).
\]
By the definition of the correlation function,
\[
H_N(t)
=
\frac{\pi}{2}\,
\mathbb{E}\bigl[f(A_N)g(B_N)\bigr].
\]

\begin{claim}
As \(N \rightarrow \infty\), we have \[
(A_N,B_N)
\xrightarrow{d}
(X,Y),
\]
where \((X,Y)\) is jointly Gaussian and satisfies
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t).
\]
\end{claim}

\begin{claimproof}
The random vectors
\[
\bigl(P(U_r),Q(V_r)\bigr)\in\mathbb{R}^{2k}
\]
are independent, identically distributed, and centered. Because the
\(k\) Gaussian blocks are independent, their covariance matrix is
\[
\begin{pmatrix}
I_k & D(t)\\
D(t) & I_k
\end{pmatrix},
\qquad
D(t)
=
\operatorname{diag}\bigl(
\rho_1(t),\ldots,\rho_k(t)
\bigr).
\]
By the multivariate central limit theorem, we have
\(
(A_N,B_N)
\xrightarrow[N\to\infty]{d}
(X,Y),
\)
where \((X,Y)\) is jointly Gaussian satisfying
\(
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij}\) and 
\(
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t),
\)
as desired. 
\end{claimproof}

Returning to the proof of the theorem, since the function
\(
(x,y)\longmapsto f(x)g(y)
\)
 is bounded and has discontinuity set with measure 0, it follows that
\[
\mathbb{E}\bigl[f(X_N)g(Y_N)\bigr]
\longrightarrow
\mathbb{E}\bigl[f(X(t))g(Y(t))\bigr].
\]
Consequently,
\[
H_N(t)\longrightarrow H(t)
\]
for every \(t\in(-1,1)\), where
\[
H(t)
=
\frac{\pi}{2}\,
\mathbb{E}\bigl[f(X(t))g(Y(t))\bigr]
\]
is the correlation function of the limiting scheme.

It remains to convert this pointwise convergence to locally uniform
convergence on the unit disk. For each \(N\), the Hermite expansions of
\(F_N\) and \(G_N\) give a holomorphic extension of \(H_N\) to
\[
\mathbb{D}
=
\{z\in\mathbb{C}:|z|<1\}.
\]
More explicitly, if
\[
F_N=\sum_{\alpha}\widehat{F_N}(\alpha)\operatorname{He}_{\alpha},
\qquad
G_N=\sum_{\alpha}\widehat{G_N}(\alpha)\operatorname{He}_{\alpha},
\]
then
\[
H_N(z)
=
\frac{\pi}{2}
\sum_{\alpha}
\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)z^{|\alpha|}.
\]
For \(z\) in the unit disk, the Cauchy--Schwarz inequality gives
\[
\begin{aligned}
|H_N(z)|
&\leq
\frac{\pi}{2}
\sum_{\alpha}
\bigl|
\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)
\bigr|
|z|^{|\alpha|} \\
&\leq
\frac{\pi}{2}
\left(
\sum_{\alpha}
|\widehat{F_N}(\alpha)|^2
\right)^{1/2}
\left(
\sum_{\alpha}
|\widehat{G_N}(\alpha)|^2
\right)^{1/2} \\
&\leq
\frac{\pi}{2}
\|F_N\|_2\|G_N\|_2
=
\frac{\pi}{2}.
\end{aligned}
\]
Here the second inequality uses \(|z|<1\), and the third follows from
the orthonormality of the Hermite polynomials.
% For \(z\in\mathbb{D}\), the Cauchy--Schwarz inequality and Parseval's identity
% give
% \[
% \begin{aligned}
% |H_N(z)|
% &\leq
% \frac{\pi}{2}
% \sum_{\alpha}
% \bigl|\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)\bigr|
% |z|^{|\alpha|} \\
% &\leq
% \frac{\pi}{2}
% \left(
% \sum_{\alpha}
% |\widehat{F_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2}
% \left(
% \sum_{\alpha}
% |\widehat{G_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2} \\
% &\leq
% \frac{\pi}{2}\|F_N\|_2\|G_N\|_2
% =
% \frac{\pi}{2}.
% \end{aligned}
% \]
Thus, the family \((H_N)_{N\geq 1}\) is locally bounded on \(\mathbb{D}\).
Since it converges pointwise on the interval \((-1,1)\), which has an
accumulation point in \(\mathbb{D}\). Vitali's theorem implies that
\((H_N)\) converges locally uniformly on \(\mathbb{D}\) to a holomorphic
function. On \((-1,1)\), this function agrees with \(H\). It is therefore
the holomorphic extension of the correlation function of the limiting
scheme.
\end{proof}

\begin{corollary}[Upper bound from a limiting Krivine scheme]
Let
\(
\mathcal{S}=(f,g,\rho_1,\ldots,\rho_k)
\)
be a limiting Krivine scheme. Let \(H\) be its correlation
function. Suppose that \(H'(0)\neq 0\), so that \(H\) has a local holomorphic inverse
at the origin. Write
\[
H^{-1}(z)
=
\sum_{j=0}^{\infty}a_{2j+1}z^{2j+1},
\]
and define its majorant by
\[
M(r)
=
\sum_{j=0}^{\infty}|a_{2j+1}|r^{2j+1}.
\]
If there exists \(\gamma>0\), within the radius of convergence of
\(H^{-1}\), such that
\(
M(\gamma)=1,
\)
then
\(
K_G
\leq
\frac{\pi}{2\gamma}.
\)
\end{corollary}
% \begin{theorem}[Finite-dimensional approximation of limiting schemes]
% Let
% \[
% \mathcal{S}=(f,g,\rho_1,\ldots,\rho_k)
% \]
% be a limiting Krivine scheme, and suppose that the discontinuity sets of
% \(f\) and \(g\) have Gaussian measure zero. Then the correlation function of
% \(\mathcal{S}\) extends holomorphically to the unit disk and is the locally
% uniform limit there of the correlation functions of ordinary
% finite-dimensional Krivine schemes.
% \end{theorem}

% \begin{proof}
% For each \(i\in\{1,\ldots,k\}\), there exist odd functions
% \(
% p_i,q_i: \R^3 \to \R 
% \)
% such that
% \(
% \|p_i\|_2=\|q_i\|_2=1
% \)
% and
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)]
% \]
% for every \(t\in(-1,1)\), where \(U,V\in\mathbb{R}^{3}\) are standard
% Gaussian vectors satisfying
% \[
% \mathbb{E}[U_aV_b]=t\delta_{ab}.
% \]

% For each positive integer \(N\), identify
% \[
% \mathbb{R}^{3N}
% =
% \prod_{i=1}^k \bigl(\mathbb{R}^{3}\bigr)^N.
% \]
% Thus, a point \(u\in\mathbb{R}^{3N}\) can be written as
% \[
% u=(u_{i,r})_{\substack{1\leq i\leq k\\1\leq r\leq N}},
% \qquad
% u_{i,r}\in\mathbb{R}^{3}.
% \]
% Define
% \[
% F_N(u)
% =
% f\left(
% \frac{1}{\sqrt{N}}\sum_{r=1}^N p_1(u_{1,r}),
% \ldots,
% \frac{1}{\sqrt{N}}\sum_{r=1}^N p_k(u_{k,r})
% \right).
% \]
% Similarly, for
% \[
% v=(v_{i,r})_{\substack{1\leq i\leq k\\1\leq r\leq N}}
% \in\mathbb{R}^{3N},
% \]
% define
% \[
% G_N(v)
% =
% g\left(
% \frac{1}{\sqrt{N}}\sum_{r=1}^N q_1(v_{1,r}),
% \ldots,
% \frac{1}{\sqrt{N}}\sum_{r=1}^N q_k(v_{k,r})
% \right).
% \]
% Because \(p_i,q_i,f\), and \(g\) are odd, both \(F_N\) and \(G_N\) are odd.
% Hence \((F_N,G_N)\) is an ordinary finite-dimensional Krivine scheme.

% Let \(H_N\) denote its correlation function. Fix \(t\in(-1,1)\), and let
% \(U^{(N)},V^{(N)}\in\mathbb{R}^{3N}\) be standard Gaussian vectors satisfying
% \[
% \mathbb{E}\bigl[U^{(N)}_aV^{(N)}_b\bigr]
% =
% t\delta_{ab}.
% \]
% Write these vectors in blocks as
% \[
% U^{(N)}=(U_{i,r})_{i,r},
% \qquad
% V^{(N)}=(V_{i,r})_{i,r},
% \]
% where the pairs \((U_{i,r},V_{i,r})\) are independent over \(i\) and \(r\),
% and each pair is a standard Gaussian pair in \(\mathbb{R}^3\) satisfying
% \[
% \mathbb{E}\bigl[(U_{i,r})_a(V_{i,r})_b\bigr]
% =
% t\delta_{ab}.
% \]

% Define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{r=1}^N p_i(U_{i,r}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{r=1}^N q_i(V_{i,r}),
% \]
% and set
% \[
% X_N=(X_{1,N},\ldots,X_{k,N}),
% \qquad
% Y_N=(Y_{1,N},\ldots,Y_{k,N}).
% \]
% Then
% \[
% H_N(t)
% =
% \frac{\pi}{2}\,
% \mathbb{E}\bigl[f(X_N)g(Y_N)\bigr].
% \]

% For each \(r\), consider the \(2k\)-dimensional random vector
% \[
% Z_r
% =
% \bigl(
% p_1(U_{1,r}),\ldots,p_k(U_{k,r}),
% q_1(V_{1,r}),\ldots,q_k(V_{k,r})
% \bigr).
% \]
% The vectors \(Z_1,Z_2,\ldots\) are independent and identically distributed,
% and
% \[
% (X_N,Y_N)
% =
% \frac{1}{\sqrt{N}}\sum_{r=1}^N Z_r.
% \]
% Since the functions \(p_i\) and \(q_i\) are odd, all coordinates of \(Z_r\)
% have mean zero. Moreover,
% \[
% \mathbb{E}[X_{i,N}X_{j,N}]
% =
% \mathbb{E}[Y_{i,N}Y_{j,N}]
% =
% \delta_{ij}
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{j,N}]
% =
% \delta_{ij}\rho_i(t).
% \]
% Indeed, coordinates with different values of \(i\) are independent, while
% for \(i=j\),
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]

% The multivariate central limit theorem therefore gives
% \[
% (X_N,Y_N)
% \xrightarrow[N\to\infty]{d}
% (X(t),Y(t)),
% \]
% where \((X(t),Y(t))\) is jointly Gaussian and satisfies
% \[
% \mathbb{E}[X_i(t)X_j(t)]
% =
% \mathbb{E}[Y_i(t)Y_j(t)]
% =
% \delta_{ij},
% \qquad
% \mathbb{E}[X_i(t)Y_j(t)]
% =
% \delta_{ij}\rho_i(t).
% \]
% This is precisely the Gaussian pair appearing in the definition of the
% limiting scheme.

% The function
% \[
% (x,y)\longmapsto f(x)g(y)
% \]
% is bounded, and its discontinuity set is contained in
% \[
% \bigl(\operatorname{Disc}(f)\times\mathbb{R}^k\bigr)
% \cup
% \bigl(\mathbb{R}^k\times\operatorname{Disc}(g)\bigr).
% \]
% Because \(X(t)\) and \(Y(t)\) are standard Gaussian vectors, the assumed
% Gaussian-nullity of the discontinuity sets implies that this union has
% probability zero under the law of \((X(t),Y(t))\). It follows that
% \[
% \mathbb{E}\bigl[f(X_N)g(Y_N)\bigr]
% \longrightarrow
% \mathbb{E}\bigl[f(X(t))g(Y(t))\bigr].
% \]
% Consequently,
% \[
% H_N(t)\longrightarrow H(t)
% \]
% for every \(t\in(-1,1)\), where
% \[
% H(t)
% =
% \frac{\pi}{2}\,
% \mathbb{E}\bigl[f(X(t))g(Y(t))\bigr]
% \]
% is the correlation function of the limiting scheme.

% It remains to upgrade this pointwise convergence to locally uniform
% convergence on the unit disk. For each \(N\), the Hermite expansions of
% \(F_N\) and \(G_N\) give a holomorphic extension of \(H_N\) to
% \[
% \mathbb{D}
% =
% \{z\in\mathbb{C}:|z|<1\}.
% \]
% More explicitly, if
% \[
% F_N=\sum_{\alpha}\widehat{F_N}(\alpha)\operatorname{He}_{\alpha},
% \qquad
% G_N=\sum_{\alpha}\widehat{G_N}(\alpha)\operatorname{He}_{\alpha},
% \]
% then
% \[
% H_N(z)
% =
% \frac{\pi}{2}
% \sum_{\alpha}
% \widehat{F_N}(\alpha)\widehat{G_N}(\alpha)z^{|\alpha|}.
% \]
% For \(z\in\mathbb{D}\), the Cauchy--Schwarz inequality and Parseval's identity
% give
% \[
% \begin{aligned}
% |H_N(z)|
% &\leq
% \frac{\pi}{2}
% \sum_{\alpha}
% \bigl|\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)\bigr|
% |z|^{|\alpha|} \\
% &\leq
% \frac{\pi}{2}
% \left(
% \sum_{\alpha}
% |\widehat{F_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2}
% \left(
% \sum_{\alpha}
% |\widehat{G_N}(\alpha)|^2|z|^{|\alpha|}
% \right)^{1/2} \\
% &\leq
% \frac{\pi}{2}\|F_N\|_2\|G_N\|_2
% =
% \frac{\pi}{2}.
% \end{aligned}
% \]
% Thus, the family \((H_N)_{N\geq 1}\) is locally bounded on \(\mathbb{D}\).
% Since it converges pointwise on the interval \((-1,1)\), which has an
% accumulation point in \(\mathbb{D}\), Vitali's theorem implies that
% \((H_N)\) converges locally uniformly on \(\mathbb{D}\) to a holomorphic
% function. On \((-1,1)\), this function agrees with \(H\). It is therefore
% the holomorphic extension of the correlation function of the limiting
% scheme.
% \end{proof}


% \begin{lemma}
% Let \(\rho_1,\ldots,\rho_k\) be allowable correlation functions. 
% For every \(t\in(-1,1)\), there is a sequence \(\left\{\left(X^{(N)},Y^{(N)}\right)\right\}_{N \ge 1}\) of pairs of finite-dimensional random vectors in \(\mathbb{R}^k\), constructed from coordinatewise
% \(t\)-correlated Gaussians, such that
% \[
% \left(X^{(N)},Y^{(N)}\right)
% \longrightarrow
% (X,Y), \qquad N \rightarrow \infty 
% \]
% where \(X,Y \in \R^k\) are standard Gaussian vectors satisfying
% \[
% \mathbb{E}[X_iY_j]
% =
% \delta_{ij}\rho_i(t).
% \]
% \end{lemma}

% \begin{proof}
% For each \(i\), choose odd variance-one functions \(p_i,q_i\) such that
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)].
% \]
% For \(N\geq 1\), define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}),
% \]
% where the pairs \((U_{i,j},V_{i,j})\) are independent over \(i\) and \(j\),
% and each pair has coordinatewise correlation \(t\).

% For every \(i\),
% \[
% \mathbb{E}[X_{i,N}^2]
% =
% \mathbb{E}[Y_{i,N}^2]
% =
% 1
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]
% Coordinates with different values of \(i\) are independent. The multivariate
% central limit theorem therefore gives the claimed convergence.
% \end{proof}

% For example, taking \(p=q=\operatorname{He}_3\) gives the correlation \(t^3\),
% while taking \(p=q=\operatorname{He}_5\) gives \(t^5\). The theorem allows
% arbitrary allowable correlations in place of these individual powers.


% \begin{theorem}
% Suppose that the discontinuity sets of \(f\) and \(g\) have Gaussian measure
% zero. Then the correlation function of a limiting Krivine scheme is the locally
% uniform limit on the unit disk of correlation functions of ordinary
% finite-dimensional Krivine schemes.
% \end{theorem}

% \begin{proof}
% For each \(i\), choose odd variance-one functions \(p_i,q_i\) such that
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)].
% \]
% For \(N\geq 1\), define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}),
% \]
% where the pairs \((U_{i,j},V_{i,j})\) are independent over \(i\) and \(j\),
% and each pair has coordinatewise correlation \(t\).

% For every \(i\),
% \[
% \mathbb{E}[X_{i,N}^2]
% =
% \mathbb{E}[Y_{i,N}^2]
% =
% 1
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]
% Coordinates with different values of \(i\) are independent. By the multivariate central limit theorem, this implies that 


% Define finite-dimensional rounding functions by
% \[
% f_N
% =
% f(X_{1,N},\ldots,X_{k,N}),
% \qquad
% g_N
% =
% g(Y_{1,N},\ldots,Y_{k,N}).
% \]
% Since the functions \(p_i,q_i,f,g\) are odd, the functions \(f_N\) and \(g_N\)
% are odd. They therefore define ordinary finite-dimensional Krivine schemes.

% Let
% \[
% H_N(t)
% =
% \frac{\pi}{2}\mathbb{E}[f_Ng_N]
% \]
% be their correlation functions. For every fixed \(t\in(-1,1)\), the previous
% theorem gives
% \[
% \bigl(X^{(N)},Y^{(N)}\bigr)
% \Longrightarrow
% (X,Y).
% \]
% The discontinuity assumption then implies
% \[
% H_N(t)\longrightarrow H(t).
% \]

% For each \(N\), the Hermite expansion of \(f_N\) and \(g_N\) shows that \(H_N\)
% is holomorphic on the unit disk and satisfies
% \[
% |H_N(z)|
% \leq
% \frac{\pi}{2}.
% \]
% The family \((H_N)\) is therefore locally bounded. Since it converges pointwise
% on the real interval \((-1,1)\), Vitali's theorem gives locally uniform
% convergence on the unit disk.
% \end{proof}




% \section{Limiting Krivine Schemes}

% The construction in this paper starts from a simple observation. A normalized
% average of degree-\(d\) Hermite polynomials converges to a Gaussian coordinate,
% while its correlation with the corresponding coordinate on the other side is
% \(t^d\). The degrees \(3\) and \(5\) used in our construction therefore produce
% the correlations \(t^3\) and \(t^5\).

% In this section, we first determine which correlation functions can be produced
% in this way. We then use them to define limiting Krivine schemes and show that
% these limiting schemes arise from ordinary finite-dimensional Krivine schemes.

% \subsection{Correlation functions}

% Let \((\operatorname{He}_d)_{d\geq 0}\) denote the orthonormal probabilist
% Hermite polynomials. If \(U,V\) are standard Gaussians with correlation \(t\),
% then
% \[
% \mathbb{E}
% \left[
% \operatorname{He}_d(U)\operatorname{He}_e(V)
% \right]
% =
% \mathbf{1}_{\{d=e\}}t^d.
% \]

% Thus a degree-\(d\) Hermite function produces the correlation \(t^d\). More
% generally, suppose that \(p\) and \(q\) are odd functions of a standard Gaussian
% vector. Writing their Hermite expansions by degree suggests that their
% correlation must have the form
% \[
% \sum_{\substack{d\geq 1\\ d\text{ odd}}} c_dt^d.
% \]
% Cauchy--Schwarz will force \(\sum_d |c_d|\leq 1\). This motivates the following
% definition.

% \begin{definition}
% A function \(\rho:(-1,1)\to\mathbb{R}\) is an allowable correlation function
% if
% \[
% \rho(t)
% =
% \sum_{\substack{d\geq 1\\ d\text{ odd}}}c_dt^d
% \qquad\text{and}\qquad
% \sum_{\substack{d\geq 1\\ d\text{ odd}}}|c_d|
% \leq 1.
% \]
% \end{definition}

% The coefficient condition implies that \(|\rho(t)|\leq |t|\) for
% \(t\in(-1,1)\). In particular, \(\rho(t)\in[-1,1]\). The functions \(t\),
% \(t^3\), and \(t^5\) are the simplest examples.

% The next theorem shows that this is exactly the class produced by odd Gaussian
% functions.

% \begin{theorem}
% A function \(\rho\) is allowable if and only if there are odd functions
% \(p,q\in L_2(\gamma_m)\), for some \(m\), such that
% \(\|p\|_2=\|q\|_2=1\) and
% \[
% \rho(t)=\mathbb{E}[p(U)q(V)],
% \]
% where \(U,V\in\mathbb{R}^m\) are standard Gaussian vectors with
% \(\mathbb{E}[U_iV_j]=t\delta_{ij}\).
% \end{theorem}

% \begin{proof}
% Suppose first that \(p\) and \(q\) are odd and have \(L_2\)-norm one. Write
% their Hermite expansions by degree as
% \[
% p=\sum_{\substack{d\geq 1\\ d\text{ odd}}}p_d,
% \qquad
% q=\sum_{\substack{d\geq 1\\ d\text{ odd}}}q_d.
% \]
% Here \(p_d\) and \(q_d\) are the degree-\(d\) Hermite components.

% Different Hermite degrees are orthogonal, while degree \(d\) contributes a
% factor \(t^d\). Hence
% \[
% \mathbb{E}[p(U)q(V)]
% =
% \sum_{\substack{d\geq 1\\ d\text{ odd}}}
% \langle p_d,q_d\rangle t^d.
% \]
% Set \(c_d=\langle p_d,q_d\rangle\). Then
% \[
% \sum_d|c_d|
% \leq
% \sum_d\|p_d\|_2\|q_d\|_2
% \leq
% \left(\sum_d\|p_d\|_2^2\right)^{1/2}
% \left(\sum_d\|q_d\|_2^2\right)^{1/2}
% =
% 1.
% \]
% Thus the resulting correlation function is allowable.

% Conversely, suppose that
% \[
% \rho(t)=\sum_{d\text{ odd}}c_dt^d,
% \qquad
% s:=\sum_{d\text{ odd}}|c_d|\leq 1.
% \]
% For \(x=(x_1,x_2,x_3)\in\mathbb{R}^3\), define
% \[
% p(x)
% =
% \sum_{d\text{ odd}}
% \sqrt{|c_d|}\operatorname{He}_d(x_1)
% +
% \sqrt{1-s}\,x_2
% \]
% and
% \[
% q(x)
% =
% \sum_{d\text{ odd}}
% \operatorname{sgn}(c_d)\sqrt{|c_d|}
% \operatorname{He}_d(x_1)
% +
% \sqrt{1-s}\,x_3.
% \]
% Both functions are odd. Orthogonality gives \(\|p\|_2=\|q\|_2=1\).

% Let \(U,V\in\mathbb{R}^3\) be standard Gaussian vectors with
% \(\mathbb{E}[U_iV_j]=t\delta_{ij}\). The terms involving \(U_2\) and \(V_3\)
% have zero cross-correlation. Therefore
% \[
% \mathbb{E}[p(U)q(V)]
% =
% \sum_{d\text{ odd}}c_dt^d
% =
% \rho(t).
% \]
% \end{proof}

% If the same function is used on both sides, then the coefficients are
% nonnegative. Indeed, if \(\rho(t)=\mathbb{E}[p(U)p(V)]\), then
% \[
% \rho(t)=\sum_{d\text{ odd}}\|p_d\|_2^2t^d.
% \]
% Thus \(c_d\geq 0\) and \(\sum_dc_d=1\). Allowing different functions on the two
% sides gives the signed coefficients in the theorem.


% \subsection{Central limit realization}

% We now explain why allowable correlation functions occur as limits of ordinary
% finite-dimensional Gaussian constructions. The idea is the same as in the
% degree-\(3\) and degree-\(5\) averages used in this paper: take many independent
% copies of the functions \(p\) and \(q\), and normalize their sums.

% \begin{theorem}
% Let \(\rho_1,\ldots,\rho_k\) be allowable correlation functions. For every
% \(t\in(-1,1)\), there are finite-dimensional random vectors
% \(X^{(N)},Y^{(N)}\in\mathbb{R}^k\), constructed from coordinatewise
% \(t\)-correlated Gaussian inputs, such that
% \[
% \bigl(X^{(N)},Y^{(N)}\bigr)
% \Longrightarrow
% (X,Y),
% \]
% where \(X,Y\) are standard Gaussian vectors satisfying
% \[
% \mathbb{E}[X_iY_j]
% =
% \delta_{ij}\rho_i(t).
% \]
% \end{theorem}

% \begin{proof}
% For each \(i\), choose odd variance-one functions \(p_i,q_i\) such that
% \[
% \rho_i(t)=\mathbb{E}[p_i(U)q_i(V)].
% \]
% For \(N\geq 1\), define
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}),
% \]
% where the pairs \((U_{i,j},V_{i,j})\) are independent over \(i\) and \(j\),
% and each pair has coordinatewise correlation \(t\).

% For every \(i\),
% \[
% \mathbb{E}[X_{i,N}^2]
% =
% \mathbb{E}[Y_{i,N}^2]
% =
% 1
% \]
% and
% \[
% \mathbb{E}[X_{i,N}Y_{i,N}]
% =
% \mathbb{E}[p_i(U)q_i(V)]
% =
% \rho_i(t).
% \]
% Coordinates with different values of \(i\) are independent. The multivariate
% central limit theorem therefore gives the claimed convergence.
% \end{proof}

% For example, taking \(p=q=\operatorname{He}_3\) gives the correlation \(t^3\),
% while taking \(p=q=\operatorname{He}_5\) gives \(t^5\). The theorem allows
% arbitrary allowable correlations in place of these individual powers.

% \subsection{Limiting schemes}

% We can now package several allowable correlations into a Krivine scheme. The
% only change from the usual definition is that the \(i\)-th pair of Gaussian
% coordinates has correlation \(\rho_i(t)\), rather than \(t\).

% \begin{definition}
% A limiting Krivine scheme consists of odd measurable functions
% \(f,g:\mathbb{R}^k\to\{-1,1\}\) and allowable correlation functions
% \(\rho_1,\ldots,\rho_k\).

% For \(t\in(-1,1)\), let \(X,Y\in\mathbb{R}^k\) be jointly Gaussian with
% \[
% \mathbb{E}[X_iX_j]
% =
% \mathbb{E}[Y_iY_j]
% =
% \delta_{ij},
% \qquad
% \mathbb{E}[X_iY_j]
% =
% \delta_{ij}\rho_i(t).
% \]
% The correlation function of the scheme is
% \[
% H(t)
% =
% \frac{\pi}{2}\mathbb{E}[f(X)g(Y)].
% \]
% \end{definition}

% The usual Krivine scheme is the special case
% \(\rho_1(t)=\cdots=\rho_k(t)=t\). The limiting scheme used in this paper has
% correlations
% \[
% (t,t,t^3,t^5).
% \]

% The point of the definition is that these limiting objects do not enlarge the
% theory artificially. They are limits of ordinary finite-dimensional Krivine
% schemes.

% \begin{theorem}
% Suppose that the discontinuity sets of \(f\) and \(g\) have Gaussian measure
% zero. Then the correlation function of a limiting Krivine scheme is the locally
% uniform limit on the unit disk of correlation functions of ordinary
% finite-dimensional Krivine schemes.
% \end{theorem}

% \begin{proof}
% For each \(\rho_i\), choose functions \(p_i,q_i\) as above and form the
% normalized sums
% \[
% X_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N p_i(U_{i,j}),
% \qquad
% Y_{i,N}
% =
% \frac{1}{\sqrt{N}}\sum_{j=1}^N q_i(V_{i,j}).
% \]
% Define finite-dimensional rounding functions by
% \[
% f_N
% =
% f(X_{1,N},\ldots,X_{k,N}),
% \qquad
% g_N
% =
% g(Y_{1,N},\ldots,Y_{k,N}).
% \]
% Since the functions \(p_i,q_i,f,g\) are odd, the functions \(f_N\) and \(g_N\)
% are odd. They therefore define ordinary finite-dimensional Krivine schemes.

% Let
% \[
% H_N(t)
% =
% \frac{\pi}{2}\mathbb{E}[f_Ng_N]
% \]
% be their correlation functions. For every fixed \(t\in(-1,1)\), the previous
% theorem gives
% \[
% \bigl(X^{(N)},Y^{(N)}\bigr)
% \Longrightarrow
% (X,Y).
% \]
% The discontinuity assumption then implies
% \[
% H_N(t)\longrightarrow H(t).
% \]

% For each \(N\), the Hermite expansion of \(f_N\) and \(g_N\) shows that \(H_N\)
% is holomorphic on the unit disk and satisfies
% \[
% |H_N(z)|
% \leq
% \frac{\pi}{2}.
% \]
% The family \((H_N)\) is therefore locally bounded. Since it converges pointwise
% on the real interval \((-1,1)\), Vitali's theorem gives locally uniform
% convergence on the unit disk.
% \end{proof}

% The boundary assumption is automatic for the threshold functions used in this
% paper. It can also be removed for general odd measurable functions by a
% standard approximation argument.

==> paper/abstract.tex <==
\abstract{

We establish new bounds on the Grothendieck constant \(\KG\):
\[
    \frac{6\pi}{11}
    \le
    \KG
    \le
    \frac{\pi}{2\log(1+\sqrt2)} - 10^{-4}.
\]
Methodologically, our lower bound approach differs from previous works by establishing limitations on the asymptotically optimal Krivine schemes, rather than giving explicit constructions of gap instances.
Our upper bound is obtained by proposing and analyzing the first asymptotic construction of rounding schemes, whereas previous works only consider low-dimensional schemes.
Together, these bounds determine the previously unknown tenths digit of \(\KG\) to be $7$. 
The bounds were discovered by a long-running collaborative effort of humans and a long-horizon AI research system that we engineered. A detailed account of the AI-assisted research process appears in a companion paper~\cite{lisaha2026longhorizon}.

}
\newpage 

\tableofcontents 

% \newpage

==> paper/ai_section.tex <==
% ============================================================================
% AI SECTION -- draft to be merged into the main paper as a single section.
% No abstract and no title: the \section below is the section itself.
% Style: anton_style.md. Items needing author confirmation are marked %% TODO.
% ============================================================================


\hypersetup{
  colorlinks=true,
  linkcolor=blue!55!black,
  urlcolor=blue!55!black,
  citecolor=blue!55!black
}

\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}
\setlist[itemize]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}
\setlist[enumerate]{leftmargin=1.6em,itemsep=2pt,topsep=3pt}

\part{AI Methodology and Analysis}
\label{sec:ai}


The results in this paper were obtained in collaboration with an autonomous
AI research system. The cubic--quintic
construction and its certificate (Theorem~\ref{thm:cubic-quintic-upper-bound})
predate the current system and were found through conversation with GPT-5.5-Pro. The lower bound $\KG\ge6\pi/11$ was
discovered and first proved by the system; we have since verified the
argument ourselves, and the proof in this paper is our revision of the
system's write-up. The system also produced further improvements on both
sides of the problem, which we report in Section~\ref{sec:ai-results} but do
not state as theorems, because their certificates have not yet been human-verified. This section documents the methodology
(Section~\ref{sec:ai-methodology}), quantifies the run and its outcomes
(Section~\ref{sec:ai-results}), reconstructs how the lower bound was found
(Section~\ref{sec:ai-case-study}), and discusses what the record shows about
the strengths and weaknesses of current AI systems as mathematical
collaborators (Sections~\ref{sec:ai-discussion} and~\ref{sec:ai-future}).

\section{Methodology}
\label{sec:ai-methodology}

\paragraph{AI models and compute.}
The run used two frontier language models: a reasoning model (OpenAI
GPT-5.5-Pro at maximal reasoning effort, replaced mid-run by GPT-5.6-Sol)
and a coding agent (Anthropic Claude Code, running Claude Opus and later
Claude Fable~5). Floating-point searches
ran on a single four-GPU node, and every Arb-certified computation was redone in interval arithmetic on CPU.

% \paragraph{The AI research system.}
% The AI research system is designed as a harness. The 
% harness couples the two models in distinct roles: (1) The \textit{reasoning model}
% serves as the brain that selects directions, develops arguments, specifies
% experiments, and audits the resulting claims; (2) The \textit{coding agent} serves as
% the executor that maintains the project repository, implements and runs
% experiments, retrieves literature, and drives the reasoning model through
% a scripted interface. The models run in bounded sessions, and no model
% context survives from one session to the next; continuity is carried by
% files, principally a problem statement, a single summary file that serves
% as working memory and into which finished work is merged, and append-only
% transcripts and experiment logs. The harness was adjusted repeatedly over
% the run in response to observed failures; we describe its final form, to
% the extent needed to interpret the record.

\paragraph{The AI research system.}
The AI research system is organized as a harness coupling two agents in distinct roles: (1) the \textit{reasoning agent} serves as the brain that selects directions, develops arguments, specifies experiments, and audits the resulting claims, and (2) the \textit{coding agent} serves as the executor that maintains the project repository, implements and runs experiments, retrieves literature, and drives the reasoning model through a scripted interface.

The agents run in bounded sessions, and no agent context survives from one session to the next. Continuity is instead carried by files, principally a problem statement, a single summary file that serves as working memory and into which finished work is merged, and append-only transcripts and experiment logs. The harness was adjusted repeatedly over the run in response to observed failures; we describe its final form, to the extent needed to interpret the record.

\paragraph{Run configuration.}
Work is organized into \emph{sessions} of a few hours, of which two to
five run concurrently on mutually distinct directions. A session passes
through fixed phases: orientation from the problem statement and summary
files, selection of a focus, a research loop in which the reasoning model
requests computations, literature, or further reasoning time, and a
closing audit that produces a calibrated summary in which every claim is
tagged as proven, numerically supported, conjectural, or heuristic. We
reserve the word theorem, here and in the rest of the paper, for
statements that we have additionally checked ourselves.

The run was initialized with our prior work on the constant: the
cubic--quintic scheme, the coefficient formulas and certification
machinery, several months of accumulated notes, and a problem statement
listing candidate directions for both bounds. The search space the run
explored is a generalization of the cubic--quintic scheme, and the
possibility of converting obstructions into lower bounds was raised, as a
suggestion, in the problem statement. The system therefore operated
downstream of the mathematical framework it was given, a point quantified
in Section~\ref{sec:ai-case-study}.

\paragraph{Human collaboration.}
Human operators (the authors) steered the run asynchronously
through text files read at the start of, and during, every session.
Steering consisted of priorities, targets, audits of the run's own claims,
and occasional mathematical pointers; about forty directives were
issued over the run. 
% The operator contributed no proof steps through this
channel.

\section{Results}
\label{sec:ai-results}

The run spanned June~16 to July~24, 2026. It comprised
roughly 240 research sessions. The reasoning model was called 2{,}091
times, consuming about 152 million tokens at an estimated \$5{,}400 in
API cost; the coding agent ran on a flat-rate subscription (Claude Max).
Table~\ref{tab:run} collects these figures, and
Table~\ref{tab:timeline} gives the timeline of the bounds.

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}ll@{}}
\toprule
Duration & June 16 -- July 24, 2026 (main phase through July 4)\\
Research sessions & $\approx240$\\
Reasoning model & GPT-5.5-Pro, later GPT-5.6-Sol; maximal effort\\
Usage and cost & 2{,}091 calls; $\approx152$M tokens; $\approx\$5{,}400$\\
Coding agent & Claude Code (Opus, later Fable 5); subscription\\
Human steering  $\approx40$ dated directives\\
\bottomrule
\end{tabular}
\caption{\textbf{The run at a glance.} Aggregates computed from the harness
telemetry. Dollar figures are list-price estimates; coding-agent usage was
only partially metered.
}
\label{tab:run}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lp{0.76\textwidth}@{}}
\toprule
Sessions & Event\\
\midrule
1 & run begins from the interval $1.6769566742\le\KG\le1.7818666070$
(the upper end is the cubic--quintic bound of this paper)\\
18 & upper-bound search plateaus; the operators direct a pivot to the
lower bound\\
44 & numerical upper bound $1.7802243$ recorded (later withdrawn)\\
55--57 & affine reframe; $\KG\ge6\pi/11$ derived\\
58--64 & $6\pi/11$ proof machine-audited; first \LaTeX{} write-up\\
92, 117 & lower bounds $27\pi/49\approx1.7311$ and
$51\pi/92\approx1.7415$ machine-verified\\
follow-up & the session-44 value found unsupported by internal audit and
withdrawn\\
follow-up & upper bound $1.781801841033$ machine-certified\\
follow-up & upper bound $1.7813319810625639$ machine-certified;
adversarial review passed\\
\bottomrule
\end{tabular}
\caption{\textbf{Timeline of the bounds produced during the run.}
Machine-verified means accepted by the verification protocol of
Section~\ref{sec:ai-methodology}. The last three events fall in the short
follow-up phases, whose sessions we do not cite individually. Of the
run's results, only $\KG\ge6\pi/11$ has additionally been verified by the
authors; it is the result stated as a theorem in this paper.}
\label{tab:timeline}
\end{table}

The run's principal outcome, and the one this paper states as a theorem,
is the lower bound $\KG\ge6\pi/11$, whose discovery
Section~\ref{sec:ai-case-study} reconstructs. Beyond it, the run produced
machine-certified upper bounds of $1.781801841033$ and then
$1.7813319810625639$, improving on the cubic--quintic value, together with
the two stronger lower bounds listed in Table~\ref{tab:timeline}. We
report these as machine-verified claims rather than theorems: each passed
the full internal protocol, but we have not yet verified their
certificates ourselves.
%% TODO: reconcile with the main paper's discussion of concurrent work
%% (e.g. Heilman's computer-assisted improvement of Krivine's bound,
%% arXiv:2606.00247).

\section{Case study: from a failed upper-bound search to a lower bound}
\label{sec:ai-lower-bound-case-study}

The lower bound is the run's main discovery. We reconstruct it here in
outline, highlighting the human interventions that shaped it, and the ingenuity of the AI system once it had the right framing.

The lower bound began with a plateauing search for a better upper bound. The system explored several variants of the limiting Krivine schemes developed in Section~\ref{sec:LimitingKrivine}. Although the constructions differed, they repeatedly encountered
the same tradeoff: suppressing the unwanted nonlinear terms in the inverse majorant series also weakened
the leading term. The run recorded this pattern, but continued to search
for further constructions rather than treating the repeated failures as
evidence of a general obstruction.

The important human contribution was in identifying there was likely an analytic obstruction, and in recognizing that proving the generality of this obstruction for all mixed and limiting schemes is mathematically valuable as the optimality theorem of Naor and Regev~\cite{naor2014krivine} would imply a lower bound for $K_G$. Thus, the operators asked the system to stop searching for new limiting Krivine schemes, and instead synthesize the its failures so far, search for patterns, and attempt to generalize and prove these for all schemes.

Once this objective was fixed, and with a bit more high-level human guidance, the system developed the central argument
and produced a complete proof (see all of Part~\ref{part:LowerBound}). It expressed the obstruction as an
affine inequality between the two leading coefficients of a scheme's
correlation function (see Equation~\ref{eq:affine-coefficient-inequality}). Because this inequality is preserved under averaging
and limits, it extends to mixed and limiting schemes. The system then
cleverly reduced the high-dimensional terms it needed to bound to one-dimensional estimates and produced
the required computer-assisted certificate, yielding
\[
    \KG \geq \frac{6\pi}{11}.
\]
The authors subsequently revised the exposition and independently verified
the proof.

This episode illustrates the different roles of the human operators and the AI system throughout the run. The system was effective at technical execution: drawing from its wealth of mathematical knowledge and its competence in problem-solving to propose lemmas and construct proofs. The human input was primarily of research judgement and mathematical taste: judging when a research direction has been somewhat exhausted, understanding that mathematical understanding and discoveries frequently come from synthesizing failures, 
and recoginizing that a new lower-bound mechanism is much more interesting than a small numerical improvement to a
known upper-bound method. Appendix~\ref{app:ai-case-study} gives the
detailed chronology.


\section{Discussion}
\label{sec:ai-discussion}

The record supports a consistent capability profile: strong technical
execution, with persistent failures in the judgement that directs it. We
summarize the strengths, then the weaknesses, exemplified by Section~\ref{sec:ai-case-study} 

make concrete, describe
the human operator's involvement, and close by relating the run to recent
AI results in mathematics.

\subsection{Strengths}

Three strengths carried the run. The first is technical range with effective
recall: given a one-word pointer to Naor's work, the system identified the
relevant theorem, verified its normalization against the paper, and computed
the slack available for a lossy transfer; given a plateau, it produced six
structurally distinct escape mechanisms in two days. The second is local
invention: the affine family, the fiber reduction, the closure lemma, and
the certificate architecture were machine products, several arriving within
hours once the question was well posed. The third is speed and reliability
of execution: from the reframe to a machine-audited, interval-certified
proof took about a day, and most individual technical errors were caught by
the system's own verification passes. In one representative episode
(sessions p44 and p49), a claimed bound of $\KG\ge1.7754518$
was refuted within five hours by an adversarial session that computed its
true margin to be approximately $-8\times10^{-8}$, and the record was
corrected to the defensible value.

\subsection{Weaknesses}

Each intervention of Section~\ref{sec:ai-case-study} was needed because a
specific capability was absent. The paragraphs below name these
capabilities and add further instances from the record.

\paragraph{Poor judgement of what is interesting.}
The system did not reliably rank work by mathematical interest. The second
and third interventions are the clearest cases: the run treated refinements
of the two-dimensional ceiling as progress when only the general bound
mattered, and, once the family of rungs existed, it valued improvements
within the family over establishing the first certified rung. The same
tendency appeared at smaller scales throughout, from sessions spent on
$10^{-5}$-sized improvements to mechanisms the run already understood, down
to reported values tuned to the edges of their enclosures. The implication
for collaboration is that the objective of the research cannot yet be
delegated. The operator's judgements of interest were few, but each
redirected weeks of machine effort, and between them the system optimized,
competently, whatever was in front of it. On a problem of this size the
space of possible intermediate constructions is unbounded, and a ranking by
expected interest is what makes the search tractable; supplying that
ranking was the human's principal ongoing contribution.

\paragraph{Lack of high-level research skills.}
The system managed individual arguments well and the research process
poorly: it did not decide when to persist, when to switch, or what a
sequence of failures implied. The first intervention is the sharpest case,
since the dualization of failures into a lower bound was suggested in the
problem statement the system re-read at every session, the six failures
were in its memory, and the step was taken only when ordered. The record
contains three further episodes of the same shape, of fourteen, roughly two
dozen, and about a dozen sessions respectively (the two-dimensional
extension, near-sharp variants of the lower bound, and the July
certification effort), in each of which the run circled a target without
progress until the operator ended the loop. The implication is that
autonomous running time does not by itself convert into progress. Once the
accessible directions were exhausted, additional sessions multiplied
execution, not judgement, and the run's rate of real progress was set by
the frequency of strategic correction; additional compute would not have
changed it. Oversight of such systems is accordingly most valuable at the
level of strategy, which is precisely the level at which the system did not
correct itself.

\paragraph{Unreliable memory.}
The harness's file-based memory preserved statements more reliably than
their qualifications. The withdrawn upper bound of Table~\ref{tab:timeline}
is the clearest case. In session 44 the run recorded a numerical upper
bound of $1.7802243$, with caveats attached; over the nineteen days the
value stood in working memory, re-summarization detached the caveats from
the headline number, and a note defending the value was written three days
before the internal audit that refuted it, finding the score inflated by a
finite truncation window and the underlying correlation profile
infeasible. A related failure occurred inside verification, where a
dedicated replay of the $51\pi/92$ certificate (session p95) passed it
because the replay inherited the framing of the argument it was checking;
the invalidating error was found the same day by a session that rebuilt the
argument from scratch (session p102). We attribute both failures to scale.
The run produced hundreds of sessions and tens of millions of tokens of
intermediate mathematics, and each new session could be shown only a small
distillate of it. What to retain, at what resolution, and with which
qualifications attached was itself decided by the models, through repeated
summarization, and repeated summarization is exactly where caveats detach
and inherited framings go unquestioned. Unlike the previous two weaknesses,
this one looks amenable to engineering: memory for such systems plausibly
needs more structure than prose summaries provide, for instance a graph of
claims carrying provenance and qualifications, so that important
information remains retrievable without being repeatedly re-serialized
through a model's context window.

\paragraph{Origins of the weaknesses.}
We believe these gaps have a common origin in how current systems are
produced. Models are trained and evaluated on problems selected for being
small enough to pose, sandbox, and score, and nothing in that regime
exercises the allocation of weeks of effort across an open-ended search.
The corpus they learn mathematics from is, moreover, made of finished
mathematics: the literature records definitions, theorems, and polished
proofs, while the process that produced them, the dead ends, the decisions
to abandon or reframe, the judgement of what was worth attempting, is
largely absent from the written record. A system trained this way can be
expected to acquire technique and the form of finished mathematics while
remaining weak at exactly the process skills described above, and that is
what we observe.

\subsection{Human operator involvement}

A useful summary of the collaboration is obtained by counting who caught
which errors. Errors in individual claims, such as wrong constants, broken
certificates, and invalid steps, were caught almost entirely by the system
itself. Failure patterns spanning many sessions, such as the three circling
episodes and the detachment of caveats from claims, were caught by the
operator in every recorded instance and by the system in none. The system
reliably falsifies a claim once the claim is specified; deciding which
claims to distrust remained a human function throughout. Consistent with
this, the operator's leverage came less from mathematical suggestions, most
of which the system correctly tested and discarded, than from calibration:
setting targets, ending loops, and auditing the run's own reporting. We also
note a regularity with design consequences: every overclaiming incident in
the record sits at a target with nearly zero margin, whereas the results
that survived verification all carry slack. This suggests that systems of
this kind are most productive when aimed at robust targets, with sharp
constants attempted only from a secured base.

\subsection{Relation to recent work}

Recent successes of AI in mathematics, including on open problems, are of
a different kind from the work reported here. Evaluator-guided search has
produced record
constructions~\cite{funsearch,novikov2025alphaevolvecodingagentscientific, charton2024patternboostconstructionsmathematicslittle},
and formal provers have shown proficiency at solving olympiad-level
problems \cite{novikov2025alphaevolvecodingagentscientific}.
%% TODO: the formal-provers citation should probably point to AlphaProof
%% (Hubert et al., Nature 651:607--613, 2026) rather than AlphaEvolve.
In recent and concurrent work, frontier models have gone further: an
internal reasoning model at OpenAI has disproved the Erd\H{o}s
unit-distance conjecture \cite{openai2026planarpointsets}, a counterexample to the Jacobian conjecture using Claude Fable 5
\cite{jacobian}, and OpenAI has announced solutions to ten open problems in mathematics and theoretical computer
science \cite{openai2026ten}. Most of these results involved resolving a
single well-posed statement by construction. Moreover, none explicitly
required significant long-horizon reasoning. Finally, all of the recent
results with frontier models were found fully autonomously, without
sustained human intervention.

Our work is an extensive case study of how humans and AI can collaborate
on mathematical research. The problem is more open-ended, requiring a
research program where over the course of weeks intermediate results
accumulate and directions are opened and abandoned. Moreover, humans were
consistently steering the system and providing feedback. We hope that our
experiences outlined in this section will be useful to future AI and mathematics researchers alike.

\section{Future directions}
\label{sec:ai-future}

\paragraph{Mathematics.}
The immediate items are the machine-verified claims of
Table~\ref{tab:timeline}: human verification of the two certified upper
bounds and of the lower bounds $27\pi/49$ and $51\pi/92$ would upgrade each
to a theorem. Beyond them, the run's internal analysis identifies the
tangent case $\lambda=\tfrac12$ of the affine family, equivalent to a sharp
degree-three chaos inequality, as the natural boundary of the method and
worth $\KG\ge9\pi/16$ if resolved.
% {\color{red}AX: If you're brave, conjecture that \(K_G = \sqrt{\pi}\)}

\paragraph{Toward AI systems for long-horizon research.}
If the diagnosis of Section~\ref{sec:ai-discussion} is right, the
requirements for progress follow from it. First, mathematical
interestingness needs to become an object of study in its own right: the
judgement that selects which questions, intermediate constructions, and
targets are worth pursuing was the most consequential input the human
supplied, and there is at present no training signal or benchmark that
rewards it. Second, the process of research mathematics needs data. What
humans actually do between problem statement and finished paper,
how they allocate effort, learn from repeated failure, and decide to
reframe, is barely recorded anywhere; records of long runs such as ours,
which preserve every step including the unsuccessful ones, are one way to
begin creating such data, and we release ours in that spirit. Third,
evaluation must move to horizons where these capabilities matter, treating
a weeks-long research program rather than a single problem as the unit of
assessment, with memory and calibration measured alongside correctness.
These conclusions carry the usual caution that they derive from one run on
one problem; replications on other open problems, successful or not, would
be the most useful follow-up work.

\paragraph{Human--AI collaboration.}
The run also suggests where collaboration of this kind is heading. Within
it, the contributions that required a human were not technical: the system
supplied the arguments, the computations, the certificates, and the first
write-up, while the human supplied the problem, the taste, and the
strategic corrections. If the technical abilities of these systems continue
to improve, this division will sharpen, and the human's role in
such collaborations will concentrate into choosing what to work on, judging
which objects and targets matter, and deciding what to trust: directing
research that one does not personally execute. A similar shift is already
under way in software engineering. We expect working modes of this kind to
become common in mathematics, and the run documented here, with its
weaknesses as much as its results, is an early picture of what they will
require of the human operator.

\paragraph{Statement on AI use.}
Large language models were used extensively in the research reported in
this paper, in the roles described in this section: GPT-5.5-Pro and
GPT-5.6-Sol (OpenAI) as the reasoning model, and Claude Opus and Claude
Fable~5 (Anthropic) as the coding agent. AI assistance was also used in
preparing parts of this manuscript. All results stated as theorems have been
verified by the authors independently of these systems, and the account of
the run given in this section reflects the authors' own reading of the
record. The authors take full responsibility for the contents of this
paper.



==> paper/asymptotic_scheme.tex <==
\section{The Cubic--Quintic Scheme}
\label{sec:scheme}

The previous section lets us work directly with fixed-dimensional limiting
Krivine schemes. We now define the two-dimensional scheme used for our upper
bound. Its first coordinate combines the correlation powers \(t,t^3,t^5\),
while its second coordinate keeps correlation \(t\). In the next two sections,
we compute its correlation function and certify its inverse majorant.

We first describe the general form of the construction. Let
\(D\subseteq\{3,5,7,\ldots\}\) be finite, choose weights
\((s_d)_{d\in D}\), and set
\[
    \sigma_d=(-1)^{(d-1)/2},
    \qquad
    V_D=1+\sum_{d\in D}s_d^2.
\]
A degree-\(d\) Hermite direction contributes the correlation \(t^d\).
After combining these directions into one normalized Gaussian coordinate,
the resulting correlation map is
\begin{equation}
    \rho_D(t)
    =
    \frac{t+\sum_{d\in D}\sigma_d s_d^2 t^d}{V_D}.
    \label{eq:general-hermite-correlation-map}
\end{equation}
The map \(\rho_D\) is allowable, since the absolute values of its
coefficients sum to one. Thus, for any \(\eta\in\mathbb{R}\), the partitions
\[
    \operatorname{sgn}\left(
        w+\frac{\eta}{\sqrt{V_D}}\He_3(x)
    \right)
    \qquad\text{and}\qquad
    \operatorname{sgn}\left(
        w-\frac{\eta}{\sqrt{V_D}}\He_3(x)
    \right)
\]
together with the correlation maps \(\rho_D(t)\) and \(t\) define a
two-dimensional limiting Krivine scheme.

For the scheme used in our proof, we take \(D=\{3,5\}\). The cubic
direction is anti-aligned between the two sides, while the quintic direction
is aligned. We use the parameters
\begin{equation}
    \eta=0.136419125,
    \qquad
    s_3=0.34101124,
    \qquad
    s_5=0.05276111.
    \label{eq:params}
\end{equation}
Set
\[
    V=1+s_3^2+s_5^2,
    \qquad
    \vartheta=\frac{\eta}{\sqrt V},
\]
and define
\begin{equation}
    \rho(t)
    =
    \frac{t-s_3^2t^3+s_5^2t^5}{V}.
    \label{eq:rho-collapsed}
\end{equation}

\begin{definition}[Cubic--quintic limiting scheme]
\label{def:cubic-quintic-scheme}
Define \(f,g:\mathbb{R}^2\to\{-1,1\}\) by
\begin{equation}
    f(w,x)
    =
    \sgn\bigl(w+\vartheta\He_3(x)\bigr),
    \qquad
    g(w,x)
    =
    \sgn\bigl(w-\vartheta\He_3(x)\bigr).
    \label{eq:cubic-quintic-partitions}
\end{equation}
Our construction is the limiting Krivine scheme
\[
    \mathcal{S}=(f,g,\rho_1,\rho_2),
    \qquad
    \rho_1(t)=\rho(t),
    \qquad
    \rho_2(t)=t.
\]
We write \(H\) for its correlation function.
\end{definition}

The map \(\rho\) is allowable because the absolute values of its
coefficients sum to \((1+s_3^2+s_5^2)/V=1\). The partitions are odd and
satisfy \(g(w,x)=f(w,-x)\). Their threshold boundaries also have Gaussian
measure zero, so the approximation theorem from the previous section
applies.

More explicitly, let \((W,X)\) and \((W',X')\) be standard Gaussian vectors.
Assume that the two coordinate pairs are independent and that
\(\operatorname{corr}(W,W')=\rho(t)\) and
\(\operatorname{corr}(X,X')=t\). Then
\begin{equation}
    H(t)
    =
    \frac{\pi}{2}
    \E\bigl[f(W,X)g(W',X')\bigr].
    \label{eq:lim-H}
\end{equation}

The signs and weights in \(\rho\) are chosen to make the cubic and quintic
coefficients of \(H\) nearly vanish. This in turn suppresses the first two
nonlinear coefficients of \(H^{-1}\). Section~\ref{sec:coefficients} makes
this relation explicit.

\begin{theorem}[Cubic--quintic upper bound]
\label{thm:cubic-quintic-upper-bound}
Let \(M\) be the inverse majorant of \(H\). At
\(\gamma=0.881545409\), we have \(M(\gamma)<1\). Consequently,
\[
    K_G
    \leq
    \frac{\pi}{2\gamma}
    \leq
    1.7818666069360661
    <
    \frac{\pi}{2\log(1+\sqrt{2})}
    -
    3.4737\cdot 10^{-4}.
\]
\end{theorem}

==> paper/certification.tex <==
\section{Proof of Cubic-Quintic Scheme}
\label{sec:certification}

Write the correlation function of the cubic--quintic limiting scheme as
\begin{equation}
  H(t)=b_1t+\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}} b_m t^m,
  \label{eq:certification-H-series}
\end{equation}
and let
\begin{equation}
  \Delta_H:=\sum_{\substack{m\ge 3\\ m\ \mathrm{odd}}}|b_m|
  \label{eq:nonlinear-coefficient-mass}
\end{equation}
be the total mass of its nonlinear coefficients.  Let
\[
  G(z)=H^{-1}(z)=\sum_{n\ge1}a_nz^n
\]
denote the local holomorphic inverse of $H$ at the origin, and define its
majorant by
\begin{equation}
  \mathcal M(r):=\sum_{n\ge1}|a_n|r^n.
  \label{eq:inverse-majorant-certification}
\end{equation}
The local inverse exists because $H'(0)=b_1>0$, by the holomorphic inverse
function theorem.

For the linear map $t\mapsto b_1t$, the condition $\mathcal M(\gamma)<1$ is
simply $\gamma<b_1$.  The next proposition shows that the nonlinear part costs
at most $\Delta_H$ of this margin.

\begin{proposition}[Inverse certificate from near-linearity]
\label{prop:inverse-certificate-near-linearity}
Assume $b_1>0$ and $\Delta_H<\infty$.  If
\begin{equation}
  \gamma+\Delta_H<b_1,
  \label{eq:near-linearity-condition}
\end{equation}
then there exists $R>\gamma$ such that the local inverse $G$ extends
holomorphically to $R\mathbb D$, maps $R\mathbb D$ into $\mathbb D$, and
satisfies
\begin{equation}
  \mathcal M(\gamma)
  \le \frac{\gamma+\Delta_H}{b_1}
  <1.
  \label{eq:near-linearity-conclusion}
\end{equation}
\end{proposition}

\begin{proof}
Set
\[
  E(t):=\sum_{m\ge3}b_mt^m,
  \qquad
  E_{\mathrm{maj}}(u):=\sum_{m\ge3}|b_m|u^m.
\]
There is a unique formal power series
\[
  V(z)=\sum_{n\ge1}v_nz^n
\]
satisfying
\begin{equation}
  b_1V(z)=z+E_{\mathrm{maj}}(V(z)).
  \label{eq:majorizing-inverse-equation}
\end{equation}
Indeed, comparison of the coefficient of $z$ gives $v_1=b_1^{-1}$.  For
$n\ge2$, the coefficient of $z^n$ in $E_{\mathrm{maj}}(V)$ depends only on
$v_1,\ldots,v_{n-1}$, so \eqref{eq:majorizing-inverse-equation} determines
$v_n$ recursively.  The same recursion shows that $v_n\ge0$ for every $n$.

Comparing coefficients in
\[
  b_1G(z)=z-E(G(z))
\]
and in \eqref{eq:majorizing-inverse-equation}, induction on $n$ gives
\begin{equation}
  |a_n|\le v_n
  \qquad(n\ge1).
  \label{eq:inverse-coefficient-domination}
\end{equation}
Indeed, at degree $n$, every nonlinear composition involves only previously
determined coefficients, and replacing each $b_m$ by $|b_m|$ removes all
possible cancellation.

Choose $R>\gamma$ so close to $\gamma$ that
\[
  q:=\frac{R+\Delta_H}{b_1}<1.
\]
Starting from $V_0(z)=0$, define
\begin{equation}
  V_{k+1}(z):=\frac{z+E_{\mathrm{maj}}(V_k(z))}{b_1}.
  \label{eq:majorizing-inverse-iteration}
\end{equation}
The series $V_k$ have nonnegative coefficients and increase coefficientwise,
meaning that each Taylor coefficient is nondecreasing in $k$.
Moreover, if $V_k(R)\le q$, then $V_k(R)<1$ and
\[
  V_{k+1}(R)
  \le \frac{R+E_{\mathrm{maj}}(1)}{b_1}
  =q.
\]
Thus $V_k(R)\le q$ for every $k$.  Their coefficientwise limit satisfies
\eqref{eq:majorizing-inverse-equation}, and hence equals $V$ by uniqueness.
The monotone convergence theorem now gives
\[
  V(R)=\sum_{n\ge1}v_nR^n\le q<1.
\]
Together with \eqref{eq:inverse-coefficient-domination}, this implies
\[
  \sum_{n\ge1}|a_n|R^n\le V(R)<1.
\]
Consequently, the Taylor series of $G$ converges on $R\mathbb D$ and takes
values in $\mathbb D$.  Since the identity $H(G(z))=z$ holds near the origin,
it holds throughout $R\mathbb D$ by the identity theorem.  Finally,
\[
  \mathcal M(\gamma)
  \le V(\gamma)
  =\frac{\gamma+E_{\mathrm{maj}}(V(\gamma))}{b_1}
  \le\frac{\gamma+\Delta_H}{b_1},
\]
because $0\le V(\gamma)\le V(R)<1$.
\end{proof}

It remains to certify $\Delta_H$.  We compute the coefficients through a
finite degree $N$ and bound the remaining tail indirectly.  The point is that
the Euler operator
\[
  D:=t\frac{d}{dt}
\]
multiplies the coefficient of $t^m$ by $m$, so $D^3$ strongly amplifies
high-degree coefficients.  The $L^2(\mathbb T)$ norm below is the
root-mean-square size of the resulting function around the unit circle
$\mathbb T:=\{z\in\mathbb C:|z|=1\}$.

\begin{lemma}[Third-order coefficient-tail bound]
\label{lem:third-order-tail}
Suppose that $D^3H$ has radial boundary values in $L^2(\mathbb T)$, with
\[
  \|D^3H\|_{L^2(\mathbb T)}^2
  :=\frac{1}{2\pi}\int_0^{2\pi}
  |D^3H(e^{i\theta})|^2\,d\theta.
\]
Then, for every odd $N$,
\begin{equation}
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
  \le
  \|D^3H\|_{L^2(\mathbb T)}
  \left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}
  \le
  \frac{\|D^3H\|_{L^2(\mathbb T)}}{\sqrt{10N^5}}.
  \label{eq:third-order-tail}
\end{equation}
\end{lemma}

\begin{proof}
Since $D^3(t^m)=m^3t^m$, Parseval's identity gives
\begin{equation}
  \|D^3H\|_{L^2(\mathbb T)}^2
  =\sum_{\substack{m\ge1\\m\ \mathrm{odd}}}m^6|b_m|^2.
  \label{eq:parseval-third-order}
\end{equation}
The Cauchy--Schwarz inequality therefore gives
\[
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}|b_m|
  =\sum_{\substack{m>N\\m\ \mathrm{odd}}}
  m^{-3}\bigl(m^3|b_m|\bigr)
  \le
  \left(\sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}\right)^{1/2}
  \|D^3H\|_{L^2(\mathbb T)}.
\]
Finally, since $x\mapsto x^{-6}$ is decreasing and consecutive odd integers
are separated by two, the monotone integral estimate gives
\[
  \sum_{\substack{m>N\\m\ \mathrm{odd}}}m^{-6}
  \le\frac12\int_N^\infty x^{-6}\,dx
  =\frac{1}{10N^5}.
\]
\end{proof}

\begin{proposition}[Certified numerical input]
\label{prop:certified-numerical-input}
For the cubic--quintic correlation function, interval arithmetic certifies
\begin{equation}
  b_1\ge0.881573822049,
  \qquad
  \sum_{\substack{3\le m\le251\\m\ \mathrm{odd}}}|b_m|
  \le1.1328860\cdot10^{-5},
  \qquad
  \|D^3H\|_{L^2(\mathbb T)}<14.443.
  \label{eq:certified-numerical-input}
\end{equation}
\end{proposition}

\begin{proof}
See Appendix~\ref{app:certification-details}.
\end{proof}

Lemma~\ref{lem:third-order-tail} and
Proposition~\ref{prop:certified-numerical-input} give
\begin{equation}
  \Delta_H
  \le
  1.1328860\cdot10^{-5}
  +\frac{14.443}{\sqrt{10\cdot251^5}}
  <1.5904724\cdot10^{-5}.
  \label{eq:certified-nonlinear-mass}
\end{equation}

\begin{theorem}[Cubic--quintic upper bound]
\label{thm:cubic-quintic-upper-bound-certified}
For
\[
  \gamma=0.881545409,
\]
the cubic--quintic limiting scheme satisfies $\mathcal M(\gamma)<1$.
Consequently,
\begin{equation}
  K_G\le\frac{\pi}{2\gamma}
  \le1.7818666069360661.
  \label{eq:certified-KG-bound}
\end{equation}
\end{theorem}

\begin{proof}
By \eqref{eq:certified-nonlinear-mass},
\[
  \gamma+\Delta_H
  <0.881545409+1.5904724\cdot10^{-5}
   =0.881561313724
   <0.881573822049
   \le b_1
\]
Proposition~\ref{prop:inverse-certificate-near-linearity} therefore gives
$\mathcal M(\gamma)<1$, together with the analytic room required by the
finite-dimensional transfer theorem.  That theorem passes the strict
certificate to all sufficiently large ordinary finite-dimensional
approximations.  The classical Krivine preprocessing theorem then gives
\eqref{eq:certified-KG-bound}.
\end{proof}


\paragraph{Reproducibility.}
  The scripts, certificates, and Arb outputs
  are available at \url{https://github.com/trishullab/grothendieck-bounds}. 

==> paper/coefficient_formula.tex <==
% Section 6: insert after the construction of the two-dimensional limiting scheme.
% This file assumes the paper's existing macros \E, \He, \sgn, \varphi, and \erf.

\section{The Correlation Coefficients}
\label{sec:coefficients}

The previous section defined our two-dimensional limiting scheme, whose two
correlation maps are \(\rho(t)\) and \(t\). We now compute its correlation
function
\[
  H(t)=\sum_{m\geq 1} b_m t^m.
\]
The key observation is that \(g(w,x)=f(w,-x)\). Thus, the Hermite
coefficients of \(f\) determine the entire series \(H\).

We use standard facts about Hermite polynomials. See  \cite{Andrews_Askey_Roy_1999} for a reference.  

Let $\mu$ be the standard Gaussian measure on $\R$, so that
\[
    d\mu(x):=\frac{1}{\sqrt{2\pi}}e^{-x^2/2}\,dx.
\]
Let \(\HermBasis_n\) denote the \(n\)-th orthonormal probabilist's Hermite polynomial. Then \(\{\HermBasis_n\}_{n\ge0}\) is an orthonormal basis for \(L^2(\mu)\).

Let \(W,X\) be independent standard Gaussians. For \(a,b\geq 0\), write
\begin{equation}
  \mathsf A_{a,b}
  =
  \E\!\left[
    f(W,X)\He_a(W)\He_b(X)
  \right].
  \label{eq:mathsfAab}
\end{equation}
Then, in \(L_2\) of the standard Gaussian measure on \(\mathbb{R}^2\),
\[
  f(w,x)
  =
  \sum_{a,b\geq 0}
  \mathsf A_{a,b}\He_a(w)\He_b(x).
\]
Since \(f(-w,-x)=-f(w,x)\), we have \(\mathsf A_{a,b}=0\) whenever
\(a+b\) is even. For a power series \(P\), we write \([t^m]P(t)\) for the
coefficient of \(t^m\).

\begin{theorem}[Coefficient formula]
\label{thm:coefficient-formula}
For every \(t\in(-1,1)\),
\begin{equation}
  H(t)
  =
  \frac{\pi}{2}
  \sum_{a,b\geq 0}
  \mathsf A_{a,b}^2\rho(t)^a(-t)^b.
  \label{eq:H-coefficient-formula}
\end{equation}
Consequently, for every \(m\geq 1\),
\begin{equation}
  b_m
  =
  \frac{\pi}{2}
  \sum_{\substack{a,b\geq 0\\a+b\leq m}}
  (-1)^b\mathsf A_{a,b}^2
  [t^{m-b}]\rho(t)^a.
  \label{eq:bm-coefficient-formula}
\end{equation}
In particular, \(b_m=0\) whenever \(m\) is even.
\end{theorem}

\begin{proof}
Let \((W,X)\) and \((W',X')\) be the Gaussian inputs used to define the
correlation function of the scheme. Thus, \(W\) and \(W'\) have correlation
\(\rho(t)\), while \(X\) and \(X'\) have correlation \(t\); the two
coordinate pairs are independent.

Since \(g(w,x)=f(w,-x)\), the Hermite expansion of \(g\) is
\[
  g(w,x)
  =
  \sum_{a,b\geq 0}
  (-1)^b\mathsf A_{a,b}\He_a(w)\He_b(x).
\]
When the two expansions are substituted into the definition of \(H\),
orthogonality leaves only matching Hermite degrees. The Hermite covariance
identity then contributes \(\rho(t)^a\) in the first coordinate and \(t^b\)
in the second. This gives \eqref{eq:H-coefficient-formula}. The series is
absolutely convergent for \(t\in(-1,1)\), since \(f\in L_2\) and
\(|\rho(t)|\leq |t|<1\).

Extracting the coefficient of \(t^m\) gives
\eqref{eq:bm-coefficient-formula}. Finally, \(\rho\) is odd and
\(\mathsf A_{a,b}\) vanishes unless \(a+b\) is odd. Hence every nonzero
summand in \eqref{eq:H-coefficient-formula} is odd in \(t\), so only odd
coefficients occur.
\end{proof}

\paragraph{Computing the Hermite coefficients.}
The coefficients in \eqref{eq:mathsfAab} reduce to
one-dimensional Gaussian integrals. Let \(Z\) be a standard Gaussian and,
for \(a\geq 0\), set
\begin{equation}
  q_a(u)
  =
  \E\!\left[\sgn(Z+u)\He_a(Z)\right].
  \label{eq:threshold-hermite-coefficients}
\end{equation}
Conditioning on \(X\) gives
\begin{equation}
  \mathsf A_{a,b}
  =
  \E\!\left[
    \He_b(X)q_a\!\left(\vartheta\He_3(X)\right)
  \right].
  \label{eq:f-coefficients-one-dimensional}
\end{equation}
The threshold coefficients have the closed form
\begin{equation}
  q_0(u)
  =
  \erf\!\left(\frac{u}{\sqrt{2}}\right),
  \qquad
  q_a(u)
  =
  \frac{2\varphi(u)}{\sqrt{a}}\He_{a-1}(-u)
  \quad (a\geq 1),
  \label{eq:threshold-hermite-closed-form}
\end{equation}
where \(\varphi(u)=(2\pi)^{-1/2}e^{-u^2/2}\). This standard identity follows
by one integration by parts; we include the proof in
Appendix~\ref{app:coefficient-formulas}.

Theorem~\ref{thm:coefficient-formula} therefore reduces each \(b_m\) to
finite coefficient extraction from powers of \(\rho\) and one-dimensional
Gaussian integrals. This is the formula used to compute the coefficient head
in the next section. A more general formula for schemes built from an
arbitrary finite set of Hermite degrees is recorded in
Appendix~\ref{app:coefficient-formulas}; it is not needed for the main
argument.



==> paper/conclusion.tex <==
\section{Conclusion}

==> paper/discussion_future_directions.tex <==
\section{Discussion and Future Directions}
\label{sec:discussion}

This section explains the parameter choices, nearby extensions, and finite-dimensional effectiveness questions.

\subsection{Why degrees three and five}

The low-order inverse relations \eqref{eq:low-inverse} explain the parameter search.  The hyperplane scheme has $H(t)=\arcsin t$, so its inverse $\sin\zeta$ has alternating nonlinear coefficients.  To increase the admissible radius, the first objective is to suppress the cubic inverse obstruction.  An anti-aligned third-chaos average changes $b_3$ in the correct direction.  Once $b_3$ is controlled, the next obstruction is quintic, and an aligned fifth-chaos average gives the next degree of freedom.

The small two-dimensional perturbation $\eta \He_3(X)$ in the base threshold is also important.  A threshold depending only on the linear combination $Z+\sum_ds_dR_d$ would reduce to a hyperplane after rotation.  The $X$-dependent cubic term changes the coefficient integrals $\mathsf A_{a,b}$ and gives the higher coefficients the needed shape.

\subsection{A degree \texorpdfstring{$7/9$}{7/9} extension}

The coefficient formula immediately extends to additional odd degrees.  For instance, taking
\[
  D=\{3,5,7,9\},
  \qquad
  \sigma_d=(-1)^{(d-1)/2},
\]
keeps the same formula \eqref{eq:general-bm}.  A preliminary numerical search gives
\begin{align*}
  \eta&=0.12569605,&
  s_3&=0.34199778,&
  s_5&=0.05153822,\\
  s_7&=0.00698313,&
  s_9&=0.00090252.
\end{align*}
For the corresponding limiting model, the estimated value is
\[
  \gamma\approx0.88157525281,
  \qquad
  \KG\lesssim1.78180628572.
\]
This extension is not used in the main theorem.  It is included to indicate that the third/fifth scheme is not isolated: the same analytic and finite-transfer machinery applies to a broader family of Gaussianized Hermite-chaos averages.

\subsection{Effective dimensions}

Corollary~\ref{cor:finite-scheme} is qualitative: it proves the existence of sufficiently large finite length $N$, but it does not give a useful dimension bound.  For the Grothendieck constant as a mathematical constant, qualitative existence of a finite scheme is enough.  For an explicit algorithmic implementation, one should quantify the convergence $H_N\to H$ on the contour used in Theorem~\ref{thm:finite-transfer}.

The natural route is a collision expansion, by which we mean an expansion separating terms with distinct indices from terms in which some indices repeat.  For fixed degree $d$ and fixed $k$, the polynomial $\He_k(P_{d,N})$ has a leading distinct-index component
\[
  \sqrt{k!}\,N^{-k/2}
  \sum_{1\le i_1<\cdots<i_k\le N}
  \He_d(U_{d,i_1})\cdots \He_d(U_{d,i_k}),
\]
which is homogeneous of total Hermite degree $dk$ and has $L^2$-norm squared $(N)_k/N^k\to1$.  The remaining collision terms have vanishing $L^2$ mass for fixed $d,k$.  This explains at the coefficient level why a limiting Hermite mode of order $k$ contributes correlation power $t^{dk}$.  Making this expansion uniform to the required degree would produce explicit finite-dimensional estimates.


==> paper/finite_dim_realization.tex <==
\section{Finite-Dimensional Realization}
\label{sec:transfer}

This section is proves that finite schemes approximate the limiting $b$-series.  Coefficientwise convergence is true, but it is not strong enough to transfer the inverse-majorant condition, which is an infinite nonlinear condition on the inverse series.  We prove a stronger analytic statement.

\subsection{Locally uniform convergence of finite correlations}

Let $H_N$ denote the arcsine-normalized correlation function of the finite scheme $(f_N,g_N)$, in the standard-normal coordinates of Section~\ref{sec:scheme}:
\[
  H_N(t)={\pi\over2}\E[f_N(\calX)g_N(\calY_t)].
\]
Here $\calX,\calY_t\in\R^{2+|D|N}$ are standard Gaussian vectors with $\E[\calX_i\calY_{t,i}]=t$ coordinatewise.

\begin{proposition}[Local uniform convergence]\label{prop:loc-unif}
The functions $H_N$ extend holomorphically to $\D$, satisfy $|H_N(z)|\le\pi/2$ on $\D$, and converge locally uniformly on $\D$ to the limiting correlation $H$.  Consequently, if
\[
  H_N(z)=\sum_{m\ge1}b_{m,N}z^m,
  \qquad
  H(z)=\sum_{m\ge1}b_mz^m,
\]
then $b_{m,N}\to b_m$ for every fixed $m$.
\end{proposition}

\begin{proof}
For fixed $N$, expand $f_N$ and $g_N$ in the orthonormal tensor Hermite basis on $\R^{2+|D|N}$:
\[
  f_N=\sum_\alpha \widehat f_N(\alpha)\He_\alpha,
  \qquad
  g_N=\sum_\alpha \widehat g_N(\alpha)\He_\alpha.
\]
Mehler's formula gives, for real $t\in(-1,1)$,
\[
  {2\over\pi}H_N(t)=\sum_\alpha \widehat f_N(\alpha)\widehat g_N(\alpha)t^{|\alpha|}.
\]
The same series is absolutely convergent for $|z|<1$, since Cauchy-Schwarz gives
\begin{align*}
  \sum_\alpha |\widehat f_N(\alpha)\widehat g_N(\alpha)| |z|^{|\alpha|}
  &\le
  \left(\sum_\alpha |\widehat f_N(\alpha)|^2 |z|^{|\alpha|}\right)^{1/2}
  \left(\sum_\alpha |\widehat g_N(\alpha)|^2 |z|^{|\alpha|}\right)^{1/2}\\
  &\le \|f_N\|_2\|g_N\|_2=1.
\end{align*}
Thus $H_N$ is holomorphic on $\D$ and $|H_N(z)|\le \pi/2$.

We next identify the pointwise limit on the real interval.  Fix $t\in(-1,1)$.  For every degree $d\in D$, the Hermite covariance identity gives
\[
  \E[\He_d(U_{d,j})\He_d(U_{d,j}')]=t^d.
\]
The multivariate central limit theorem yields
\[
  \bigl(P_{d,N},P_{d,N}'\bigr)_{d\in D}
  \Rightarrow
  \bigl(R_d,R_d'\bigr)_{d\in D},
\]
where $(R_d,R_d')$ is a Gaussian pair with correlation $t^d$, and the pairs are independent over distinct $d$.  This convergence is joint with $(Z,Z',X,X')$, which are independent of the Hermite averages.

The limiting discontinuity set of the product of signs is contained in the union of the two threshold hypersurfaces
\begin{align*}
  z+\eta \He_3(x)+\sum_{d\in D}s_dr_d&=0,\\
  z'-\eta \He_3(x')+\sum_{d\in D}\sigma_ds_dr_d'&=0.
\end{align*}
This union has limiting probability zero: after conditioning on all variables except $Z$, the first threshold has probability zero because $Z$ has a density, and similarly for the second threshold using $Z'$.  The bounded continuous mapping theorem therefore gives $H_N(t)\to H(t)$ for every real $t\in(-1,1)$.

The family $\{H_N\}$ is locally bounded on $\D$ and converges pointwise on a set with an accumulation point.  Vitali's theorem gives locally uniform convergence on $\D$ to the unique holomorphic function agreeing with the real limiting correlation.  Coefficient convergence follows from Cauchy's formula.
\end{proof}

\begin{remark}
Proposition~\ref{prop:loc-unif} justifies the limiting coefficient formula as the fixed-degree limit of genuine finite-dimensional schemes.  But it does not by itself imply that the finite inverse series satisfy $\sum_n|A_{n,N}|\gamma^n\le1$.  Tail control for the inverse series requires the inverse-branch stability theorem below.
\end{remark}

\subsection{Analytic stability of inverse branches}

\begin{theorem}[Finite inverse-majorant transfer]\label{thm:finite-transfer}
Let $F_N,F\in\Hol(\D)$, assume $F_N\to F$ locally uniformly on $\D$, and assume $F_N(0)=F(0)=0$.  Suppose that $G$ is a holomorphic inverse branch of $F$ on a neighborhood of $\ol{D(0,R_0)}$, with values in $\D$:
\[
  F(G(\zeta))=\zeta,
  \qquad |\zeta|\le R_0.
\]
Write
\[
  G(\zeta)=\sum_{n\ge1}A_n\zeta^n.
\]
Let $0<\gamma<R_0$, and assume the strict majorant inequality
\[
  \sum_{n\ge1}|A_n|\gamma^n<1.
\]
Then, for all sufficiently large $N$, $F_N$ has a holomorphic inverse branch at the origin,
\[
  G_N(\zeta)=F_N^{-1}(\zeta)=\sum_{n\ge1}A_{n,N}\zeta^n,
\]
defined on a neighborhood of $\gamma\ol\D$, and
\[
  \sum_{n\ge1}|A_{n,N}|\gamma^n<1.
\]
Moreover $A_{n,N}\to A_n$ for every fixed $n$.
\end{theorem}

\begin{proof}
Choose nested radii
\[
  \gamma<\rho<r<R<R_0.
\]
Let
\[
  \Omega=G(D(0,R)).
\]
Since $G$ is a conformal inverse branch on a neighborhood of $\ol{D(0,R)}$, the boundary $\partial\Omega$ is the image of $|\zeta|=R$.  For $t\in\partial\Omega$, we have $|F(t)|=R$.  Therefore, for all $|\zeta|\le r$,
\[
  |F(t)-\zeta|\ge R-r,
  \qquad t\in\partial\Omega.
\]
The compact contour $\partial\Omega$ is contained in $\D$.  By locally uniform convergence, for all large $N$,
\[
  \sup_{t\in\partial\Omega}|F_N(t)-F(t)|<R-r.
\]
Rouche's theorem then implies that, for every $|\zeta|\le r$, the equations $F_N(t)=\zeta$ and $F(t)=\zeta$ have the same number of solutions in $\Omega$, counted with multiplicity.  The equation $F(t)=\zeta$ has exactly one solution in $\Omega$, namely $t=G(\zeta)$.  Hence $F_N(t)=\zeta$ also has exactly one solution in $\Omega$.  In particular, since $F_N(0)=0$, the zero at $0$ is simple, and these solutions define a holomorphic inverse branch $G_N$ on $D(0,r)$, with values in $\Omega$.

The inverse branches converge uniformly on $\ol{D(0,r)}$.  Indeed, by the argument-principle formula,
\[
  G_N(\zeta)= {1\over 2\pi i}\int_{\partial\Omega}
  {tF_N'(t)\over F_N(t)-\zeta}\,dt,
  \qquad |\zeta|\le r.
\]
The denominators are uniformly bounded away from zero on $\partial\Omega\times\ol{D(0,r)}$, and $F_N'\to F'$ uniformly on $\partial\Omega$.  Thus $G_N\to G$ uniformly on $\ol{D(0,r)}$, which implies fixed inverse-coefficient convergence.

It remains to control the tail.  Put
\[
  B=\sup_{t\in\ol\Omega}|t|<\infty.
\]
Since $G_N(D(0,r))\subseteq\Omega$, Cauchy's estimate on the circle $|\zeta|=\rho$ gives
\[
  |A_{n,N}|\le B\rho^{-n},
  \qquad n\ge1,
\]
for all large $N$.  Let
\[
  \delta=1-\sum_{n\ge1}|A_n|\gamma^n>0.
\]
Choose $M$ so large that
\[
  B\sum_{n>M}\left({\gamma\over\rho}\right)^n< {\delta\over3}.
\]
For all sufficiently large $N$, fixed-coefficient convergence gives
\[
  \sum_{n\le M}|A_{n,N}|\gamma^n
  \le \sum_{n\le M}|A_n|\gamma^n+{\delta\over3}.
\]
Therefore
\begin{align*}
  \sum_{n\ge1}|A_{n,N}|\gamma^n
  &\le \sum_{n\le M}|A_n|\gamma^n+{\delta\over3}
  +B\sum_{n>M}\left({\gamma\over\rho}\right)^n\\
  &< \sum_{n\ge1}|A_n|\gamma^n+{2\delta\over3}<1.
\end{align*}
\end{proof}

\begin{corollary}[Finite schemes from a limiting certificate]\label{cor:finite-scheme}
Assume the limiting correlation $H$ has a holomorphic inverse branch
\[
  G(\zeta)=H^{-1}(\zeta)=\sum_{n\ge1}A_n\zeta^n
\]
with values in $\D$ on a neighborhood of $\ol{D(0,R_0)}$.  Let $0<\gamma<R_0$, and suppose
\[
  \sum_{n\ge1}|A_n|\gamma^n<1.
\]
Then, for all sufficiently large lengths $N$, the genuine finite-dimensional scheme $(f_N,g_N)$ satisfies the inverse-majorant condition at radius $\gamma$.  Consequently
\[
  \KG\le {\pi\over2\gamma}.
\]
\end{corollary}

\begin{proof}
Apply Proposition~\ref{prop:loc-unif} and Theorem~\ref{thm:finite-transfer} with $F_N=H_N$ and $F=H$, then invoke Theorem~\ref{thm:krivine-criterion} for the finite scheme after the scaling convention stated at the start of Section~\ref{sec:scheme}.
\end{proof}

\begin{corollary}[Endpoint and margin]\label{cor:margin}
If the limiting inverse branch is holomorphic with values in $\D$ on a neighborhood of $\Gamma\ol\D$ and
\[
  \sum_{n\ge1}|A_n|\Gamma^n\le1,
\]
then every $\gamma<\Gamma$ transfers to all sufficiently high finite-dimensional schemes.  If the inequality at $\Gamma$ is strict and the same analytic neighborhood is available, then $\Gamma$ itself transfers.
\end{corollary}

\begin{proof}
For $\gamma<\Gamma$, the majorant is strict because $A_1\neq0$:
\[
  \sum_{n\ge1}|A_n|\gamma^n<\sum_{n\ge1}|A_n|\Gamma^n\le1.
\]
Apply Corollary~\ref{cor:finite-scheme}.  The strict endpoint case is the same argument with $\gamma=\Gamma$.
\end{proof}


==> paper/introduction.tex <==


% \subsection{Main Points}
% \begin{itemize}
%     \item Krivine's rounding scheme involves $f,g:\R^k \rightarrow \{1,-1\}$ for some $k$ and we look at $E[f(X) g(Y)]$ where the coordiantes of $X, Y$ are (a) Independent, standard Gaussian and (b) are $t$-correlated.

%     \item The key observation now is that we can study functions $f,g:\R^k \rightarrow \{1,-1\}$, where the coordinates are
%     (a) Independent, standard Gaussian and
%     (b) $X_i, Y_i$ are $p_i(t)$-correlated for any $p_i :\R \to \R$ that are mean $0$ polynomials with variance $1$. 

%     The idea for this is to replace each $X_i$ as $(1/\sqrt{N})\sum_{j=1}^N p_i(X_{i,j})$ where $X_{i,j}$ are independent $N(0,1)$ variables. If we do the same for $Y_i = (1/\sqrt{N})\sum_{j=1}^N p_i(Y_{i,j})$, then $\E[X_i Y_i] = p_i(t)$. Further, in the limit, by the central limit theorem, $X_i, Y_i$ approach $N(0,1)$. 

%     \item One way to use it is now is to consider rounding schemes of the form $f(X) = \sign(P(X))$, where $P(X) = \sum_i q_i(X_i)$ (make sure $P$ is odd still). We can choose a few of the correlations, for example say $X_3, X_4$ so that they cancel out some terms coming from the first two. 
%     \item Concretely, for instance we can take $P(X_1,X_2,X_3,X_4) = X_1 + \eta \He_3(X_2) + s_3 X_3 + s_4 X_4$, where the correlation between $X_3, Y_3$ is $t^3$, and correlation between $X_4, Y_4$ is $t^5$. A form of this gives a bound like $3.4 \times 10^{-4}$. 
%     \item We now have a different search space: choose the correlations $p_i(t)$ in a way to cancel out the lower-order terms or even try other things and do similar computations as before. 
% \end{itemize}

% \subsection{Paper structure}


\section{Introduction}

The Grothendieck inequality~\cite{Gro53,LP68} states that there exists a universal constant $K<\infty$ such that for every $m,n\in\N$ and every matrix $A=(a_{ij})\in\R^{m\times n}$,
\begin{equation}\label{eq:grothendieck-ineq}
  \max_{\eps_i,\delta_j\in\{\pm1\}}
  \left|\sum_{i=1}^m\sum_{j=1}^n a_{ij}\eps_i\delta_j\right|
  \le
  \sup_{u_i,v_j\in S^{m+n-1}}
  \left|\sum_{i=1}^m\sum_{j=1}^n a_{ij}\ip{u_i}{v_j}\right|
  \le
  K\max_{\eps_i,\delta_j\in\{\pm1\}}
  \left|\sum_{i=1}^m\sum_{j=1}^n a_{ij}\eps_i\delta_j\right|.
\end{equation}
Here $S^{m+n-1}$ denotes the unit sphere in $\R^{m+n}$.  The Grothendieck constant $\KG$ is the infimum of $K$ for which this inequality holds.

The inequality is equivalent to the statement that the integrality gap of the canonical semidefinite relaxation for maximizing the bilinear form $x^\top Ay$ over $x\in\{-1,1\}^m$ and $y\in\{-1,1\}^n$ is bounded by an absolute constant.
This connection leads to efficient algorithms for approximating combinatorial problems, such as matrix cut norms~\cite{AN06}.  Beyond this algorithmic role, Grothendieck's inequality is central in the geometry of Banach spaces, operator spaces, harmonic analysis, and quantum information; see, for example, the surveys and monographs~\cite{KN11,pisier2011grothendieckstheorempastpresent,DFS08}.

However, the exact value of $\KG$ is still unknown.
% On the lower bound, one seeks matrices for which the vector optimum is large relative to the sign optimum.
On the lower bound, existing strategies aim to construct matrices for which the vector optimum is large relative to the sign optimum.
While Grothendieck's original work implies that $\KG \geq \pi/2$~\cite{Gro53}, this was substantially improved by Davie~\cite{Davie1984LowerBoundKG} and Reeds~\cite{Reeds1991LowerBoundKG}, who independently used a high-dimensional Gaussian-operator construction to prove
\[
\KG
\geq K_{\mathrm{DR}} = 1.6769\ldots
\]
The Davie--Reeds inequality was the best-known result for more than four decades, until two recent works by
Heilman~\cite{heilman2026lowerboundgrothendiecksconstant} and Jones and Malavolta~\cite{jones2026grothendieckconstantstrictlylarger} independently showed that $\KG \geq K_{\mathrm{DR}}+10^{-26}$
and $\KG \geq K_{\mathrm{DR}}+10^{-12}$, respectively.


% Broadly speaking, lower-bound approaches involve constructing matrices for which the vector optimum is large relative to the sign optimum.


% Heilman proved $\KG \geq K_{\mathrm{DR}}+10^{-26}$ ~\cite{heilman2026lowerboundgrothendiecksconstant}, while Jones and Malavolta proved $\KG \geq K_{\mathrm{DR}}+10^{-12}$~\cite{jones2026grothendieckconstantstrictlylarger}.


% Heilman 
% Heilman

% Two recent works established that it is not optimal: Heilman proved $\KG \geq K_{\mathrm{DR}}+10^{-26}$ ~\cite{heilman2026lowerboundgrothendiecksconstant}, while Jones and Malavolta proved $\KG \geq K_{\mathrm{DR}}+10^{-12}$~\cite{jones2026grothendieckconstantstrictlylarger}.



On the upper bound, Krivine's seminal result~\cite{Kri77} proved that
\begin{equation}\label{eq:krivine-bound-intro}
  \KG\le {\pi\over 2\log(1+\sqrt2)}=1.7822\ldots
\end{equation}
The proof is constructive: it gives a rounding scheme that maps input vectors $u_i,v_j$ to signs $\eps_i,\delta_j\in\{\pm1\}$ after an infinite-dimensional preprocessing step and a random hyperplane rounding step.
Krivine also conjectured that this bound was tight, and this stood for over three decades until it was disproven by Braverman, Makarychev, Makarychev, and Naor in 2011; specifically, they ``mixed'' the hyperplane rounding scheme with a non-hyperplane one to establish the strict inequality $\KG < \tfrac{\pi}{2\log(1+\sqrt2)}$~\cite{braverman2011grothendieckconstantstrictlysmaller}.
Interestingly, however, Naor and Regev subsequently showed that mixed Krivine schemes (\cref{sec:krivine-rounding-scheme}) are in fact optimal: in the limit of dimension, there exists such a scheme that yields arbitrarily good approximations of $K_G$~\cite{naor2014krivine}.
This thus opened a strategy for attacking the strict inequality's unspecified numerical gap, and was leveraged in recent works by Heilman~\cite{heilman2026upperboundgrothendiecksconstant} and Li et al.~\cite{LiSahaXueChaudhuriKlivansKothariMeka2026} to independently arrive at explicit numerical improvements on the order of $10^{-5}$.


% Interestingly, however, Naor and Regev subsequently showed that such ``Krivine schemes'' (\cref{sec:krivine-rounding-scheme}) are, in fact, optimal: in the limit of dimension, oblivious Krivine schemes yield arbitrarily good approximations of $K_G$~\cite{naor2014krivine}.
% Based on these developments, recent works by Heilman~\cite{heilman2026upperboundgrothendiecksconstant} and Li et al.~\cite{LiSahaXueChaudhuriKlivansKothariMeka2026} independently gave the first explicit numerical improvement of order $10^{-5}$.

% using a certified computer-assisted implementation of related Krivine preprocessing ideas. 



% Krivine further conjectured this bound to be optimal, and this stood for over three decades until its disproof by Braverman, Makarychev, Makarychev, and Naor, who showed that it is, in fact, strict, by mixing the hyperplane scheme with a non-hyperplane two-dimensional rounding scheme~\cite{braverman2011grothendieckconstantstrictlysmaller}.

% Braverman, Makarychev, Makarychev, and Naor later disproved Krivine's conjectured optimality of \eqref{eq:krivine-bound-intro}, proving that $\KG<\pi/(2\log(1+\sqrt2))$ by mixing the hyperplane scheme with a non-hyperplane two-dimensional rounding scheme~\cite{braverman2011grothendieckconstantstrictlysmaller}.


% Naor and Regev showed that Krivine schemes are optimal, where in the limit of dimension oblivious Krivine schemes yield arbitrarily good approximations of $K_G$~\cite{naor2014krivine}.

% Krivine also conjectured that this bound was optimal. This conjecture stood for over three decades, until Braverman, Makarychev, Makarychev, and Naor disproved it by mixing the hyperplane scheme with a non-hyperplane scheme~\cite{braverman2011grothendieckconstantstrictlysmaller}.
% Specifically, they used this mixed rounding scheme to establish the strict inequality
% $\KG< \tfrac{\pi}{2\log(1+\sqrt2)}$, but did not quantify the gap.
% Krivine also conjectured that this bound was optimal, a conjecture that stood for over three decades until Braverman, Makarychev, Makarychev, and Naor disproved it by mixing the hyperplane scheme with a non-hyperplane one~\cite{braverman2011grothendieckconstantstrictlysmaller}.


%Our work significantly extends their approach for an upper bound and finds a surprising new approach to improve the lower bounds at the same time. 


\paragraph{This work.}
In this paper, we make the following contribution:
% In this paper, we make two main mathematical contributions:
% In this paper, we make two main mathematical contributions and an AI contribution:
\begin{enumerate}
    \item \textbf{Upper bound.} We introduce \emph{limiting Krivine schemes}, an analytic framework for constructing and studying asymptotic families of increasingly high-dimensional rounding schemes. Using this framework, we construct a new ``cubic--quintic'' scheme that yields
    \[
        % K_G \le 1.7818666069,
        K_G
        \le {\pi\over 2\log(1+\sqrt2)} - 3.47 \times 10^{-4}
        = 1.7818 \ldots.
    \]
    % improving Krivine's classical upper bound by  \(>3.47 \cdot 10^{-4}\).
    This differs from previous works, which only considered one- or two-dimensional rounding schemes, and in particular positively answers a question posed by Braverman et al.~\cite{braverman2011grothendieckconstantstrictlysmaller} about whether increasing dimension can lead to improved bounds on $K_G$.

    \item \textbf{Lower bound.} We find a new approach to proving lower bounds on $K_G$ and show:
    \[
        K_G \ge \frac{6\pi}{11}=1.7135\ldots.
    \]
    Together with our upper bound, this determines the tenths digit of \(K_G\) to be 7.
    Notably, our approach is to show a fundamental limitation of Krivine schemes and then apply a result from Naor and Regev~\cite{naor2014krivine}.
    
    % In particular, unlike all previous work that relied on explicit construction of gap instances, our approach shows a limitation on Krivine schemes, and then invokes the result from Naor and Regev~\cite{naor2014krivine} to prove a lower bound.

    \item \textbf{AI methodology.}
    We further detail our use of AI in mathematics research in a companion paper~\cite{lisaha2026longhorizon}.
    Because mathematics research is a long-horizon task that comprises complex goals, persistent memory, and delayed rewards, it is often unclear how to effectively use AI.
    Our work thus provides an extensive case study on how to develop and interact with emerging AI systems.    
    Critically, this system is also highly collaborative with human interaction, which allows it to effectively explore promising proof strategies.

\end{enumerate}




% Our proof for the upper bound... (say something in one line). The proof combines a universal constraint on the first and third coefficients of Gaussian correlation functions with an optimality result for the inverse-majorant method on Krivine schemes. 

% \paragraph{Technical overview of the Lower Bound}. We prove the following theorem:

% \begin{theorem}\label{thm:lower-bound}
% The Grothendieck constant satisfies
% \[
%         K_G\ge\frac{6\pi}{11} \approx 1.7136.
% \]
% \end{theorem}

% A sketch of the proof is as follows. 

% First, recall the inverse-series step in Krivine's rounding argument. If
% \[
%         H^{-1}(z)=\sum_{j\ge0}a_{2j+1}z^{2j+1},
% \]
% define the absolute-coefficient majorant $M_H(s):=\sum_{j\ge0}|a_{2j+1}|s^{2j+1}$. The standard tensor preprocessing gives the implication
% \begin{equation}
%         M_H(\gamma)\le1
%         \quad\Longrightarrow\quad
%         K_G\le\frac{\pi}{2\gamma}.
%         \label{eq:inverse-majorant-bound}
% \end{equation}
% We refer to~\eqref{eq:inverse-majorant-bound} as the \emph{inverse-majorant bound}.

% The conceptual starting point is the theorem of Naor and Regev that Krivine schemes are optimal \cite{naor2014krivine}. By reworking the construction in their proof, we show that the inverse-majorant bound is itself asymptotically optimal after allowing mixtures and increasing dimension: there are limiting mixed correlation functions with admissible parameters converging to $\pi/(2K_G)$. This transfer is established in Section~\ref{sec:majorant_optimal}.

% It therefore remains to prove a universal upper bound on such admissible parameters. For arbitrary odd measurable sign functions $f,g:\R^d\to\{\pm1\}$, write
% \[
%         H_{f,g}(t)=b_1t+b_3t^3+b_5t^5+\cdots.
% \]
% The technical core of the argument is the affine inequality
% \[
%         b_3\ge 2b_1-\frac{11}{6}.
% \]
% Section~\ref{sec:preliminaries} sets up the Gaussian--Hermite formulation, and Section~\ref{sec:affine-strip} proves this inequality by decomposing $f$ and $g$ into their agreement and disagreement parts and reducing the required estimates to one-dimensional inequalities. Its linearity in $(b_1,b_3)$ is essential, because it makes the inequality invariant under mixtures and coefficientwise limits.

% Section~\ref{sec:strip_majorant} then shows that the affine inequality controls the inverse-majorant bound: every admissible value must satisfy $\gamma\le11/12$. Applying this barrier to the asymptotically optimal sequence constructed in Section~\ref{sec:majorant_optimal} gives
% \[
%         \frac{\pi}{2K_G}\le\frac{11}{12},
% \]
% which is exactly Theorem~\ref{thm:lower-bound}.


% \paragraph{Technical overview of the Upper Bound}. (Give references to sections of the technical part)

% - Recall classical Krivine schemes... (standard correlation)

% - Define Limiting Krivine schemes... (arbitrary correlation)

% - Show that these schemes can be arbitrarily approximated by classical (finite) Krivine schemes, in a specific sense

% - Therefore inverse-majorant bound on Limiting Krivine schemes translates to upper bounds on $K_G$, so this is a new search space

% - We then study a specific instantiation of limiting Krivine schemes: the cubic--quintic scheme...

% - We show how to derive the inverse-majorant bound on this by bounding the tail of the taylor expansion of $H$... 




% This paper studies a different way to build high-dimensional rounding schemes.  The construction starts with \emph{Gaussianized Hermite-chaos averages}, defined formally in Definition~\ref{def:gaussianized-chaos}.  This is our terminology for normalized finite averages of Hermite polynomials that converge to Gaussian coordinates while preserving the covariance powers of the corresponding Wiener chaos.  The underlying standard objects are Hermite polynomials and Wiener chaos; for background, see Janson's treatment of Gaussian Hilbert spaces~\cite{Janson1997GaussianHilbertSpaces}.  The reason these averages are useful is simple: if $(X,Y)$ are standard Gaussians with correlation $t$, then the orthonormal probabilist Hermite polynomials satisfy
% \[
%   \E[\He_m(X)\He_n(Y)]=\delta_{mn}t^n.
% \]
% Thus a degree-$d$ Hermite coordinate contributes a covariance factor $t^d$.  By combining degree $3$ and degree $5$ averages with opposite relative signs, we obtain a limiting correlation function whose cubic and quintic coefficients are nearly zero.  This removes the first two nonlinear obstructions in the inverse-majorant condition used by Krivine preprocessing.

% \subsection{The result}

% % Write
% % \[
% %   \rhohyp:=\log(1+\sqrt2),
% %   \qquad
% %   \Khyp:={\pi\over2\rhohyp}={\pi\over2\log(1+\sqrt2)}.
% % \]
% % The certified radius in this paper is
% % \begin{equation}\label{eq:gamma-main}
% %   \gamma=0.881545409>\rhohyp.
% % \end{equation}
% % This corresponds to the raw correlation value
% % \[
% %   c={2\gamma\over \pi}=0.5612090874\ldots
% % \]
% % and to the Grothendieck bound
% % \[
% %   {1\over c}={\pi\over 2\gamma}=1.7818666069360661\ldots .
% % \]
% % The improvement over the hyperplane/Krivine value is
% % \[
% %   \Khyp-{\pi\over 2\gamma}=3.473712553\cdot10^{-4}\ldots .
% % \]

% \begin{theorem}[Main theorem]\label{thm:main}
% There is a finite-dimensional Krivine rounding family such that
% \[
%   \KG < {\pi\over 2\log(1+\sqrt2)}-3.4737\cdot 10^{-4}.
% \]
% \end{theorem}

% The computation in this draft is rigorous.  The inequalities used in the proof are interval enclosures, organized in Sections~\ref{sec:sobolev-tail}--\ref{sec:assembly}.  The implementation uses Arb, the rigorous interval-arithmetic library of Johansson~\cite{johansson2017arb}.

% \subsection{Overview of the construction}

% For the moment, write $\He_n$ for the orthonormal probabilist Hermite polynomial.  For every length $N$, define
% \[
%   P_{3,N}=N^{-1/2}\sum_{j=1}^N \He_3(U_j),
%   \qquad
%   P_{5,N}=N^{-1/2}\sum_{j=1}^N \He_5(V_j),
% \]
% where the variables are independent standard Gaussians.  The finite rounding pair is
% \begin{align*}
%   f_N &= \sgn\bigl(Z+\eta \He_3(X)+s_3P_{3,N}+s_5P_{5,N}\bigr),\\
%   g_N &= \sgn\bigl(Z-\eta \He_3(X)-s_3P_{3,N}+s_5P_{5,N}\bigr).
% \end{align*}
% Thus degree $3$ is anti-aligned between the two sides, while degree $5$ is aligned.  The relative signs are chosen so that degree $2k+1$ has sign $(-1)^k$.

% For fixed $t\in(-1,1)$, paired inputs with coordinatewise Gaussian correlation $t$ satisfy
% \[
%   \E[P_{3,N}P_{3,N}']=t^3,
%   \qquad
%   \E[P_{5,N}P_{5,N}']=t^5.
% \]
% Hence, as $N\to\infty$, the relevant limiting model is a four-dimensional Gaussian threshold pair
% \begin{align*}
%   f(z,x,r_3,r_5)&=\sgn\bigl(z+\eta \He_3(x)+s_3r_3+s_5r_5\bigr),\\
%   g(z,x,r_3,r_5)&=\sgn\bigl(z-\eta \He_3(x)-s_3r_3+s_5r_5\bigr),
% \end{align*}
% with coordinate correlations
% \[
%   \rho_Z=t,
%   \qquad
%   \rho_X=t,
%   \qquad
%   \rho_3=t^3,
%   \qquad
%   \rho_5=t^5.
% \]
% These powers record the Hermite degrees used in the finite averages: a degree-$d$ Hermite coordinate contributes covariance $t^d$.

% The limiting normalized correlation is an odd series
% \[
%   H(t)=\sum_{m\ge1}b_m t^m.
% \]
% For the displayed parameters, the leading coefficients are certified as
% \[
%   b_1\ge0.8815738220,
%   \qquad b_3=3.4538733\cdot 10^{-9},
%   \qquad b_5=-9.0435536\cdot 10^{-11}.
% \]
% Since the inverse coefficients satisfy
% \[
%   A_1={1\over b_1},\qquad
%   A_3=-{b_3\over b_1^4},\qquad
%   A_5={3b_3^2-b_1b_5\over b_1^7},
% \]
% the near-vanishing of $b_3$ and $b_5$ removes the first two nonlinear inverse obstructions.

% \subsection{Proof architecture}\label{subsec:architecture}

% The proof is organized so that every analytic reduction is separated from the interval-arithmetic estimates.  The headers below match the section titles.

% \paragraph{Section~\ref{sec:krivine}: Krivine Rounding Scheme.}
% This section copies the Krivine-rounding interface from the reference format used in the companion paper~\cite{LiSahaXueChaudhuriKlivansKothariMeka2026}.  It defines the arcsine-normalized Gaussian correlation function, the local inverse, the inverse majorant, and $\gamma$-admissibility.  The proof is deferred to Appendix~\ref{app:preprocessing}.

% \paragraph{Section~\ref{sec:scheme}: The finite Gaussianized Hermite-chaos family.}
% Definitions~\ref{def:Hermite}, \ref{def:gaussianized-chaos}, \ref{def:finite-family}, and~\ref{def:finite-35} define the actual finite-dimensional schemes.  Definition~\ref{def:limiting-model} defines the limiting model, where the covariance powers $t^3$ and $t^5$ record the Hermite degrees in the finite construction.

% \paragraph{Section~\ref{sec:coefficients}: Coefficients of the limiting model.}
% Definitions~\ref{def:degree-normalization}, \ref{def:qk}, and~\ref{def:Cabk} give the general weighted-degree formula for $b_m=[t^m]H(t)$.  The specialized collapsed formula in Proposition~\ref{prop:collapsed-coefficients} is the one used by the certificate.

% \paragraph{Section~\ref{sec:transfer}: Finite-dimensional realization of the limiting certificate.}
% This is the delicate analytic transfer step.  Proposition~\ref{prop:loc-unif} proves locally uniform convergence $H_N\to H$ on the unit disk.  Theorem~\ref{thm:finite-transfer} then transfers a strict inverse-majorant certificate from $H$ to $H_N$ using Rouche's theorem and Cauchy estimates.  Fixed-degree coefficient convergence alone would not control the inverse tail.

% \paragraph{Section~\ref{sec:wiener}: A Wiener-algebra certificate for the limiting inverse.}
% Definition~\ref{def:wiener-data} introduces the Wiener-algebra quantities used to control the inverse.  Theorem~\ref{thm:simple-wiener} proves that it is enough to show $\gamma+\eta_0<b_1$ and $\eta_1<b_1$ for the nonlinear masses $\eta_0=\sum_{m\ge3}|b_m|$ and $\eta_1=\sum_{m\ge3}m|b_m|$.

% \paragraph{Section~\ref{sec:sobolev-tail}: The coefficient tail through a Sobolev norm.}
% The tail of $\eta_0$ and $\eta_1$ is reduced to the single scalar norm $B_3=\norm{\Dop^3H}_{L^2(\T)}$ by Cauchy-Schwarz.

% \paragraph{Section~\ref{sec:sobolev-norm}: Bounding the Sobolev norm.}
% The norm $B_3$ is bounded by representing $\Dop^3H$ as a trace of a two-dimensional differential kernel and applying an averaged Minkowski inequality before the certified circle quadrature.

% \paragraph{Section~\ref{sec:assembly}: Assembling the certificate and proving the main theorem.}
% This section combines the certified head sums, the Sobolev tail, and the Wiener criterion to prove limiting admissibility at $\gamma=0.881545409$.  The finite-transfer theorem then gives an actual finite-dimensional Krivine rounding scheme and proves Theorem~\ref{thm:main}.

% \paragraph{Section~\ref{sec:formulas}: Computational formulas.}
% This section records the exact integrals, kernels, and quadrature remainders used by the interval certificate.

% \paragraph{Section~\ref{sec:impl}: Implementation notes.}
% This section explains several numerical choices in the certificate, including the use of real-axis integration, the Sobolev tail, and the cancellation-free quadrature remainder.

% \paragraph{Section~\ref{sec:discussion}: Discussion and future directions.}
% The final section explains why the third/fifth sign pattern cancels the first inverse obstructions, records a possible $7/9$ extension, and discusses how one could extract explicit finite dimensions from the collision expansion.


==> paper/krivine.tex <==
\section{Rounding Schemes}

In this section, we will define a new class of rounding schemes. But first, we recall classical Krivine schemes ~\cite{krivine1977constante}. 

\subsection{Classical Krivine rounding schemes}
\label{sec:krivine-rounding-scheme}

% \rnote{First sentence is repeating.}
A Krivine rounding scheme is a pair of partitions of $\R^d$, $f,g: \R^d \rightarrow \{-1,1\}$, such that $f,g$ are odd functions. We will work with $f,g$ that satisfy some additional properties. To describe these, we first introduce some basic setup~\cite{braverman2011grothendieckconstantstrictlysmaller}. 

% First, we introduce $H_{f,g}$, which measures the scaled correlation between $f$ and $g$ evaluated on correlated Gaussian vectors. 

\begin{definition}[Gaussian correlation function]\label{def:gaussian-correlation}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions.
Let $X, Y$ be standard jointly Gaussian vectors in $\mathbb{R}^k$ satisfying
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}t.
\]
The \emph{arcsine-normalized correlation function} associated to $(f,g)$ is
\[
H_{f,g}(t)
:=
\frac{\pi}{2}\,
\mathbb{E}\left[
f\left(X\right)
g\left(
Y
\right)
\right],
\qquad -1<t<1.
\]
\end{definition}

We will use the following basic properties of the Gaussian correlation function and its inverse $H_{f,g}^{-1}$ in our analysis (see \cite{braverman2011grothendieckconstantstrictlysmaller}).

\begin{lemma}\label[lemma]{lemma:correlation-profile-analytic}
Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd measurable functions. Then $H_{f,g}$ is odd and
extends holomorphically to the strip
\[
S:=\{z\in\mathbb{C}: |\operatorname{Re}z|<1\}.
\]
In particular, if $H_{f,g}'(0)\neq 0$, then $H_{f,g}$ has a unique \textbf{local inverse branch} at
the origin, i.e., there are open neighborhoods
$U,V\subset\C$ of $0$ such that
\(
    H_{f,g}:U\to V
\)
is biholomorphic. We write
\(
    H_{f,g}^{-1}:V\to U
\)
for this local inverse, chosen so that $H_{f,g}^{-1}(0)=0$. This inverse is
unique when restricted to this branch, and is an odd function.
\end{lemma}

% The next lemma develops 

\begin{lemma}[Local Inverse Expansion]\label[lemma]{lemma:local-inverse-expansion}

Let $f,g:\mathbb{R}^k\to\{-1,1\}$ be odd and measurable functions with $H'_{f,g}(0) \neq 0$. Let $H^{-1}_{f,g}$ be the unique local inverse branch of $H_{f,g}$ at the origin. Then,
\begin{itemize}
\item $H^{-1}_{f,g}$ is odd. 
    \item $H^{-1}_{f,g}$ has a Taylor-series expansion at the origin: $H^{-1}_{f,g}(\zeta) = \sum_{n\geq 1} a_n \zeta^n$. 
\end{itemize}
Further, if $\gamma > 0$ is such that $\sum_{n \geq 1} |a_n| \gamma^n \leq 1$, then the Grothendieck constant 
$$ K_G \leq \frac{\pi}{2\gamma}.$$ 
\end{lemma}

% For completeness, we give a proof of this  in~\cref{app:krivine-preprocessing}.

With the above notation, we define the \textbf{inverse majorant series} for the rounding scheme $(f,g)$ as 
\[
M_{f,g}(s):=\sum_{n\ge 1}|a_n|s^n.
\]

We are now ready to define Krivine schemes. 

\begin{definition}[$\gamma$-admissible Krivine Rounding Scheme]
\label[definition]{def:gamma-admissible}
    For $f,g:\mathbb{R}^k\to\{-1,1\}$ odd and measurable functions with $H'_{f,g}(0) \neq 0$, and $\gamma > 0$, we say $(f,g)$ is a $\gamma$-admissible Krivine rounding scheme if the conditions of \cref{lemma:local-inverse-expansion} hold. 
\end{definition}
We note that Krivine~\cite{Kri77} used a $\gamma$-admissible Krivine rounding scheme to show that \(K_G \le \frac{\pi}{2\gamma}.\)

==> paper/limiting_schemes.tex <==
\subsection{Preliminaries}

We first state Vitali's theorem, which lets us convert pointwise convergence to uniform convergence. See~\cite{schiff1993normal} for a reference. 

\begin{fact}[Vitali's convergence theorem]
Let \(h_1,h_2,\ldots\) be holomorphic functions on a connected open set
\(\Omega\). Suppose that:
\begin{enumerate}
    \item the sequence \((h_N)_{N\geq 1}\) is locally bounded on \(\Omega\); and
    \item \(h_N(z)\) converges for every \(z\) in some subset of \(\Omega\)
    having an accumulation point in \(\Omega\).
\end{enumerate}
Then \((h_N)_{N\geq 1}\) converges locally uniformly on \(\Omega\) to a
holomorphic function.
\end{fact}


\subsection{Limiting Krivine rounding schemes}
\label{sec:LimitingKrivine}

In this section, we extend classical Krivine schemes by allowing them to have arbitrary correlations among variables (up to some criteria). We will show that we can state asymptotic statements about classical Krivine schemes using this extended class of schemes, that we call \textit{limiting Krivine schemes}. This gives us analytic machinery for searching and analyzing limits of high dimensional schemes that were previously inaccessible via standard techniques. It is first instructive for us to start with a motivating example. 

\paragraph{Motivating example.}
Consider the two-dimensional classical Krivine rounding scheme
\[
f(X_1,X_2)=\operatorname{sgn}(X_1+\lambda X_2),
\qquad
g(Y_1,Y_2)=\operatorname{sgn}(Y_1+\lambda Y_2),
\]
where \(X_1,X_2,Y_1,Y_2\) are standard Gaussians, \(X_1\) is independent of \(X_2\), \(Y_1\) is independent of \(Y_2\), and
\[
\operatorname{corr}(X_1,Y_1)
=
\operatorname{corr}(X_2,Y_2)
=
t.
\]
In a classical Krivine scheme, every pair of corresponding coordinates has correlation \(t\). Suppose instead that we would like the first pair to have correlation \(t\), but the second pair to have correlation \(t^3\). To obtain this from a classical high-dimensional scheme, define
\[
U_N=\frac{1}{\sqrt N}\sum_{j=1}^N \mathrm{He}_3(X_{2,j}),
\qquad
V_N=\frac{1}{\sqrt N}\sum_{j=1}^N \mathrm{He}_3(Y_{2,j}),
\]
where the pairs \((X_{2,j},Y_{2,j})\) are independent standard Gaussian pairs with correlation \(t\). The Hermite identity gives
\[
\mathbb{E}[U_NV_N]
=
\mathbb{E}[\mathrm{He}_3(X_{2,1})\mathrm{He}_3(Y_{2,1})]
=
t^3.
\]
Moreover, by the central limit theorem, \((U_N,V_N)\) converges in distribution to a standard Gaussian pair \((U,V)\) with correlation \(t^3\). Thus, the classical rounding schemes
\[
F_N=\operatorname{sgn}(X_1+\lambda U_N),
\qquad
G_N=\operatorname{sgn}(Y_1+\lambda V_N)
\]
converge to the fixed-dimensional Gaussian rounding scheme
\[
f(X_1,U)=\operatorname{sgn}(X_1+\lambda U),
\qquad
g(Y_1,V)=\operatorname{sgn}(Y_1+\lambda V),
\]
in which the two coordinate pairs have correlations \(t\) and \(t^3\), respectively.

To use this construction, we need to carefully justify the following analytic steps:
\begin{enumerate}
    \item Pointwise convergence of the correlation functions must be strengthened to locally uniform convergence;
    \item An inverse-majorant $\gamma$-admissibility proved for the limiting scheme must remain valid for all sufficiently large finite-dimensional approximations.
\end{enumerate}

We now generalize this construction and prove both properties. First, we define the notion of allowable correlation maps.  
\begin{definition}[Allowable correlation map]
\label{def:allowable-correlation-map}
A function \(\rho:(-1,1)\to\mathbb{R}\) is an \emph{allowable correlation map}
if it admits an expansion
\[
\rho(t)
=
\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}} c_d t^d,
\qquad
\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}}|c_d|
\leq 1.
\]
\end{definition}

We can now state the definition of limiting Krivine schemes. 

\begin{definition}[Limiting Krivine Schemes]
A $k$-dimensional \emph{limiting Krivine scheme} is a tuple $\mathcal{S} = (f, g, \rho)$, where  \(f,g:\mathbb{R}^k\to\{-1,1\}\) are odd measurable functions where the discontinuity sets have Gaussian measure zero, and \(\rho = (\rho_1,\ldots,\rho_k)\) is a tuple of allowable correlation maps.  

The arcsine-normalized correlation function of this scheme is given by 
\[
H_{f, g, \rho}(t)
=
\frac{\pi}{2}\mathbb{E}[f(X)g(Y)].
\]
where \(X,Y\in\mathbb{R}^k\) are jointly Gaussian such that
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t).
\]
\end{definition}

\begin{remark}
    This is a generalization of the usual high dimensional Krivine schemes with $\rho_i(t) = t$ for all $i$. 

    At this stage, \(H_{f, g, \rho}\) is defined only on \((-1,1)\); in particular, we do not assume that it extends holomorphically to the strip associated with classical Krivine schemes.
\end{remark}

The motivation for this definition is that every limiting Krivine scheme can be approximated arbitrarily well by ordinary finite-dimensional Krivine schemes, as we will show below. This allows us to use the usual projection scheme to round the vectors, and get the inverse-majorant machinery for free. We make this precise in the following theorem.  

\begin{theorem}[Finite-dimensional approximation of limiting schemes]
Let \(\mathcal S=(f,g,\rho_1,\ldots,\rho_k)\) be a limiting Krivine scheme. Then there exists a sequence of ordinary finite-dimensional Krivine schemes
\(
\mathcal S_1,\mathcal S_2,\ldots,
\)
of increasing dimension, whose correlation functions $H_{\mathcal S_1}, H_{\mathcal S_2}, \ldots$ converge to the correlation function $H_{\mathcal S}$ of \(\mathcal S\), uniformly on every compact subset of \((-1,1)\).
\end{theorem}

We dedicate the rest of the section to proving this theorem. First, we prove an equivalence condition on allowability of a function. 

\begin{lemma}[Allowable function criteria]
A map \(\rho\) is allowable if and only if there are odd functions
\(p,q: \R^3 \to \R\), such that
\(\|p\|_2=\|q\|_2=1\) and
\[
\rho(t)=\mathbb{E}[p(U)q(V)],
\]
where \(U,V\in\mathbb{R}^m\) are standard Gaussian vectors with
\(\mathbb{E}[U_iV_j]=t\delta_{ij}\).
\end{lemma}

\begin{proof}
Suppose first that \(p\) and \(q\) are odd and have \(L_2\)-norm one. Write
their Hermite expansions by degree as
\[
p=\sum_{\substack{d\geq 1\\ d\text{ odd}}}p_d,
\qquad
q=\sum_{\substack{d\geq 1\\ d\text{ odd}}}q_d.
\]
Here \(p_d\) and \(q_d\) are the degree-\(d\) Hermite components.

Different Hermite degrees are orthogonal, while degree \(d\) contributes a
factor \(t^d\). Hence
\[
\mathbb{E}[p(U)q(V)]
=
\sum_{\substack{d\geq 1\\ d\text{ odd}}}
\langle p_d,q_d\rangle t^d.
\]
Set \(c_d=\langle p_d,q_d\rangle\). Then
\[
\sum_d|c_d|
\leq
\sum_d\|p_d\|_2\|q_d\|_2
\leq
\left(\sum_d\|p_d\|_2^2\right)^{1/2}
\left(\sum_d\|q_d\|_2^2\right)^{1/2}
=
1.
\]
Thus the resulting correlation map is allowable.

Conversely, suppose that
\[
\rho(t)=\sum_{d\text{ odd}}c_dt^d,
\qquad
s:=\sum_{d\text{ odd}}|c_d|\leq 1.
\]
For \(x=(x_1,x_2,x_3)\in\mathbb{R}^3\), define
\[
p(x)
=
\sum_{d\text{ odd}}
\sqrt{|c_d|}\operatorname{He}_d(x_1)
+
\sqrt{1-s}\,x_2
\]
and
\[
q(x)
=
\sum_{d\text{ odd}}
\operatorname{sgn}(c_d)\sqrt{|c_d|}
\operatorname{He}_d(x_1)
+
\sqrt{1-s}\,x_3.
\]
Both functions are odd. Orthogonality gives \(\|p\|_2=\|q\|_2=1\).

Let \(U,V\in\mathbb{R}^3\) be standard Gaussian vectors with
\(\mathbb{E}[U_iV_j]=t\delta_{ij}\). The terms involving \(U_2\) and \(V_3\)
have zero cross-correlation. Therefore
\[
\mathbb{E}[p(U)q(V)]
=
\sum_{d\text{ odd}}c_dt^d
=
\rho(t).
\]
\end{proof}

We are now ready to prove our theorem, which follows as a direct corollary of the stronger statement we prove below. 

\begin{theorem}[Finite-dimensional approximation of limiting schemes]
Let \((f,g,\rho_1,\ldots,\rho_k)\) be a limiting Krivine scheme.
Then its correlation function extends holomorphically to the unit disk and is
the locally uniform limit there of the correlation functions of ordinary
finite-dimensional Krivine schemes.
\end{theorem}

\begin{proof}
By the above lemma, for each \(i\in\{1,\ldots,k\}\), there exist odd measurable functions 
\(
p_i,q_i:\mathbb{R}^3\to\mathbb{R}
\)
with $\|p\|_2 = \|q\|_2 = 1$ such that, whenever \(U,V\in\mathbb{R}^3\) are joint standard Gaussian vectors with
\(
\mathbb{E}[U_aV_b]=t\delta_{ab},
\)
we have
\[
\mathbb{E}[p_i(U)q_i(V)]
=
\rho_i(t).
\]
We combine these functions into vector-valued maps. Write
\(u\in\mathbb{R}^{3k}\) in \(k\) blocks as
\[
u=\bigl(u^{(1)},\ldots,u^{(k)}\bigr),
\qquad
u^{(i)}\in\mathbb{R}^3,
\]
and define
\[
P(u)
=
\bigl(
p_1(u^{(1)}),\ldots,p_k(u^{(k)})
\bigr),
\]
\[
Q(u)
=
\bigl(
q_1(u^{(1)}),\ldots,q_k(u^{(k)})
\bigr).
\]
For each positive integer \(N\), define functions on
\(\bigl(\mathbb{R}^{3k}\bigr)^N\) by
\[
F_N(u_1,\ldots,u_N)
=
f\left(
\frac{1}{\sqrt{N}}\sum_{r=1}^N P(u_r)
\right)
\]
and
\[
G_N(v_1,\ldots,v_N)
=
g\left(
\frac{1}{\sqrt{N}}\sum_{r=1}^N Q(v_r)
\right).
\]
Since \(P\), \(Q\), \(f\), and \(g\) are odd, the functions \(F_N\) and
\(G_N\) are odd. They therefore define an ordinary finite-dimensional
Krivine scheme.

Let \(H_N\) denote the correlation function of this scheme. Fix
\(t\in(-1,1)\), and let
\[
(U_1,V_1),\ldots,(U_N,V_N)
\]
be independent pairs of standard Gaussian vectors in \(\mathbb{R}^{3k}\)
satisfying
\[
\mathbb{E}[(U_r)_a(V_r)_b]
=
t\delta_{ab}.
\]
Define
\[
A_N
=
\frac{1}{\sqrt{N}}\sum_{r=1}^N P(U_r),
\qquad
B_N
=
\frac{1}{\sqrt{N}}\sum_{r=1}^N Q(V_r).
\]
By the definition of the correlation function,
\[
H_N(t)
=
\frac{\pi}{2}\,
\mathbb{E}\bigl[f(A_N)g(B_N)\bigr].
\]

\begin{claim}
As \(N \rightarrow \infty\), we have \[
(A_N,B_N)
\xrightarrow{d}
(X,Y),
\]
where \((X,Y)\) is jointly Gaussian and satisfies
\[
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij},
\qquad
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t).
\]
\end{claim}

\begin{claimproof}
The random vectors
\[
\bigl(P(U_r),Q(V_r)\bigr)\in\mathbb{R}^{2k}
\]
are independent, identically distributed, and centered. Because the
\(k\) Gaussian blocks are independent, their covariance matrix is
\[
\begin{pmatrix}
I_k & D(t)\\
D(t) & I_k
\end{pmatrix},
\qquad
D(t)
=
\operatorname{diag}\bigl(
\rho_1(t),\ldots,\rho_k(t)
\bigr).
\]
By the multivariate central limit theorem, we have
\(
(A_N,B_N)
\xrightarrow[N\to\infty]{d}
(X,Y),
\)
where \((X,Y)\) is jointly Gaussian satisfying
\(
\mathbb{E}[X_iX_j]
=
\mathbb{E}[Y_iY_j]
=
\delta_{ij}\) and 
\(
\mathbb{E}[X_iY_j]
=
\delta_{ij}\rho_i(t),
\)
as desired. 
\end{claimproof}

Returning to the proof of the theorem, since the function
\(
(x,y)\longmapsto f(x)g(y)
\)
 is bounded and has discontinuity set with measure 0, it follows that
\[
\mathbb{E}\bigl[f(X_N)g(Y_N)\bigr]
\longrightarrow
\mathbb{E}\bigl[f(X(t))g(Y(t))\bigr].
\]
Consequently,
\[
H_N(t)\longrightarrow H(t)
\]
for every \(t\in(-1,1)\), where
\[
H(t)
=
\frac{\pi}{2}\,
\mathbb{E}\bigl[f(X(t))g(Y(t))\bigr]
\]
is the correlation function of the limiting scheme.

It remains to convert this pointwise convergence to locally uniform
convergence on the unit disk. For each \(N\), the Hermite expansions of
\(F_N\) and \(G_N\) give a holomorphic extension of \(H_N\) to
\[
\mathbb{D}
=
\{z\in\mathbb{C}:|z|<1\}.
\]
More explicitly, if
\[
F_N=\sum_{\alpha}\widehat{F_N}(\alpha)\operatorname{He}_{\alpha},
\qquad
G_N=\sum_{\alpha}\widehat{G_N}(\alpha)\operatorname{He}_{\alpha},
\]
then
\[
H_N(z)
=
\frac{\pi}{2}
\sum_{\alpha}
\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)z^{|\alpha|}.
\]
For \(z\) in the unit disk, the Cauchy--Schwarz inequality gives
\[
\begin{aligned}
|H_N(z)|
&\leq
\frac{\pi}{2}
\sum_{\alpha}
\bigl|
\widehat{F_N}(\alpha)\widehat{G_N}(\alpha)
\bigr|
|z|^{|\alpha|} \\
&\leq
\frac{\pi}{2}
\left(
\sum_{\alpha}
|\widehat{F_N}(\alpha)|^2
\right)^{1/2}
\left(
\sum_{\alpha}
|\widehat{G_N}(\alpha)|^2
\right)^{1/2} \\
&\leq
\frac{\pi}{2}
\|F_N\|_2\|G_N\|_2
=
\frac{\pi}{2}.
\end{aligned}
\]
Here the second inequality uses \(|z|<1\), and the third follows from
the orthonormality of the Hermite polynomials.
Thus, the family \((H_N)_{N\geq 1}\) is locally bounded on \(\mathbb{D}\).
Since it converges pointwise on the interval \((-1,1)\), which has an
accumulation point in \(\mathbb{D}\). Vitali's theorem implies that
\((H_N)\) converges locally uniformly on \(\mathbb{D}\) to a holomorphic
function. On \((-1,1)\), this function agrees with \(H\). It is therefore
the holomorphic extension of the correlation function of the limiting
scheme.
\end{proof}
We now show the following. 
\begin{theorem}[Upper bound from a limiting Krivine scheme]
\label{thm:upper_bound_limiting_scheme}
Let
\(
\mathcal{S}=(f,g,\rho_1,\ldots,\rho_k)
\)
be a limiting Krivine scheme. Let \(H\) be its correlation
function. Suppose that \(H'(0)\neq 0\), so that \(H\) has a local holomorphic inverse
at the origin. Write
\[
H^{-1}(z)
=
\sum_{j=0}^{\infty}a_{2j+1}z^{2j+1},
\]
and define its majorant by
\[
M(r)
=
\sum_{j=0}^{\infty}|a_{2j+1}|r^{2j+1}.
\]
If there exists \(\gamma>0\), within the radius of convergence of
\(H^{-1}\), such that
\(
M(\gamma)=1,
\)
then
\(
K_G
\leq
\frac{\pi}{2\gamma}.
\)
\end{theorem}


The only remaining thing left to show that an inverse-majorant bound for the
limiting correlation function passes to its finite-dimensional
approximations. We first prove this analytic stability statement.

\begin{lemma}[Finite inverse-majorant transfer]
\label{lem:finite-inverse-majorant-transfer}
Let $F_N,F$ be holomorphic on $\D$, suppose that $F_N\to F$ locally
uniformly on $\D$, and assume that $F_N(0)=F(0)=0$. Suppose that $G$ is a
holomorphic inverse branch of $F$ on a neighborhood of
$\overline{D(0,R_0)}$, takes values in $\D$, and satisfies
$
F(G(\zeta))=\zeta,$ with 
$
 |\zeta|\leq R_0.
$
Write
$
G(\zeta)=\sum_{n\geq 1}A_n\zeta^n.
$
If $0<\gamma<R_0$ and
$
\sum_{n\geq 1}|A_n|\gamma^n<1,
$
then, for all sufficiently large $N$, the function $F_N$ has a holomorphic
inverse branch
\[
G_N(\zeta)=F_N^{-1}(\zeta)=\sum_{n\geq 1}A_{n,N}\zeta^n
\]
defined on a neighborhood of $\overline{D(0,\gamma)}$, and
$
\sum_{n\geq 1}|A_{n,N}|\gamma^n<1.
$
Moreover, $A_{n,N}\to A_n$ for every fixed $n$.
\end{lemma}

\begin{proof}
The proof has three steps. First, Rouch\'e's theorem shows that the inverse
branch of $F$ persists for $F_N$. Second, the resulting inverse branches
converge to $G$, which controls every fixed coefficient. Finally, a Cauchy
estimate on a slightly larger disk controls the remaining tail uniformly in
$N$.

Choose radii
\(
\gamma<\rho<r<R<R_0
\)
and set
\(
\Omega=G(D(0,R)).
\)
Because $G$ is an inverse branch of $F$, it is injective and has nonzero
derivative on a neighborhood of $\overline{D(0,R)}$. Hence
\(
\partial\Omega=G(\partial D(0,R)).
\)
For $w\in\partial\Omega$, we therefore have $|F(w)|=R$. Thus, for every
$|\zeta|\leq r$,
\[
|F(w)-\zeta|\geq R-r,
\qquad w\in\partial\Omega.
\]
The contour $\partial\Omega$ is a compact subset of $\D$. Since
$F_N\to F$ locally uniformly, for all sufficiently large $N$,
\[
\sup_{w\in\partial\Omega}|F_N(w)-F(w)|<\frac{R-r}{2}.
\]
Fix such an $N$. For every $|\zeta|\leq r$, Rouch\'e's theorem implies that
$F_N(w)-\zeta$ and $F(w)-\zeta$ have the same number of zeros in $\Omega$,
counted with multiplicity. The equation $F(w)=\zeta$ has exactly one
solution in $\Omega$, namely $w=G(\zeta)$. Therefore $F_N(w)=\zeta$ also has
exactly one solution in $\Omega$.

These solutions define a holomorphic function $G_N$ on $D(0,r)$. One may
write it using the argument principle as
\[
G_N(\zeta)
=
\frac{1}{2\pi i}
\int_{\partial\Omega}
\frac{wF_N'(w)}{F_N(w)-\zeta}\,dw,
\qquad |\zeta|<r.
\]
This is the unique solution of $F_N(w)=\zeta$ in $\Omega$. In particular,
$G_N(0)=0$ and
\(
F_N(G_N(\zeta))=\zeta.
\)
Thus $G_N$ is the inverse branch of $F_N$ at the origin.

The same argument-principle formula holds for $G$. The denominators above
are uniformly bounded away from zero on
$\partial\Omega\times\overline{D(0,r)}$, and local uniform convergence of
$F_N$ implies uniform convergence of $F_N'$ to $F'$ on $\partial\Omega$.
It follows that
\(
G_N\longrightarrow G
\)
uniformly on $\overline{D(0,r)}$. By Cauchy's coefficient formula,
\(
A_{n,N}\longrightarrow A_n
\)
for every fixed $n$.

It remains to control all coefficients at once. Let
\(
B=\sup_{w\in\overline\Omega}|w|.
\)
Since $G_N(D(0,r))\subseteq\Omega$, Cauchy's estimate on the circle
$|\zeta|=\rho$ gives
\(
|A_{n,N}|\leq B\rho^{-n},
\qquad n\geq 1,
\)
for all sufficiently large $N$.

Set
\(
\delta
=
1-\sum_{n\geq 1}|A_n|\gamma^n
>0.
\)
Choose $M$ large enough that
\(
B\sum_{n>M}\left(\frac{\gamma}{\rho}\right)^n
<\frac{\delta}{3}.
\)
Since the first $M$ coefficients converge, for all sufficiently large $N$,
\(
\sum_{n\leq M}|A_{n,N}|\gamma^n
\leq
\sum_{n\leq M}|A_n|\gamma^n
+
\frac{\delta}{3}.
\)
Combining the head and tail bounds gives
\begin{align*}
\sum_{n\geq 1}|A_{n,N}|\gamma^n
&\leq
\sum_{n\leq M}|A_n|\gamma^n
+
\frac{\delta}{3}
+
B\sum_{n>M}\left(\frac{\gamma}{\rho}\right)^n \\
&<
\sum_{n\geq 1}|A_n|\gamma^n
+
\frac{2\delta}{3}
<1.
\end{align*}
This proves the claim.
\end{proof}
We will now prove ~\cref{thm:upper_bound_limiting_scheme}.
% \begin{theorem}[Upper bound from a limiting Krivine scheme]
% \label{thm:upper-bound-from-limiting-scheme}
% Let
% \(
% \mathcal{S}=(f,g,\rho_1,\ldots,\rho_k)
% \)
% be a limiting Krivine scheme. Let $H$ be its correlation function. Suppose
% that $H'(0)\neq 0$, so that $H$ has a local holomorphic inverse at the
% origin. Write
% \[
% H^{-1}(z)
% =
% \sum_{j=0}^{\infty}a_{2j+1}z^{2j+1},
% \]
% and define its majorant by
% \[
% M(r)
% =
% \sum_{j=0}^{\infty}|a_{2j+1}|r^{2j+1}.
% \]
% If there exists $\gamma>0$, within the radius of convergence of $H^{-1}$,
% such that
% \(
% M(\gamma)=1,
% \)
% then
% \(
% \KG
% \leq
% \frac{\pi}{2\gamma}.
% \)
% \end{theorem}

\begin{proof}
We first move from $\gamma$ to an arbitrary smaller radius $\gamma'<\gamma$, where the majorant inequality is strict. We then transfer this strict certificate to a finite-dimensional approximation and finally let $\gamma'$ approach $\gamma$.

Let $H_N$ be the correlation functions of the ordinary finite-dimensional
Krivine schemes supplied by the finite-dimensional approximation theorem.
Thus
\(
H_N\longrightarrow H
\)
locally uniformly on $\D$. Since all of the schemes are odd,
$H_N(0)=H(0)=0$.

The equality $M(\gamma)=1$ need not remain true under a small perturbation,
so we first work at a slightly smaller radius. Fix any
\(
0<\gamma'<\gamma.
\)
Because
\(
a_1=\frac{1}{H'(0)}\neq 0,
\)
the majorant is strictly increasing on the positive real axis. Hence
\(
M(\gamma')<M(\gamma)=1.
\)
Choose $R_0$ such that
\(
\gamma'<R_0<\gamma.
\)
Then $M(R_0)<1$. If $G=H^{-1}$ denotes the inverse power series, then for
$|z|\leq R_0$,
\(
|G(z)|
\leq
M(|z|)
\leq
M(R_0)
<1.
\)
Thus $G$ is holomorphic on a neighborhood of
$\overline{D(0,R_0)}$ and takes values in $\D$. Moreover, the identity
$H(G(z))=z$ holds near the origin. Both sides are holomorphic on
$D(0,R_0)$, so the identity theorem gives
\[
H(G(z))=z,
\qquad |z|<R_0.
\]
Therefore $G$ is an inverse branch of $H$ on this disk.

We may now apply Lemma~\ref{lem:finite-inverse-majorant-transfer} at the
radius $\gamma'$. For all sufficiently large $N$, the inverse branch of
$H_N$ has an expansion
\[
H_N^{-1}(z)=\sum_{n\geq 1}a_{n,N}z^n
\]
satisfying
\[
\sum_{n\geq 1}|a_{n,N}|(\gamma')^n<1.
\]
The classical Krivine criterion applied to this finite-dimensional scheme
therefore yields
\(
\KG\leq \frac{\pi}{2\gamma'}.
\)
This holds for every $\gamma'<\gamma$. Letting $\gamma'$ increase to
$\gamma$ gives
\[
\KG\leq \frac{\pi}{2\gamma},
\]
as claimed.
\end{proof}


==> paper/lower_bound_general.tex <==
\section{Proof Overview}
\label{sec:proof-idea}

% \rnote{The section names are odd; also too many sections. Its helpful to state what a section is going to do at the beginning of the section. For example, 9.1. }

\begin{theorem}\label{thm:lower-bound}
The Grothendieck constant satisfies
\[
        K_G\ge\frac{6\pi}{11} = 1.7136\ldots.
\]
\end{theorem}

A sketch of the proof is as follows. First, recall the inverse-series step in Krivine's rounding argument. If
\[
        H^{-1}(z)=\sum_{j\ge0}a_{2j+1}z^{2j+1},
\]
define the absolute-coefficient majorant $M_H(s):=\sum_{j\ge0}|a_{2j+1}|s^{2j+1}$. The standard tensor preprocessing gives the implication
\begin{equation}
        M_H(\gamma)\le1
        \quad\Longrightarrow\quad
        K_G\le\frac{\pi}{2\gamma}.
        \label{eq:inverse-majorant-bound}
\end{equation}
We refer to~\eqref{eq:inverse-majorant-bound} as the \emph{inverse-majorant bound}.

The conceptual starting point is the theorem of Naor and Regev that Krivine schemes are optimal \cite{naor2014krivine}. By reworking the construction in their proof, we show that the inverse-majorant bound is itself asymptotically optimal after allowing mixtures and increasing dimension: there are limiting mixed correlation functions with admissible parameters converging to $\pi/(2K_G)$. This transfer is established in Section~\ref{sec:majorant_optimal}.

It therefore remains to prove a universal upper bound on such admissible parameters. For arbitrary odd measurable sign functions $f,g:\R^d\to\{\pm1\}$, write
\[
        H_{f,g}(t)=b_1t+b_3t^3+b_5t^5+\cdots.
\]
The technical core of the argument is the affine coefficient inequality
\[
        b_3\ge 2b_1-\frac{11}{6}.
\]
Section~\ref{sec:preliminaries} sets up the Gaussian--Hermite formulation, and Section~\ref{sec:affine-strip} proves this inequality by decomposing $f$ and $g$ into their agreement and disagreement parts and reducing the required estimates to one-dimensional inequalities. Its linearity in $(b_1,b_3)$ is essential, because it makes the inequality stable under mixtures and coefficientwise limits.

Section~\ref{sec:strip_majorant} then shows that the affine coefficient inequality controls the inverse-majorant bound: every admissible value must satisfy $\gamma\le11/12$. Applying this barrier to the asymptotically optimal sequence constructed in Section~\ref{sec:majorant_optimal} gives
\[
        \frac{\pi}{2K_G}\le\frac{11}{12},
\]
which is exactly Theorem~\ref{thm:lower-bound}.

\section{Preliminaries on Gaussian Hermite Expansions}
\label{sec:preliminaries}

Let
\[
        X\sim N(0,I_d)
\]
be a standard Gaussian vector in $\R^d$. We define the \textit{inner product} as the Gaussian expectation:
\[
        \ip{F}{G}=\E[F(X)G(X)].
\]
We use the orthonormal 1D Hermites
\[
        \HermBasis_0=1,\qquad
        \HermBasis_1(s)=s,\qquad
        \HermBasis_2(s)=\frac{s^2-1}{\sqrt2},\qquad
        \HermBasis_3(s)=\frac{s^3-3s}{\sqrt6}.
\]

In $d$ dimensions the Hermite basis is indexed by multi-indices. If
\[
        \alpha=(\alpha_1,\ldots,\alpha_d),
        \qquad |\alpha|=\alpha_1+\cdots+\alpha_d,
\]
then
\[
        \HermBasis_\alpha(X)=\prod_{i=1}^d \HermBasis_{\alpha_i}(X_i).
\]
Any square integrable function has a Hermite expansion, written as
\[
        F=P_0F+P_1F+P_2F+P_3F+\ldots,
\]
where $P_iF$ is the orthogonal projection of $F$ onto the span of all $\HermBasis_\alpha$ with total degree $|\alpha|=i$.

In particular, the degree-one Hermites span
\[
        \cH_1=\operatorname{span}\{X_1,\ldots,X_d\}.
\]
Here,
\[
        P_1F=\ip{c_F}{X},
        \qquad
        c_F=\E[F(X)X]\in\R^d.
\]
Its norm is
\[
        \norm{P_1F}^2=\norm{c_F}_{\ell_2}^2.
\]

Similarly, $P_3F$ is the projection onto the full total degree-three Hermite span. We will not list all basis elements. The important point is that it includes pure cubic directions such as $\HermBasis_3(X_i)$ and mixed directions such as $\HermBasis_2(X_i)\HermBasis_1(X_j)$ and $\HermBasis_1(X_i)\HermBasis_1(X_j)\HermBasis_1(X_\ell)$.

For signs $f,g:\R^d\to\{\pm1\}$, if
\[
        H_{f,g}(t)=\frac\pi2\E[f(X)g(X'_t)]
\]
with $(X,X'_t)$ a pair of correlated standard Gaussian vectors, then Mehler's identity gives
\[
        H_{f,g}(t)=\frac\pi2\sum_{m\ge0}\ip{P_mf}{P_mg}t^m.
\]
Here
\[
        b_1=[t]H_{f,g}=\frac\pi2\ip{P_1f}{P_1g},
        \qquad
        b_3=[t^3]H_{f,g}=\frac\pi2\ip{P_3f}{P_3g}.
\]

For the rest of the paper, we will use the shorthand
\[
        \nu:=\sqrt{\frac{2}{\pi}}=\E|Z|,
        \qquad Z\sim N(0,1).
\]

We want to prove
\begin{equation}
        b_3\ge 2b_1-\frac{11}{6}.
        \label{eq:affine-strip}
\end{equation}

For example, the hyperplane partitions lie on this line. For $f=g=\sgn(X_1)$,
\[
        \norm{P_1f}=\nu,
        \qquad
        \norm{P_3f}^2=\frac{\nu^2}{6}.
\]
Thus
\[
        (b_1,b_3)=\left(1,\frac16\right),
\]
and this point lies exactly on the line since $1/6=2-11/6$.

Instead of proving the strip directly, it suffices to prove
\begin{equation}
        B_1(f,g)
        :=\norm{P_1f}\norm{P_1g}
          +\ip{P_1f}{P_1g}
          -\ip{P_3f}{P_3g}
        \le \frac{11}{6}\nu^2.
        \label{eq:b1-bound}
\end{equation}
Indeed, by Cauchy--Schwarz,
\[
        \norm{P_1f}\norm{P_1g}\ge \ip{P_1f}{P_1g}.
\]
So~\eqref{eq:b1-bound} implies
\[
        2\ip{P_1f}{P_1g}-\ip{P_3f}{P_3g}\le \frac{11}{6}\nu^2.
\]
Multiplying by $\pi/2$ and using $\nu^2=2/\pi$ gives~\eqref{eq:affine-strip}.

\section{Proof of the Affine Coefficient Inequality}
\label{sec:affine-strip}

\subsection{The agreement--disagreement substitution}
\label{sec:agreement-disagreement}

We define a change of variables based on where $f$ and $g$ agree or disagree. Set the functions $h,k$ to be
\[
        h=\frac{f+g}{2},\qquad k=\frac{f-g}{2}.
\]
Then
\[
        f=h+k,
        \qquad
        g=h-k.
\]
Since $f,g$ are signs,
\[
        h,k\in\{-1,0,1\},
        \qquad
        hk=0,
        \qquad
        h^2+k^2=1.
\]
Think of $h$ as the agreement part and $k$ as the disagreement part between $f$ and $g$. This change of variables considerably simplifies the proof.

Let
\[
        u=P_1h,
        \qquad
        v=P_1k.
\]
Then
\[
        P_1f=u+v,
        \qquad
        P_1g=u-v.
\]
Hence
\[
        \ip{P_1f}{P_1g}=\norm{u}^2-\norm{v}^2.
\]
Also
\[
        \norm{P_1f}\norm{P_1g}
        =\norm{u+v}\norm{u-v}
        \le \norm{u}^2+\norm{v}^2,
\]
using $ab\le(a^2+b^2)/2$ after expanding $\norm{u\pm v}^2$.

For degree three,
\[
        P_3f=P_3h+P_3k,
        \qquad
        P_3g=P_3h-P_3k,
\]
so
\[
        \ip{P_3f}{P_3g}=\norm{P_3h}^2-\norm{P_3k}^2.
\]
Putting these together,
\begin{align*}
        B_1(f,g)
        &\le
        \bigl(\norm{u}^2+\norm{v}^2\bigr)
        +\bigl(\norm{u}^2-\norm{v}^2\bigr)
        -\bigl(\norm{P_3h}^2-\norm{P_3k}^2\bigr)\\
        &=2\norm{P_1h}^2-\norm{P_3h}^2+\norm{P_3k}^2.
\end{align*}

So it is enough to prove
\begin{equation}
\boxed{\displaystyle
        D_1(h,k):=2\norm{P_1h}^2-\norm{P_3h}^2+\norm{P_3k}^2
        \le \frac{11}{6}\nu^2
}
\label{eq:hk-reduction}
\end{equation}

In order to prove this, we have to handle each of the three expressions $\norm{P_1h}^2$, $\norm{P_3h}^2$, $\norm{P_3k}^2$ carefully. In particular, we need to prove upper bounds on $\norm{P_1h}^2$, $\norm{P_3k}^2$ and a lower bound on $\norm{P_3h}^2$.

\begin{remark}
    Note that in the inequality before~\eqref{eq:hk-reduction} the term $\norm{v}^2=\norm{P_1k}^2$ conveniently cancels. This is a result of the choice of the strip $b_3\ge 2b_1-11/6$. Stronger lower bounds can be proved with the same method, but this is more complicated because one also has to bound $\norm{P_1k}^2$.
\end{remark}

\subsection{Reduction to one Gaussian coordinate}
\label{sec:rotation}

The linear part of $h$ has the form
\[
        P_1h(X)=\ip{c_h}{X}.
\]
The coefficient vector is $c_h\in\R^d$, and
\[
        \norm{P_1h}=\norm{c_h}_{\ell_2}.
\]
If $c_h\neq0$, rotate coordinates so the first coordinate points in the $c_h$ direction. After this rotation, and after renaming the coordinates, we write
\[
        X=(S,T),
        \qquad S\sim N(0,1),\quad T\sim N(0,I_{d-1}),
\]
with $S$ independent of $T$, and
\[
        P_1h(S,T)=\norm{P_1h}\,S.
\]
If $P_1h=0$, choose any direction as $S$.

Define
\[
        x:=\frac{\norm{P_1h}}{\nu}\in[0,1].
\]
The bound $x\le1$ follows from
\[
        \norm{P_1h}=\sup_{\norm{e}=1}\E[h(X)\ip{e}{X}]
        \le \E|Z|=\nu.
\]
After rotation,
\[
        \ip{h}{S}=\norm{P_1h}=\nu x.
\]

\subsection{The agreement terms}
\label{sec:agreement}

The agreement part of $D_1$ is $2\norm{P_1h}^2-\norm{P_3h}^2$. The helpful negative term is
\[
        -\norm{P_3h}^2.
\]
To use it, we only need a lower bound on $\norm{P_3h}^2$.

In any dimension,
\[
        \norm{P_3h}^2
        \ge \ip{h}{\HermBasis_3(S)}^2,
\]
because $\HermBasis_3(S)$ is one orthonormal degree-three Hermite direction. The trick we will use is to condition on the transverse variables, so define
\[
        A(s):=\E_T[h(s,T)].
\]
This is the average value of $h$ along the slice $S=s$. Since $h\in[-1,1]$,
\[
        |A(s)|\le1.
\]
Also, for every function $\varphi$ depending only on $S$, it is a straightforward conditioning to show that
\[
        \E[h(S,T)\varphi(S)]=\E[A(S)\varphi(S)].
\]
In particular,
\[
        \E[A(S)S]=\ip{h}{S}=\nu x
\]
and
\[
        \ip{h}{\HermBasis_3(S)}=\E[A(S)\HermBasis_3(S)].
\]

This is the same trick as in the two-dimensional note. The problem is now a variational problem in the one variable function $A$, even though we are working in $d$ dimensions. To bound the agreement part, it is sufficient to relax $A$, and answer the following question:

\begin{quote}
``Among all $A:\R\to[-1,1]$ with $\E[A(S)S]=\nu x$, how small can the cubic coefficient be?''
\end{quote}

The answer is the rearrangement lemma.

Define
\[
        W(S):=S^3-3S=\sqrt6\,\HermBasis_3(S).
\]
Also define
\[
        \Delta(x):=x+2(1+x)\log\frac{1+x}{2},
        \qquad
        \Delta_+(x):=\max\{\Delta(x),0\}.
\]

\begin{lemma}[One-dimensional rearrangement]
Let $S\sim N(0,1)$ and $x\in[0,1]$. Then
\[
        \sup_{\substack{|A|\le1\\ \E[A(S)S]=\nu x}}
        \E[A(S)(S^3-3S)]
        =-\nu\Delta(x).
\]
\end{lemma}

\begin{proof}
Fix $r\ge0$ by
\[
        e^{-r^2/2}=\frac{1+x}{2},
\]
and put
\[
        \mu=r^2-3.
\]
Let $W=S^3-3S$. Then
\[
        W-\mu S=S^3-3S-(r^2-3)S=S(S^2-r^2).
\]

For any feasible $A$,
\begin{align*}
        \E[AW]
        &=\E[A(W-\mu S)]+\mu\E[AS]\\
        &=\E[A(W-\mu S)]+\mu\nu x\\
        &\le \E|W-\mu S|+\mu\nu x,
\end{align*}
using $|A|\le1$.

Equality is attained by
\[
        A_*(S)=\sgn(W-\mu S)=\sgn(S)\sgn(S^2-r^2),
\]
provided $A_*$ has the right first moment. It does, because
\[
        A_*(S)S=|S|\sgn(S^2-r^2),
\]
so
\begin{align*}
        \E[A_*(S)S]
        &=2\E[|S|\one_{|S|>r}]-\E|S|\\
        &=2\nu e^{-r^2/2}-\nu\\
        &=\nu x.
\end{align*}
Thus $A_*$ is feasible and attains the dual upper bound.

It remains to compute its value. Since
\[
        \sgn(S)(S^3-3S)=|S|^3-3|S|,
\]
we get
\begin{align*}
        \E[A_*W]
        &=\E[(|S|^3-3|S|)\sgn(S^2-r^2)]\\
        &=2\E[(|S|^3-3|S|)\one_{|S|>r}]
          -\E[|S|^3-3|S|].
\end{align*}
The Gaussian tail moments are
\[
        \E[|S|\one_{|S|>r}]=\nu e^{-r^2/2},
        \qquad
        \E[|S|^3\one_{|S|>r}]=\nu(r^2+2)e^{-r^2/2}.
\]
Also
\[
        \E|S|=\nu,
        \qquad
        \E|S|^3=2\nu.
\]
Therefore
\begin{align*}
        \E[A_*W]
        &=2\nu(r^2-1)e^{-r^2/2}+\nu\\
        &=\nu\left(1+(1+x)(r^2-1)\right)\\
        &=\nu\left((1+x)r^2-x\right).
\end{align*}
Since $r^2=-2\log((1+x)/2)$,
\[
        \E[A_*W]
        =-\nu\left(x+2(1+x)\log\frac{1+x}{2}\right)
        =-\nu\Delta(x).
\]
This proves the lemma.
\end{proof}

% We delegate the proof to Appendix~\ref{app:rearrangement_lemma}, which uses standard variational techniques. Using this rearrangement lemma gives the desired bound on the agreement part.

\begin{corollary}[Diagonal bound]
For the general-dimensional ternary $h$ above,
\[
        \norm{P_3h}^2\ge \frac{\nu^2}{6}\Delta_+(x)^2.
\]
Consequently
\[
        2\norm{P_1h}^2-\norm{P_3h}^2
        \le
        \nu^2\left(2x^2-\frac16\Delta_+(x)^2\right).
\]
\end{corollary}

\subsection{The disagreement term}
\label{sec:disagreement}

Now we have to bound the disagreement term
\(
        \norm{P_3k}^2.
\)
For each fixed vector \(t\), restrict \(k\) to the one-dimensional line obtained by varying \(S\) while holding \(T=t\). We call this restriction the \textbf{fiber} of \(k\) over \(t\), and write
\[
    u_t(s):=k(s,t).
\]
Since \(k\in\{-1,0,1\}\), every fiber \(u_t\) is a one-dimensional ternary function. For $j=0,1,2,3$, define
\[
        K_j(t):=\E_S[k(S,t)\HermBasis_j(S)].
\]
Thus $K_j$ is the $j$th Hermite coefficient of the $S$-fiber, as a function of the transverse variable $t$. In two dimensions, the four degree-three basis elements were
\[
        \HermBasis_3(S),\qquad
        \HermBasis_2(S)\HermBasis_1(T),\qquad
        \HermBasis_1(S)\HermBasis_2(T),\qquad
        \HermBasis_3(T).
\]
In general dimensions, this becomes the orthogonal decomposition
\[
        \cH_3(S,T)
        =\bigoplus_{j=0}^3 \cH_j(S)\otimes \cH_{3-j}(T).
\]
This just says that a total degree-three Hermite can spend $j$ degrees in $S$ and $3-j$ degrees in $T$.

Therefore
\[
        P_3k
        =\sum_{j=0}^3 \HermBasis_j(S)\,\Pi^T_{3-j}K_j(T),
\]
where $\Pi^T_{3-j}$ is the orthogonal projection in the $T$ variable onto transverse Hermite degree $3-j$. Hence
\begin{equation}
        \norm{P_3k}^2
        =\sum_{j=0}^3 \norm{\Pi^T_{3-j}K_j}^2.
        \label{eq:p3k-decomposition}
\end{equation}
Since the $\Pi^T_{3-j}$ are orthogonal projections onto closed subspaces, they decrease norm, so we get the simpler upper bound
\[
        \norm{P_3k}^2
        \le \sum_{j=0}^3\norm{K_j}^2
        =\E_T\sum_{j=0}^3\left(\E_S[k(S,T)\HermBasis_j(S)]\right)^2.
\]
For a one dimensional ternary function $u$, define
\[
        V(u):=\sum_{j=0}^3\left(\E[u(Z)\HermBasis_j(Z)]\right)^2.
\]
Then the previous inequality becomes
\begin{equation}
        \boxed{\norm{P_3k}^2\le \E_T V(u_T).}
        \label{eq:p3k-fiber-bound}
\end{equation}

For a ternary function $u:\R\to\{-1,0,1\}$, define its weighted support budget
\[
        \beta(u):=\E[|Z|u(Z)^2].
\]
Since $u^2=\one_{u\neq0}$,
\[
        \beta(u)=\E[|Z|\one_{u(Z)\neq0}].
\]
So $\beta(u)$ is the $|Z|$-weighted Gaussian size of the support of the fiber.

\begin{theorem}[Fiber inequality]
For every ternary $u:\R\to\{-1,0,1\}$,
\begin{equation}
        V(u)\le 3\nu\beta(u)-\beta(u)^2.
        \label{eq:fiber-inequality}
\end{equation}
\end{theorem}


\paragraph{Proof sketch}. This is proved in Appendix~\ref{app:fiber-certificate}, which reduces ~\eqref{eq:fiber-inequality} to a finite computational check. Here, we briefly sketch out the proof. The inequality is genuinely finite-dimensional: $V(u)$ depends only on the four moments $\E[u\HermBasis_j]$, $0\le j\le3$. By the dual formula for the Euclidean norm,
\[
        \sqrt{V(u)}=\sup_{\norm{a}_2=1}\E[u(Z)p_a(Z)],
        \qquad
        p_a(Z)=\sum_{j=0}^3a_j\HermBasis_j(Z).
\]
For fixed $p_a$ and a fixed support price $\tau\ge0$, pointwise maximization over the three values of $u$ gives
\[
        \max_{v\in\{-1,0,1\}}\bigl(v\,p_a(z)-\tau|z|\,v^2\bigr)
        =\bigl(|p_a(z)|-\tau|z|\bigr)_+,
\]
with maximizer the threshold rule
\[
        u(z)=\sgn(p_a(z))\one_{\{|p_a(z)|\ge \tau |z|\}};
\]
threshold functions are thus the exact optimizers of the priced problem, not merely plausible candidates. The infinite-dimensional search over $u$ therefore collapses to the four-parameter family $(a,\tau)$, whose active sets are cut out by one-dimensional polynomial inequalities; the content of~\eqref{eq:fiber-inequality} is the inequality $3\nu\beta-m^2\ge\beta^2$ along this family, where $m=\int_E|p_a|\,d\gamma$ and $\beta=\int_E|z|\,d\gamma$ over the active set $E$. The constant fiber $u\equiv1$ (that is, $p_a=\HermBasis_0$, $\tau=0$) realizes $\rho:=(3\nu\beta-m^2)/\beta^2=3-\pi/2\approx1.4292$, and numerical scans over the family find no smaller value. This suggests that~\eqref{eq:fiber-inequality} --- which asserts only $\rho\ge1$ --- holds with about $0.43$ of true headroom, though we do not prove this sharper assertion.

Appendix~\ref{app:fiber-certificate} turns this into a proof: it reduces~\eqref{eq:fiber-inequality} to two certified regimes (a direction-free high-budget bound and a Fenchel-dual low-budget bound), each consisting of finitely many one-dimensional inequalities that are verified in outward-rounded interval arithmetic. 

\paragraph{Reproducibility.}
  The scripts, certificates, and Arb outputs for this 
  are available at \url{https://github.com/trishullab/grothendieck-bounds}. 

\vspace{\baselineskip}

Apply~\eqref{eq:fiber-inequality} to each fiber $u_T$. From~\eqref{eq:p3k-fiber-bound},
\[
        \norm{P_3k}^2
        \le
        \E_T\left[3\nu\beta(u_T)-\beta(u_T)^2\right].
\]
We now prove the following bound. Note that this step is dimension-free.

\begin{theorem}[Fiber Residual Bound \#1]
We have the fiber bound
\begin{equation}
        \norm{P_3k}^2
        \le
        \nu^2\left(3(1-x)-(1-x)^2\right).
        \label{eq:fiber-residual-one}
\end{equation}
\end{theorem}

\begin{proof}
We do this by relating the average budget to $x$. Since
\[
        \nu x=\E[hS]
\]
and
\[
        hS\le |S|h^2,
\]
we get
\begin{align*}
        \nu x
        &\le \E[|S|h^2]\\
        &=\E[|S|(1-k^2)]\\
        &=\nu-\E[|S|k^2].
\end{align*}
Therefore
\[
        \E[|S|k^2]\le \nu(1-x).
\]
But
\[
        \E[|S|k^2]
        =\E_T\E_S[|S|k(S,T)^2]
        =\E_T\beta(u_T).
\]
Let
\[
        b:=\E_T\beta(u_T).
\]
Then
\[
        b\le \nu(1-x).
\]

The function
\[
        \phi(t)=3\nu t-t^2
\]
is concave, so Jensen gives
\[
        \E_T\phi(\beta(u_T))\le \phi(\E_T\beta(u_T))=3\nu b-b^2.
\]
On $[0,\nu]$, $\phi$ is increasing. Hence, using $b\le \nu(1-x)$, we obtain~\eqref{eq:fiber-residual-one}.
\end{proof}

This is our first fiber residual bound. But this bound is not best for small $x$. We also use a second cruder bound.

\begin{theorem}[Fiber Residual Bound \#2]
    \begin{equation}
        \norm{P_3k}^2
        \le
        2\PhiG(\sqrt{-2\log x})-1.
        \label{eq:fiber-residual-two}
\end{equation}
\end{theorem}

\begin{proof}
Let
\[
        \rho(s):=\E_T[k(s,T)^2].
\]
Then $0\le\rho\le1$ and
\[
        \norm{k}^2_2=\E\rho(S).
\]
Also
\[
        \E[|S|\rho(S)]=\E[|S|k(S,T)^2]\le \nu(1-x).
\]
Since $P_3$ is an orthogonal projection,
\[
        \norm{P_3k}^2\le \norm{k}^2_2=\E\rho(S).
\]

Given a budget on $\E[|S|\rho(S)]$, the way to maximize $\E\rho(S)$ is to spend the budget where $|S|$ is smallest. Thus the extremal support is centered around zero.

Let
\[
        r_x:=\sqrt{-2\log x}
\]
for $x\in(0,1]$, with the convention $r_0=\infty$. Then
\[
        \E[|S|\one_{|S|\le r_x}]=\nu(1-e^{-r_x^2/2})=\nu(1-x).
\]
Therefore the bathtub principle gives
\[
        \norm{P_3k}^2
        \le
        \mathbb P(|S|\le r_x)
        =2\PhiG(\sqrt{-2\log x})-1,
\]
which proves~\eqref{eq:fiber-residual-two}.
\end{proof}

Combining the two fiber residual bounds, define
\begin{equation}
        R(x):=
        \min\left\{
        3(1-x)-(1-x)^2,
        \frac{1}{\nu^2}\left(2\PhiG(\sqrt{-2\log x})-1\right)
        \right\}.
        \label{eq:residual-function}
\end{equation}
Then
\[
        \norm{P_3k}^2\le \nu^2R(x).
\]

\subsection{The final inequality}
\label{sec:putting-together}

From the diagonal bound and the residual bound,
\[
        D_1(h,k)
        \le
        \nu^2\left(2x^2-\frac16\Delta_+(x)^2+R(x)\right).
\]
So it remains to prove the scalar inequality
\begin{equation}
        E_1(x):=2x^2-\frac16\Delta_+(x)^2+R(x)
        \le \frac{11}{6}
        \qquad(0\le x\le1).
        \label{eq:scalar-reduction}
\end{equation}

Let
\[
        r_-:=\frac{1-1/\sqrt3}{2},
        \qquad
        r_+:=\frac{1+1/\sqrt3}{2}.
\]
These are the roots of
\[
        x^2-x+\frac16=0.
\]

Now we do some simple casework based on the range in which $x$ lies. Everything is simple algebra.

\subsection*{Low range: $0\le x\le r_-$}

Use the crude bound $R(x)\le 1/\nu^2=\pi/2$ and drop the negative term:
\[
        E_1(x)\le 2x^2+\frac\pi2
        \le 2r_-^2+\frac\pi2.
\]
Now
\[
        2r_-^2+\frac\pi2
        =\frac23-\frac1{\sqrt3}+\frac\pi2
        <\frac{11}{6}.
\]

\subsection*{Middle range: $r_-\le x\le r_+$}

Use the fiber branch of $R$ and again drop the negative term:
\begin{align*}
        E_1(x)
        &\le 2x^2+3(1-x)-(1-x)^2\\
        &=x^2-x+2.
\end{align*}
Since $x\in[r_-,r_+]$,
\[
        x^2-x+\frac16\le0.
\]
Therefore
\[
        x^2-x+2\le \frac{11}{6}.
\]

\subsection*{High range: $r_+\le x\le1$}

Use the fiber branch again. We need the cubic correction.
It suffices to show
\begin{equation}
        \Delta(x)^2\ge 6x^2-6x+1.
        \label{eq:high-range-correction}
\end{equation}
Indeed, then
\begin{align*}
        E_1(x)
        &\le 2x^2+3(1-x)-(1-x)^2-\frac16(6x^2-6x+1)\\
        &=\frac{11}{6}.
\end{align*}

To prove~\eqref{eq:high-range-correction}, first note that
\[
        \Delta(x)-(3x-2)
        =2\left((1-x)+(1+x)\log\frac{1+x}{2}\right).
\]
Writing $t=(1+x)/2$, the bracket becomes
\[
        2\bigl((1-t)+t\log t\bigr)\ge0
\]
for $0<t\le1$. Hence
\[
        \Delta(x)\ge 3x-2.
\]
For $x\ge r_+$, both sides needed below are nonnegative, and
\[
        (3x-2)^2-(6x^2-6x+1)=3(1-x)^2\ge0.
\]
Thus
\[
        \Delta(x)^2\ge (3x-2)^2\ge 6x^2-6x+1.
\]
This proves the high range.

Combining the three ranges proves~\eqref{eq:scalar-reduction}.

We have thus shown
\[
        D_1(h,k)\le \frac{11}{6}\nu^2.
\]
As explained earlier, this implies the affine coefficient inequality
\[
        b_3\ge 2b_1-\frac{11}{6}.
\]
Since this is affine, it is preserved under mixtures.

\section{The Affine Coefficient Inequality Bounds the Inverse Majorant}
\label{sec:strip_majorant}

\begin{definition}[Admissible majorant value]\label{def:admissible-majorant}
Let $H$ be odd and analytic near the origin, with $H'(0)>0$. Let $H^{-1}$ denote the local inverse branch satisfying $H^{-1}(0)=0$, and write
\[
        H^{-1}(z)=\sum_{j\ge0}a_{2j+1}z^{2j+1}.
\]
A number $\gamma>0$ is \emph{admissible} for $H$ if this series converges absolutely at $\gamma$ and
\[
        \sum_{j\ge0}|a_{2j+1}|\gamma^{2j+1}\le1.
\]
\end{definition}

We now turn the affine coefficient inequality proved in Section~\ref{sec:affine-strip} into a universal barrier for the inverse-majorant parameter. The coefficients $b_1$ and $b_3$ depend linearly on the correlation function, so the strip is preserved under mixtures and coefficientwise limits. Section~\ref{sec:majorant_optimal} will apply this barrier to the limiting mixed functions supplied by the Naor--Regev construction.

\begin{proposition}[The majorant barrier]\label{prop:majorant-barrier}
Let
\[
        H(t)=b_1t+b_3t^3+b_5t^5+\cdots
\]
be odd and analytic near the origin. Suppose that
\[
        0<b_1\le1,
        \qquad
        b_3\ge2b_1-\frac{11}{6}.
\]
Then every admissible value for $H$ satisfies
\[
        \gamma\le\frac{11}{12}.
\]
\end{proposition}

\begin{proof}
Write
\[
        H^{-1}(z)=a_1z+a_3z^3+\cdots.
\]
Comparing the coefficients of $z$ and $z^3$ in $H(H^{-1}(z))=z$ gives
\[
        a_1=\frac1{b_1},
        \qquad
        a_3=-\frac{b_3}{b_1^4}.
\]

If $b_1\le11/12$, admissibility gives
\[
        1\ge |a_1|\gamma=\frac{\gamma}{b_1},
\]
so $\gamma\le11/12$.

Suppose now that $b_1>11/12$. The strip gives
\[
        b_3\ge2\left(b_1-\frac{11}{12}\right)>0.
\]
Let
\[
        M_H(s):=\sum_{j\ge0}|a_{2j+1}|s^{2j+1},
\]
allowing the value $+\infty$. Using only the first two terms,
\begin{align*}
        M_H\left(\frac{11}{12}\right)
        &\ge
        \frac{11}{12b_1}
        +\frac{2(b_1-\frac{11}{12})}{b_1^4}
          \left(\frac{11}{12}\right)^3\\
        &=1+
        \frac{(b_1-\frac{11}{12})
        \left(2(\frac{11}{12})^3-b_1^3\right)}{b_1^4}
        >1.
\end{align*}
The last inequality uses $b_1\le1$ and $2(11/12)^3>1$. If some $\gamma\ge11/12$ were admissible, monotonicity of $M_H$ would give
\[
        M_H\left(\frac{11}{12}\right)\le M_H(\gamma)\le1,
\]
a contradiction.
\end{proof}

\section{The Inverse Majorant Bound is Optimal}
\label{sec:majorant_optimal}

The key global input is obtained by reworking the construction in the proof of Naor and Regev's optimality theorem. We first record the notion of mixing needed to state it.

\begin{definition}[Mixed rounding scheme]\label{def:mixed-rounding}
Fix $d\in\mathbb N$. A $d$-dimensional \emph{mixed rounding scheme} is a probability distribution $\mu$ on pairs of measurable sign functions
\[
        f,g:\R^d\to\{\pm1\}.
\]
One pair $(f,g)$ is sampled from $\mu$ and then used for every vector in the rounding procedure. Its averaged correlation function is
\[
        H_\mu(t):=\E_{(f,g)\sim\mu}H_{f,g}(t).
\]
A \emph{limiting mixed correlation function} is a coefficientwise limit of averaged correlation functions of mixed rounding schemes, possibly in increasing dimensions.
\end{definition}

The admissible values from Definition~\ref{def:admissible-majorant} are the parameters appearing in the inverse-majorant bound~\eqref{eq:inverse-majorant-bound}. For an actual mixed scheme, the standard tensor preprocessing argument turns an admissible value $\gamma$ into the upper bound $K_G\le\pi/(2\gamma)$. The next lemma shows that, after allowing mixtures and increasing dimension, these bounds can approach $K_G$ itself.

\begin{lemma}[Optimality of the inverse-majorant bound]\label{lem:inverse-majorant-optimal}
There exist odd analytic limiting mixed correlation functions $H_k$ and admissible values $\gamma_k$ such that
\[
        \gamma_k\le\frac{\pi}{2K_G}
        \qquad\text{and}\qquad
        \gamma_k\longrightarrow\frac{\pi}{2K_G}.
\]
Equivalently, the resulting upper bounds satisfy
\[
        \frac{\pi}{2\gamma_k}\longrightarrow K_G.
\]
Thus, after allowing mixtures and increasing dimension, the inverse-majorant bound is asymptotically optimal.
\end{lemma}

\begin{proof}
We use the construction in the proof of Theorem~1.1 of \cite{naor2014krivine}. We do not use their theorem statement directly.

For each $k$, their equation~(4) gives a probability measure $\nu_k$ on pairs of sign assignments on $S^{k-1}$ whose averaged kernel is
\[
        \frac{1}{K_G}\ip{x}{y}.
\]
After radial extension, their equations~(5) and~(6) give an odd analytic normalized correlation function
\[
        H_k(t)=\frac{\pi}{2K_G}f_k(t),
\]
where $f_k$ is the function defined in their equation~(6). By partitioning the sphere into finitely many small Borel sets and extending the sampled signs as step functions, one obtains ordinary mixed rounding schemes whose averaged kernels converge uniformly to the kernel above. Hence $H_k$ is a limiting mixed correlation function in the sense of Definition~\ref{def:mixed-rounding}.

Naor and Regev write
\[
        f_k^{-1}(z)=\sum_{n\ge0}b_n(k)z^{2n+1}.
\]
Immediately before their Lemma~2.1, they choose a number $c_k\le1$ such that
\[
        \sum_{n\ge0}|b_n(k)|c_k^{2n+1}\le1,
\]
and Lemma~2.1 proves that $c_k\to1$. Define
\[
        \gamma_k:=\frac{\pi c_k}{2K_G}.
\]
Since
\[
        H_k^{-1}(z)=f_k^{-1}\left(\frac{2K_G}{\pi}z\right),
\]
the absolute inverse majorant of $H_k$ at $\gamma_k$ is exactly
\[
        \sum_{n\ge0}|b_n(k)|c_k^{2n+1}\le1.
\]
Thus $\gamma_k$ is admissible. Since $c_k\le1$ and $c_k\to1$,
\[
        \gamma_k\le\frac{\pi}{2K_G}
        \qquad\text{and}\qquad
        \gamma_k\longrightarrow\frac{\pi}{2K_G}.
\]
The equivalent statement about the resulting upper bounds follows by taking reciprocals.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:lower-bound}]
Let $H_k$ and $\gamma_k$ be supplied by Lemma~\ref{lem:inverse-majorant-optimal}. Sections~\ref{sec:preliminaries} and~\ref{sec:affine-strip} establish the affine coefficient inequality for every pair of odd sign functions in every dimension. It therefore holds for every mixed scheme, because $b_1$ and $b_3$ average linearly. Passing to the coefficientwise limit shows that
\[
        b_3(H_k)\ge2b_1(H_k)-\frac{11}{6}.
\]
This is the point at which preservation under mixing is used.

We also have $0<b_1(H_k)\le1$. Positivity follows because $\gamma_k$ is admissible. For the upper bound, every sign function $f$ satisfies
\[
        \norm{P_1f}
        =\sup_{\norm{u}=1}\left|\E[f(X)\ip{X}{u}]\right|
        \le\E|S|=\nu,
\]
so $|b_1(f,g)|\le(\pi/2)\nu^2=1$. This bound is also preserved under mixtures and coefficientwise limits.

Proposition~\ref{prop:majorant-barrier} now gives
\[
        \gamma_k\le\frac{11}{12}.
\]
Letting $k\to\infty$ and using Lemma~\ref{lem:inverse-majorant-optimal},
\[
        \frac{\pi}{2K_G}\le\frac{11}{12}.
\]
Rearranging proves the result.
\end{proof}


==> paper/statement_ai_use.tex <==
  \paragraph{Statement on AI use.}
  The research reported in this paper made extensive use of large language      
  models: GPT-5.5-Pro and GPT-5.6-Sol (OpenAI) served as the reasoning          
  models, and Claude Opus and Claude Fable~5 (Anthropic) as the coding          
  agents, operating within the AI research system described in the companion    paper~\cite{lisaha2026longhorizon}.               
  AI assistance was also used in preparing parts of this manuscript.            
  Every result stated as a theorem has been independently verified by the       
  authors, and the authors take full responsibility for the contents of this    
  paper. 

==> paper/technical_overview.tex <==
\section{Technical Overview}

Here, we provide the background and exposition of the main ideas in our work.

\subsection{The upper bound}

\paragraph{Classical Krivine rounding schemes.}
A classical Krivine scheme consists of odd sign functions \(f,g:\mathbb R^k\to\{-1,1\}\). Its normalized correlation function is
\(
    H_{f,g}(t):=\frac{\pi}{2}\mathbb E[f(X)g(Y)],
\)
where \(X,Y\) are standard Gaussian vectors with coordinatewise correlation \(t\). Suppose \(H^{-1}(z)=\sum_{n\geq 1}a_nz^n\), and let its \emph{majorant} series be  \(M(s):=\sum_{n\geq 1}|a_n|s^n\). Krivine's tensor preprocessing
(\cref{app:krivine-preprocessing})
gives
\(
    M(\gamma)\leq 1
    \implies 
    K_G\leq\frac{\pi}{2\gamma}.
\)
The upper-bound problem is therefore to construct a correlation function whose inverse has a large admissible  $\gamma$ so that $M(\gamma) = 1$.


\paragraph{Limiting Krivine rounding schemes.}
In ordinary Krivine schemes, we need individual Gaussian coordinates $X_i, Y_i$ to have coordinate-wise correlation $t$. We enlarge the search space by allowing $X_i, Y_i$ to have coordinate-wise correlation
\[
    \rho_i(t)=\sum_{\substack{d\geq 1\\ d\ \mathrm{odd}}}c_{i,d}t^d,
    \qquad
    \sum_d|c_{i,d}|\leq 1.
\]
This gives us more degrees of freedom in designing \(H\) whose associated \(M\) has larger \(\gamma\) satisfying $M(\gamma) = 1$.

% This flexibility in correlation structure allows us to find correlation functions \(H\) whose corresponding inverse majorants \(M\) have larger radii \(\gamma\).

% In our construction, we use the central limit theorem to realize arbitrary correlations as above.  
% In our construction, the powers \(t^d\) arise from Hermite polynomials: if \(U,V\) are correlated standard Gaussians, then \(\mathbb E[\operatorname{He}_d(U)\operatorname{He}_d(V)]=t^d\). 

% A limiting scheme is thus a fixed-dimensional model of a family of high-dimensional schemes built from normalized sums of Hermite polynomials.

% \rnote{The previous sentence is too vague and terse. You can just state the idea; we come up with an intermediate function and use central-limit theorem to realize arbitrary correlations as above.}


\paragraph{Approximation of limiting schemes using classical schemes.}
% While we may design the correlation function \(H\) to admit any \(\rho\) of the above structure, it is not immediately 
While we may design the correlations between variables to admit any \(\rho\) of the above structure, it is not immediately clear how the rounding algorithm works. 
Here, we show that any limiting scheme can in fact be approximated arbitrarily well by classical Krivine schemes, whose rounding algorithm is established. 
Therefore, it suffices to find a limiting scheme whose inverse majorant $M$ admits a high $\gamma$ with $M(\gamma) = 1$.
% In order to use limiting schemes, we show that every limiting scheme can be approximated by classical Krivine schemes.

More precisely, we construct a sequence $\mathcal{S}_1, \mathcal{S}_2, \ldots$ of classical Krivine schemes of increasing dimension \(k\), whose correlation functions $H_{\mathcal{S}_1}, H_{\mathcal{S}_2}, \dots$ converge to the correlation function $H_{\mathcal{S}}$ of a limiting scheme $\mathcal{S}$.
The main idea is to use the central limit theorem to collapse the increasing number of Gaussian random variables in the classical schemes \(\mathcal{S}_k = (f_k, g_k)\), where \(f_k, g_k : \mathbb{R}^k \to \{\pm 1\}\).

  
% Therefore, it suffices to find a limiting rounding scheme that gives a good upper bound on \(K_G\), and a way to generate a sequence of classical rounding schemes that asymptotically approximates it.

% The main idea of the proof is to use the central limit theorem to collapse the increasing dimensions.

% This lets us search for the upper-bound construction entirely within the class of limiting schemes.

% \rnote{Reads a bit like bullet points. No need for putting Vitali's theorem here. Need less jargon here.}


% 

\paragraph{The cubic--quintic scheme.}
A limiting Krivine scheme that attains the paper's stated upper bound on \(K_G\) is defined as follows.
% Our construction is a two-dimensional limiting scheme.
For suitable parameters \(s_3,s_5,\vartheta>0\), set
\[
    \rho(t):=
    \frac{t-s_3^2t^3+s_5^2t^5}{1+s_3^2+s_5^2},
\]
and use the partitions
\[
    f(w,x)=\operatorname{sgn}\!\left(w+\vartheta\operatorname{He}_3(x)\right),
    \qquad
    g(w,x)=\operatorname{sgn}\!\left(w-\vartheta\operatorname{He}_3(x)\right).
\]
We set the first coordinate \(w\) to have correlation \(\rho(t)\), and set the second coordinate \(x\) to have correlation \(t\).

% This limiting Krivine scheme gives our stated upper bound on \(K_G\).
% , and we show how to approximate it by classical schemes.

% The first Gaussian coordinate pair has correlation \(\rho(t)\), while the second has correlation \(t\). 
% The cubic direction is anti-aligned between the two sides and the quintic direction is aligned. 
% The parameters are chosen to cancel out the first nonlinear coefficients of the resulting correlation function. 
% \rnote{Could explicitly spell out, the final form $H_{f,g}$.}


\paragraph{Deriving the upper bound.}
In order to prove the upper bound (which we denote as $K_G^{UB}$), one needs to show that the inverse majorant $M(\gamma) \leq 1$ holds, for $\gamma=\frac{\pi}{2K_G^{UB}}$.
Doing this is non-trivial, and requires both an analytic step and a computational step. 

For the analytic step, write
\(H(t)=b_1t+\sum_{m\geq 3}b_mt^m\), and let
\(\Delta_H:=\sum_{m\geq 3}|b_m|\) denote its total nonlinear coefficient mass. We prove that it is sufficient to show 
\[
    \gamma+\Delta_H<b_1.
\]
Thus, rather than computing the inverse series \(H^{-1}\), it is enough to certify a lower bound on the linear coefficient \(b_1\) and an upper bound on \(\Delta_H\).
We then compute the first terms of $\{b_n\}$ using a formula involving the Hermite coefficients of $f$ and $g$, which are one-dimensional Gaussian integrals. Finally, we bound the tail of $\Delta_H$ through a single boundary-norm estimate for \(D^3H\), where \(D=t\frac{d}{dt}\). Rigorous interval arithmetic verifies the resulting finite collection of inequalities, yielding the claimed upper bound on \(K_G\).



% The computational verification is reduced to a simple criterion on the coefficients of the correlation function. 
% \rnote{What computational verification; this is a big jump from above. This is almost assuming familiarity with our previous paper.}
% Write
% \(H(t)=b_1t+\sum_{m\geq 3}b_mt^m\), and let
% \(\Delta_H:=\sum_{m\geq 3}|b_m|\) denote its total nonlinear coefficient mass. We show that
% \[
%     \gamma+\Delta_H<b_1
%     \qquad\Longrightarrow\qquad
%     M_H(\gamma)<1.
% \]
% Thus, rather than computing the inverse series \(H^{-1}\), it is enough to certify a lower bound on the linear coefficient \(b_1\) and an upper bound on \(\Delta_H\). We reduce these two estimates to a finite computer-assisted calculation. The initial coefficients of \(H\) are enclosed directly using one-dimensional Gaussian integrals, while the remaining coefficient tail is bounded through a single boundary-norm estimate for \(D^3H\), where \(D=t\frac{d}{dt}\). Rigorous interval arithmetic verifies the resulting finite collection of inequalities, yielding the claimed upper bound on \(K_G\).


\subsection{The lower bound}

\paragraph{Mixed Krivine schemes are optimal.}
Naor and Regev~\cite{naor2014krivine} proved that mixed Krivine schemes are asymptotically optimal. We use a quantitative consequence of their construction: there exist limiting mixed correlation functions \(H_k\) with admissible inverse-majorant parameters \(\gamma_k\) satisfying
\[
    \gamma_k\longrightarrow\frac{\pi}{2K_G}.
\]
Consequently, any universal upper bound on the admissible parameter of a Krivine correlation function gives a lower bound on \(K_G\).


\paragraph{The affine coefficient inequality.}
To obtain this upper bound, we ask which Taylor coefficients can actually arise from a Krivine correlation function. For odd sign functions \(f,g:\mathbb R^d\to\{-1,1\}\), write
\[
    H_{f,g}(t)=b_1t+b_3t^3+\cdots.
\]

Surprisingly, we show that there is the clean constraint on the first two coefficients:
\begin{equation}
    b_3\geq 2b_1-\frac{11}{6}.
    \label{eq:affine-coefficient-inequality}
\end{equation}
Its affine form is important, since it is preserved under mixtures and coefficientwise limits. 

Pushing the affine inequality to the inverse series $H^{-1}$ yields bounds on the inverse coefficients $a_1$ and $a_3$, which in turn gives $\gamma \leq \frac{11}{12}$. This results in the desired $K_G \geq \frac{6\pi}{11}$ .


% It also gives the desired barrier on the inverse majorant. Indeed, if
% \[
%     H^{-1}(z)=a_1z+a_3z^3+\cdots,
% \]
% then
% \[
%     a_1=\frac{1}{b_1},
%     \qquad
%     a_3=-\frac{b_3}{b_1^4}.
% \]
% Combining these identities with \eqref{eq:affine-coefficient-inequality}, the bound \(b_1\leq 1\), and the first two terms of the inverse majorant shows that every admissible parameter satisfies
% \[
%     \gamma\leq\frac{11}{12}.
% \]
% Since the asymptotically optimal family above has
% \(\gamma_k\to\pi/(2K_G)\), this yields
% \[
%     K_G\geq\frac{6\pi}{11}.
% \]

% \paragraph{Agreement and disagreement.}
% We prove \eqref{eq:affine-coefficient-inequality} using the Hermite expansions of \(f\) and \(g\). Let \(P_iF\) denote the projection of a function \(F\) onto Hermite degree \(i\). Mehler's identity gives
% \[
%     b_1=\frac{\pi}{2}\langle P_1f,P_1g\rangle,
%     \qquad
%     b_3=\frac{\pi}{2}\langle P_3f,P_3g\rangle.
% \]
% Writing
% \[
%     \nu:=\mathbb E|Z|=\sqrt{\frac{2}{\pi}},
% \]
% the affine inequality is therefore equivalent to
% \[
%     2\langle P_1f,P_1g\rangle
%     -\langle P_3f,P_3g\rangle
%     \leq \frac{11}{6}\nu^2.
% \]

% The useful change of variables is
% \[
%     h:=\frac{f+g}{2},
%     \qquad
%     k:=\frac{f-g}{2}.
% \]
% Here \(h\) is supported where \(f\) and \(g\) agree, while \(k\) is supported where they disagree. Moreover,
% \[
%     h,k\in\{-1,0,1\},
%     \qquad
%     h^2+k^2=1.
% \]
% Substituting \(f=h+k\) and \(g=h-k\), the left-hand side above becomes
% \[
%     2\|P_1h\|^2-2\|P_1k\|^2
%     -\|P_3h\|^2+\|P_3k\|^2.
% \]
% After dropping the nonpositive term \(-2\|P_1k\|^2\), it is enough to prove
% \begin{equation}
%     2\|P_1h\|^2-\|P_3h\|^2+\|P_3k\|^2
%     \leq \frac{11}{6}\nu^2.
%     \label{eq:agreement-disagreement-reduction}
% \end{equation}
% The first two terms involve the agreement function \(h\), while the final term measures the degree-three contribution of the disagreement function \(k\). We bound these two contributions separately.









% \paragraph{The affine coefficient inequality.}
% We can ask 



% Pushing the affine inequality to the inverse series $H^{-1}$ yields bounds on the inverse coefficients $a_1$ and $a_3$, which in turn gives $\gamma \leq \frac{11}{12}$. This results in the desired $K_G \leq \frac{6\pi}{11}$ .




% \paragraph{The affine coefficient inequality.}
% For a square-integrable function \(F\) on Gaussian space, let \(P_iF\) denote its orthogonal projection onto the Hermite polynomials of total degree \(i\). If
% \(H_{f,g}(t)=b_1t+b_3t^3+\cdots\) is the normalized correlation function of \(f\) and \(g\), then the basic orthogonality properties of Hermite polynomials give
% \(b_1=\frac{\pi}{2}\langle P_1f,P_1g\rangle\) and
% \(b_3=\frac{\pi}{2}\langle P_3f,P_3g\rangle\).
% Our main coefficient estimate is
% \begin{equation}
%     b_3\geq 2b_1-\frac{11}{6}.
%     \label{eq:affine-coefficient-inequality}
% \end{equation}
% Since \(\nu:=\mathbb E|Z|=\sqrt{2/\pi}\), this is equivalent to
% \[
%     2\langle P_1f,P_1g\rangle-\langle P_3f,P_3g\rangle
%     \leq \frac{11}{6}\nu^2.
% \]

% \rnote{Talking about $P_i F$ here seems a bit odd. I don't think that'll help in understanding yet. It might help to motivate the general approach. Something like ... We can ask what sets of coeffecients $(b_1, b_3, \cdots)$ can in fact be realized as Taylor-coefficients of a correlation function. Surprisingly, we show that there are some non-trivial clean constraints: ...}

\paragraph{Hermite expansion.} The approach to proving this is by looking at Hermite expansions of $f, g$. For a square-integrable function \(F\) on Gaussian space, let \(P_iF\) denote its orthogonal projection onto the Hermite polynomials of total degree \(i\).  If
\(H_{f,g}(t)=b_1t+b_3t^3+\cdots\) is the normalized correlation function of \(f\) and \(g\), then the basic orthogonality properties of Hermite polynomials give
\(b_1=\frac{\pi}{2}\langle P_1f,P_1g\rangle\) and
\(b_3=\frac{\pi}{2}\langle P_3f,P_3g\rangle\).
Our affine coefficient inequality is
\begin{equation*}
    b_3\geq 2b_1-\frac{11}{6}.
\end{equation*}
Since \(\nu:=\mathbb E|Z|=\sqrt{2/\pi}\), this is equivalent to
\[
    2\langle P_1f,P_1g\rangle-\langle P_3f,P_3g\rangle
    \leq \frac{11}{6}\nu^2.
\]

\paragraph{Agreement and disagreement.}
In order to prove the inequality, we make a key substitution. The substitution is to write
\(h:=(f+g)/2\) and \(k:=(f-g)/2\). The function \(h\) can be thought of as the \textit{agreement part}, where \(f\) and \(g\) agree, while \(k\) is the corresponding \textit{disagreement part}. Moreover,
\(h,k\in\{-1,0,1\}\) and \(h^2+k^2=1\).

% \rnote{This section seems like its jumping. After stating the inequality clearly for $b_3, b_1$, you can then say we approach proving this by looking at Hermite expansions of $f,g$. In particualr $b_3 = blah $ .. }
Substituting \(f=h+k\) and \(g=h-k\) into the preceding inequality, and discarding a nonpositive term, it suffices to prove
\begin{equation}
    2\|P_1h\|^2-\|P_3h\|^2+\|P_3k\|^2
    \leq \frac{11}{6}\nu^2.
    \label{eq:agreement-disagreement-reduction}
\end{equation}
The first two terms depend only on the agreement function \(h\), while the final term measures the degree-three contribution of the disagreement function \(k\). We bound these two parts separately.


\paragraph{Agreement terms.}
Rotate coordinates so that \(P_1h\) lies in a single Gaussian direction \(S\), and write
\(x:=\|P_1h\|/\nu\in[0,1]\). The positive agreement term is then
\(2\|P_1h\|^2=2\nu^2x^2\).

To control the helpful negative term \(-\|P_3h\|^2\), average \(h\) over all coordinates transverse to \(S\). Namely, writing the Gaussian input as \((S,T)\), set
\(A(s):=\mathbb E_T[h(s,T)]\). Then \(|A|\leq1\) and
\(\mathbb E[A(S)S]=\nu x\). A one-dimensional rearrangement inequality shows that this prescribed linear moment forces a cubic Hermite moment:
\[
    \|P_3h\|^2
    \geq
    \frac{\nu^2}{6}\Delta_+(x)^2
\]
for an explicit function \(\Delta\). Thus, a large linear agreement term necessarily creates a compensating cubic agreement term.

\paragraph{Disagreement term.}
For each fixed transverse vector \(t\), consider the one-dimensional slice
\(u_t(s):=k(s,t)\). Since \(k\in\{-1,0,1\}\), each \(u_t\) is a ternary function on the Gaussian line. The degree-three Hermite decomposition implies
\[
    \|P_3k\|^2
    \leq
    \mathbb E_T V(u_T),
    \qquad
    V(u):=
    \sum_{j=0}^3
    \bigl(\mathbb E[u(Z)\psi_j(Z)]\bigr)^2.
\]
We control these first four Hermite moments through the weighted support
\(\beta(u):=\mathbb E[|Z|u(Z)^2]\). The key one-dimensional estimate is
\begin{equation}
    V(u)\leq 3\nu\beta(u)-\beta(u)^2.
    \label{eq:one-dimensional-support-inequality}
\end{equation}
Conceptually, this says that a ternary function cannot have both a support concentrated cheaply near the origin and a large projection onto all Hermite degrees at most three. The inequality admits an exact finite-dimensional dual reduction. After introducing a support price \(c\), the optimizing ternary function has the threshold form
\(
    u(z)=\operatorname{sgn}(p(z))
    \mathbf 1_{\{|p(z)|\geq c|z|\}},
\)
where \(p\) is a unit cubic Hermite polynomial. The resulting one-dimensional Gaussian integral inequalities are verified using outward-rounded interval arithmetic. Finally, \(h^2+k^2=1\) relates the average weighted support of the slices \(u_T\) to the agreement parameter \(x\). Combining this relation with
\eqref{eq:one-dimensional-support-inequality} gives an explicit upper bound on
\(\|P_3k\|^2\) in terms of \(x\). Together with the agreement estimate, this reduces
\eqref{eq:agreement-disagreement-reduction} to an elementary scalar inequality on
\(x\in[0,1]\), proving \eqref{eq:affine-coefficient-inequality}.




% \section{Technical Overview}

% Here, we provide an exposition of the main ideas in our work. 

% \paragraph{Classical Krivine schemes.} ... 

% \paragraph{Limiting Krivine schemes.} ... 

% \paragraph{Approximation of limiting schemes with classical schemes.} ...

% \paragraph{The cubic-quintic scheme.} ...

% \paragraph{Deriving the upper bound.} ...

% \paragraph{Krivine schemes are optimal.} ... 

% \paragraph{Affine inequality.} ... 

% \paragraph{Deriving the lower bound.} ... 

% \paragraph{Technical overview of the Lower Bound.} We prove the following theorem:

% \begin{theorem}\label{thm:lower-bound}
% The Grothendieck constant satisfies
% \[
%         K_G\ge\frac{6\pi}{11} \approx 1.7136.
% \]
% \end{theorem}

% A sketch of the proof is as follows. 

% First, recall the inverse-series step in Krivine's rounding argument. If
% \[
%         H^{-1}(z)=\sum_{j\ge0}a_{2j+1}z^{2j+1},
% \]
% define the absolute-coefficient majorant $M_H(s):=\sum_{j\ge0}|a_{2j+1}|s^{2j+1}$. The standard tensor preprocessing gives the implication
% \begin{equation}
%         M_H(\gamma)\le1
%         \quad\Longrightarrow\quad
%         K_G\le\frac{\pi}{2\gamma}.
%         \label{eq:inverse-majorant-bound}
% \end{equation}
% We refer to~\eqref{eq:inverse-majorant-bound} as the \emph{inverse-majorant bound}.

% The conceptual starting point is the theorem of Naor and Regev that Krivine schemes are optimal \cite{naor2014krivine}. By reworking the construction in their proof, we show that the inverse-majorant bound is itself asymptotically optimal after allowing mixtures and increasing dimension: there are limiting mixed correlation functions with admissible parameters converging to $\pi/(2K_G)$. This transfer is established in Section~\ref{sec:majorant_optimal}.

% It therefore remains to prove a universal upper bound on such admissible parameters. For arbitrary odd measurable sign functions $f,g:\R^d\to\{\pm1\}$, write
% \[
%         H_{f,g}(t)=b_1t+b_3t^3+b_5t^5+\cdots.
% \]
% The technical core of the argument is the affine inequality
% \[
%         b_3\ge 2b_1-\frac{11}{6}.
% \]
% Section~\ref{sec:preliminaries} sets up the Gaussian--Hermite formulation, and Section~\ref{sec:affine-strip} proves this inequality by decomposing $f$ and $g$ into their agreement and disagreement parts and reducing the required estimates to one-dimensional inequalities. Its linearity in $(b_1,b_3)$ is essential, because it makes the inequality invariant under mixtures and coefficientwise limits.

% Section~\ref{sec:strip_majorant} then shows that the affine inequality controls the inverse-majorant bound: every admissible value must satisfy $\gamma\le11/12$. Applying this barrier to the asymptotically optimal sequence constructed in Section~\ref{sec:majorant_optimal} gives
% \[
%         \frac{\pi}{2K_G}\le\frac{11}{12},
% \]
% which is exactly Theorem~\ref{thm:lower-bound}.


% \paragraph{Technical overview of the Upper Bound}. (Give references to sections of the technical part)

% - Recall classical Krivine schemes... (standard correlation)

% - Define Limiting Krivine schemes... (arbitrary correlation)

% - Show that these schemes can be arbitrarily approximated by classical (finite) Krivine schemes, in a specific sense

% - Therefore inverse-majorant bound on Limiting Krivine schemes translates to upper bounds on $K_G$, so this is a new search space

% - We then study a specific instantiation of limiting Krivine schemes: the cubic--quintic scheme...

% - We show how to derive the inverse-majorant bound on this by bounding the tail of the taylor expansion of $H$... 



